The Shape of Alerts: Detecting Malware Using Distributed Detectors by Robustly Amplifying Transient Correlations

We introduce a new malware detector - Shape-GD - that aggregates per-machine detectors into a robust global detector. Shape-GD is based on two insights: 1. Structural: actions such as visiting a website (waterhole attack) by nodes correlate well with malware spread, and create dynamic neighborhoods of nodes that were exposed to the same attack vector. However, neighborhood sizes vary unpredictably and require aggregating an unpredictable number of local detectors' outputs into a global alert. 2. Statistical: feature vectors corresponding to true and false positives of local detectors have markedly different conditional distributions - i.e. their shapes differ. The shape of neighborhoods can identify infected neighborhoods without having to estimate neighborhood sizes - on 5 years of Symantec detectors' logs, Shape-GD reduces false positives from ~1M down to ~110K and raises alerts 345 days (on average) before commercial anti-virus products; in a waterhole attack simulated using Yahoo web-service logs, Shape-GD detects infected machines when only ~100 of ~550K are compromised.

==> abstract.tex <==

WARNING!!!!

UNUSED.

ABSTRACT in paper.tex

% Anomaly-based intrusion detection systems promise to expose 
% previously unknown malware
% %i.e., new malware whose signatures are not yet present in malware databases,
% and thus form an important security primitive.
% %model benign applications' system calls and network traffic
% However, even the best anomaly detectors suffer from high false
% positives and are susceptible to mimicry attacks (where
% malware is deliberately crafted to look very similar to benign programs).

% In this paper, we address the challenge of composing noisy
% per-device local detectors into an accurate and robust global
% anomaly detector.  % Specifically, we propose to dynamically
% construct communities of local detectors and aggregate the local
% detector outputs in order to pin-point anomalous communities.
% Interestingly, since our global detector adapts to changes in
% underlying network to identify malware-infested neighborhoods
% dynamically, we do not have to place static observers on network
% nodes.  % We evaluate our technique on networks A, B, and C, where
% each node on the network is a mobile device running Android
% applications with real human user inputs, and find that our
% technique significantly improves the time to detection of new
% malware compared to a naive baseline. %by X\%
%
Behavioral malware detectors, by using statistical methods, promise to
expose previously unknown malware and thus form an important security
primitive. However, even the best detectors suffer from high false
positives and negatives.  In this paper, we address the challenge of
composing a community of weak per-device behavioral detectors (aka
local detectors) into an accurate and robust global anomaly detector.

Our system consists of feature-vector driven local detectors at
individual nodes; aggregating alerts (that flag the
possibility of malware being present) from this community of local
detectors enables global inference of malware.
%
% Specifically, we propose to dynamically construct communities of local
% detectors and aggregate the local detector outputs in order to
% pin-point anomalous communities.
%
%
Our system -- Shape GD -- combines two insights -- one structural and
the other statistical: {\em Structural:} actions such as visiting a
website (waterhole attack) or membership in a shared email thread
(phishing attack) by nodes
correlate well with malware spread
and creates a {\em neighbohood} of nodes; 
and {\em Statistical:} feature vectors corresponding
to true and false positives of local detectors have markedly different
conditional distributions (i.e. their histogram shapes differ).



% Crucially this
% property allows our global detector to be robust to noise in estimates
% of community size and data reporting behavior by individual users.


% \todo{We prototype our system on a community of Android devices.  Using 18
% different local detectors and 10 different malware tainted Android
% apps (AVG, Wikipedia, Yelp, etc.), we show, using a custom-built
% evaluation platform on which popular mobile applications are driven by
% real user inputs, that our global detector significantly improves
% malware detection probabilities in a variety of network settings.}

We evaluate Shape GD through emulation on a community of Windows
systems, where we collect data from a few thousand malware and benign
applications. We evaluate our system in the settings of a phishing
attack in a corporate setting, and a waterhole attack through a
popular website. In both these scenarios, we show that Shape GD
detects the presence of malware robustly, and at early stages of
infection.


% \item[3.] \textbf{Local/Global Detector Experiments:} We have
%   conducted experiments with 18 local detectors (random forest, SVM,
%   decision trees, ensemble methods, etc) and 10 Android apps
%   (Wikipedia, AVG, Walmart, Yelp, among others). First, we confirm the
%   premise that, on Android, a vast majority of local detectors' true
%   and false positive rates are about 80\%:15\% (see
%   Figure~\ref{fig:ROC}). Importantly, our key observation that the
%   conditional distributions differ at the global level, is borne out
%   by our experiments.  For 8 out of 10 apps, we observe a sharp
%   statistical separation between the scores resulting from the local
%   detector's TP and FP feature vectors. This manifests in the global
%   ROC curves: With 3000 samples fed to LDs and filtering by their
%   alerts, we can get a global TP:FP rates arbitrarily close to
%   100\%:0\% for 5 apps (AVG, Buzzfeed, All Recipes, Wikipedia, Zedge),
%   and about 95\%:5\% for two apps (see Figures~\ref{fig:GD_ROC} for
%   details of other apps). These can be further driven down
%   (theoretically, exponentially fast) by increasing the data set size.


% \item[4.] \textbf{Network Experiments:} We experiment with three
%   network topologies — grids, random graphs, and social network graphs
%   — and evaluate our global detector using standard generative models
%   for malware propagation on these graphs. The combination of shape
%   and censoring alerts enables malware to be detected when less than
%   10\% of the nodes are infected at false positive rate about 5\% (for
%   social network) and less than 1\% for the other networks with the
%   Wikipedia app (see Figure~\ref{fig:detect_vs_prctile}). Further, the number of
%   observations needed to detect at this level of reliability grows
%   only logarithmically with the network size (i.e., only a vanishingly
%   small fraction of the community need to report alerts, see
%   Figure~\ref{fig:wiki_vs_censoring_threshold}).


% Our global detector the presence of malware using (a) biased samples
% (self selection bias from local detectors) and the shape difference
% between the conditional distributions of FP feature vectors and TP
% feature vectors, and (b) alert censoring using thresholding based on
% graph-dependent alert densities. Crucially, this algorithm is robust
% to community size and data reporting dynamics, and the resulting
% variability in sample sizes.


% Interestingly, since our global detector adapts to changes in underlying
% network to identify malware-infested neighborhoods dynamically,  
% we do not have to place static observers on network nodes. 
% % 
% We evaluate our technique on networks A, B, and C, where each node on the
% network is a mobile device running Android applications with real human user
% inputs, and find that our technique significantly 
% improves the time to detection of new malware compared to a naive baseline. %by X\%




% \item[1.] \textbf{Algorithm:} We develop a novel global detector that
%   infers the presence of malware using (a) biased samples (self
%   selection bias from LDs) and the shape difference between the
%   conditional distributions of FP feature vectors and TP feature
%   vectors, and (b) alert censoring using thresholding based on
%   graph-dependent alert densities. Crucially, this algorithm is robust
%   to community size and data reporting dynamics, and the resulting
%   variability in sample sizes.

% \item[2.] \textbf{Platform:} We build a realistic evaluation platform
%   on which popular mobile applications are driven by real user inputs,
%   where we guarantee that a diverse set of malware payloads execute
%   correctly, and simulate a variety of network models for malware
%   propagation using a large network of emulators. \todo{number for
%     hours of sim and dataset}

% \item[3.] \textbf{Local/Global Detector Experiments:} We have
%   conducted experiments with 18 local detectors (random forest, SVM,
%   decision trees, ensemble methods, etc) and 10 Android apps
%   (Wikipedia, AVG, Walmart, Yelp, among others). First, we confirm the
%   premise that, on Android, a vast majority of local detectors' true
%   and false positive rates are about 80\%:15\% (see
%   Figure~\ref{fig:ROC}). Importantly, our key observation that the
%   conditional distributions differ at the global level, is borne out
%   by our experiments.  For 8 out of 10 apps, we observe a sharp
%   statistical separation between the scores resulting from the local
%   detector's TP and FP feature vectors. This manifests in the global
%   ROC curves: With 3000 samples fed to LDs and filtering by their
%   alerts, we can get a global TP:FP rates arbitrarily close to
%   100\%:0\% for 5 apps (AVG, Buzzfeed, All Recipes, Wikipedia, Zedge),
%   and about 95\%:5\% for two apps (see Figures~\ref{fig:GD_ROC} for
%   details of other apps). These can be further driven down
%   (theoretically, exponentially fast) by increasing the data set size.


% \item[4.] \textbf{Network Experiments:} We experiment with three
%   network topologies — grids, random graphs, and social network graphs
%   — and evaluate our global detector using standard generative models
%   for malware propagation on these graphs. The combination of shape
%   and censoring alerts enables malware to be detected when less than
%   10\% of the nodes are infected at false positive rate about 5\% (for
%   social network) and less than 1\% for the other networks with the
%   Wipikepdia app (see Figure~\ref{fig:detect_vs_prctile}). Further, the number of
%   observations needed to detect at this level of reliability grows
%   only logarithmically with the network size (i.e., only a vanishingly
%   small fraction of the community need to report alerts, see
%   Figure~\ref{fig:wiki_vs_censoring_threshold}).


==> accenture.tex <==
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/accenture/histogram/histogram.eps}\par
   \caption{Histogram of benign and malicious ShapeScores in an enterprise network: 
            The ShapeScore is computed
     from neighborhood sizes of 1,000 FVs (experiment repeated 100
     times to generate the histograms).  Though the histograms overlap,
     Shape-based GD can reliably flag some malicious neighborhoods.}
\label{fig:accenture-hist}
\end{figure}


We applied Shape GD to one month (February 2016) of security logs in a Fortune
500 enterprise. This dataset is extremely noisy and heterogeneous -- unlike our
homogeneous dataset in the paper which models deployments like {\tt osquery} in 
Facebook. In contrast, this dataset includes an average of 
almost 250 Million security-related log entries per day from almost 20 different local
detectors (Blue Coat, Symantec, McAfee, F5, Cisco, etc), generated from a system with over
150K devices (including personal computers, mobile devices, servers, firewalls,
routers, and other network elements), all recorded in a `market leading' SIEM
tool for global malware analysis. Devices come and go, log entries can be
delayed by up to two months, and logs with confirmed signature-based malware
infections are very rare (0.29\%). Hence, ground truth infection data is hard
to get. The goal here is to filter the 5.5 Billion log entries including 700,000
different server IPs in February 2016 to a few tens of incidents that can be manually
analyzed.



%We deployed Shape GD in a SIEM environment within Accenture company~\cite{accenture_company}
%and conducted preliminary experiments.
%Accenture's SIEM infrastructure stores logs collected across 100,000 devices over 
%a year long period; it contains 65 billions of log entries total.
%%Out of 200,000 reporting devices <?> are end hosts, the others are network
%%devices. 
%The data come from 18 different monitoring tools such
%ArcSight, Blue Coat, F5, Cisco and etc. Almost all end host devices 
%run antiviruses supplied by Symantec and Microsoft.
%
%For processing such enormous amount of data we choose Apache Spark~\cite{apache_spark},
%a large-scale data processing framework, which run
%in a cluster composed of 18 worker nodes equipped
%with 2.74 TB of RAM and 576 virtual cores.
%
%The way the data is organized imposes a set of new challenges that are
%orthogonal to the design of Shape GD, but affect its detection results.

First, the data is high-dimensional and sparse. Each log entry contains 468
categories filled out with mostly categorical values, and most rows have no
content or are filled out with uninformative default values. 
%The architects of Accenture's SIEM chose such a high-dimensional
%representation to unify logs reported by different tools that are not designed
%to work together.
Directly using one-hot encoding to represent categorical data produces a
330,000-dimensional vector, hence we use the top 20 security-critical
dimensions and encode data manually before applying one-hot encoding to yield
364 dimensional vectors. Determining unique identities for devices and
identifying usernames and domain-names associated with IP addresses in rows
takes several analysis passes over the sparse dataset.
%combination of manual encoding of data and ch whose dimensionality is a sum of
%the number of observed distinct values within each category. Obviously, such
%extreme dimensionality which is far beyond Spark's data processing
%capabilities. To address this challenge, we select only a subset of
%categories, perform manual feature encoding based on our expertise, and only
%after that we use one-hot encoding.  To speed up data processing, we have to
%stick to small number of categories (fewer than we would like to use), thus
%the resulting feature vectors have only 364 dimensions.
%
%The second challenge is matching log entries reported by different monitoring
%tools. Their logs may have inconsistent fields filled out, which prevents easy
%matching and requires to do multiple passes on the database to extract
%information. 
%
%
%: high-dimensional data, hard and expensive to correlate logs provided
%different tools, logs contain lots of missing or default values, and there is
%little documentation explaining what system events make all these monitoring
%tools generate log events. For example, one tool may report device's IP, while
%the other may fill it out with a loopback-address "127.0.0.1".  In this case,
%we have to extract user names associated with a specific set of IPs, and then
%query the database again to extract logs associated with those users.  The
%problem stems from the fact that the monitoring tools were not been designed
%or configured for large-scale data processing, instead, each of them reports
%its own data only.


%\textbf{Results}
%We obtained preliminary results by running Shape GD on one month of data --
%the data that was logged in Februrary 2016, the first month when the SIEM 
%became fully functional. This data subset includes 5.5 billion of log entries
%coming from 700,000 different IPs.% and 355,000 unique accounts.


We form neighborhoods based on the accessed domains, thus a neighborhood 
includes devices accessing different URLs hosted in the same domain. 
This yields 400,000 unique neighborhoods.
%Even such a coarse-grained neighborhood template leads to forming
%an enormous number of neighborhoods -- 400,000 unique neighborhoods.
%Such neighborhoods capture waterhole attacks and malware communication with
%its command and control servers.
We apply two heuristics to rank those neighborhoods in terms of their
maliciousness. First, we run SecureRank algorithm, 
which is an adaptation of PageRank algorithm for the problem
of ranking domains in terms of their potential maliciousness.
We initialize the SecureRank algorithm by labeling domains belonging to certain Blue Coat's
categories (e.g. Suspicious, Spam, Scam/Questionable/Illegal, etc) as malicious.
%The actual 'malicious' weight we assign depends on empirical observations that we 
%made when analyzing data.
SecureRank 
%converges fast to the final solution and 
outputs a sorted list of
domain names based on their malicious score.
%We manually checked some domains in the malicious part of the spectrum and
%discovered that 
%%they are not necessarily malicious, i.e. 
%SecureRank has high false positive rate.
%\mikhail{TODO: how much?}

%This is why we employ 
Our second heuristic is to query VirusTotal scanner to obtain
information about security incidents related to a particular domain.
VirusTotal's reports include the number of malicious URLs, the number of
malware samples communicating to a particular domain, the number of samples
embedding URL strings leading to the domain under investigation. If VirusTotal
does not have information about incidents related to a particular domain, then
we discard the domain from the list of suspicious domains (i.e., the candidates
for neighborhood formation process).
%We extracted end host alerts from the logs to validate the hypothesis whether
%those two heuristics are enough to conclude that a domain is compromised.  And
%it turns out that they have 
%Even filtering domains using VirusTotal yields an unacceptably high false
%positive rate.  \mikhail{TODO: How much?}

\noindent \textbf{Training Shape GD.} To build a reference histogram, we select the top
20 benign domains given by Secure Rank (and confirmed using VirusTotal),
aggregate all 31 Million log records related to communication with those
domains, and learn a reference vector-histogram.  The next step in the training
process is to determine threshold $\gamma$, which depends on the distribution
of benign neighborhood scores.  For this reason, we select the top 100 benign
domains from our domain list (not including the previously used 20 domains),
build neighborhoods for each domain, randomly select 1,000 records from each
neighborhood, and compute ShapeScore.  We select a thousand records because we
want our Shape GD to operate on domains that have more than a thousand records.
Thus, if during testing a domain's neighborhood yields less than a thousand
records, we have to discard it.  
%We experiment with three settings of the threshold $\gamma$ -- 97-th, 98-th, and 99-th percentiles.

{
\footnotesize
\begin{table}[htb]	
	\resizebox{\columnwidth}{!}{%
    \begin{tabular}{| l | l | l |}
    \hline
    $\gamma$, percentile & Flagged nbds & Prevented incidents \\ \hline
    97 & 25 & 15 \\
    98 & 15 & 11 \\
    99 & 5  & 7 \\  \hline
    \end{tabular}
    }
    \label{tbl:accenture_results}
   \caption{Shape GD prioritizing a total of 100 candidate neighborhoods and 30 confirmed exploits.}
%   	\caption{{\small \sf Running Shape GD on an enterprise's heterogeneous SIEM infrastructure. 
%      Shape GD takes as input the top 100 suspicious domains found using SecureRank and VirusTotal,
%      that generate a total to 30 alerts in the dataset. 
%   	We vary the threshold parameter $\gamma$ from 97th up to 99th percentile and observe that
%   	at 97 percentile, Shape GD flags only 25 neighborhoods/domains as malicious and yet pre-empt 15 of the 30
%      exploits.  
%      %and the number of 
%   	At 99 percentile, the prevented exploits drops from 15 to 7; however, the confidence that
%   	a flagged neighborhood is actually malicious increases.}}
\end{table}
}

\noindent \textbf{Testing Shape GD.} We select the top 100 {\em suspicious} domains
according to SecureRank followed by VirusTotal, form a neighborhood of end hosts using
each of these 100 domains,
select the first 1000 records in chronological order, 
%(we want to detect malware as soon as possible),
and run Shape GD. 
%Figure~\ref{fig:accenture-hist} shows the histogram of 
%ShapeScores generated by benign (blue bars) and malicious (red bars) neighborhoods.
%It is clear that malicious and benign neighborhoods' scores do not separate 
%as well as in our homogeneous system -- 
%the diversity of LDs and their feature vectors, and the sparsity
%of this dataset makes it an {\em extremely} challenging deployment point.
%In effect, the reduced detection rate implies that
%Yet, one can see that ShapeScore is discriminative enough to separate
%out a significant fraction of malicious neighborhoods. 


We experimented with three values of the threshold $\gamma$ -- 97th, 98th, 99th
percentiles (Table~\ref{tbl:accenture_results}). For each threshold we computed
the number of security incidents that could have been prevented during February
once Shape GD declares the domain (i.e.  its neighborhood) as infected.
%time period, this statistics is based on the number of end host alerts in our
%database.
These thresholds result in labeling 25, 15, and 5 domains/neighborhoods
(respectively) as infected, and yet pre-empt 15, 11, and 7 (respectively) of
the 30 exploits.  Increasing $\gamma$ from 97th percentile to 99th percentile
enables an analyst to trade off the number of domains that need to be
manually analyzed with the number of exploits that were pre-empted.

%but increases Shape GD's discriminative ability
%from 3$\times$ up to 7$\times$ (the ratio of the fraction of domains that an
%analyst needs to check to the fraction of exploits that she will prevent).


%We analyzed the end hosts that access those hosts in February and counted the number
%of alerts that the end host protection system raised when an end host accessed one
%of those domains. Such an estimate is very conservative in the sense that the end host 
%protection system might have raised an alert or blocked a sample when malware
%was performing local actions without trying to access the Internet.

%In the far right column -- ShapeScore -- we can easily spot an outlier domain
%{\tt j.maxmind.com}.  Its ShapeScore is 2--3 times higher than the threshold.
%On querying VirusTotal, we found out that this domain has hosted 57 malicious
%URLs, 100 malware samples have communicated with this domain and 100 samples
%embed this domain in their strings.  

%Based on the data in the SIEM data base,
%seven users had malware communicating to this host in February alone {\em
%after} Shape GD had raised an alert. 

%Shape GD could have reliably spotted this domain
%name and if the incident response team had processed the results fast enough, at least
%seven infections could have been prevented.

%For each value of $\gamma$ threshold we compute the number of incidents that could 
%have been prevented, the same parameter per each flagged neighborhood and for each 
%unflagged neighborhood (the last two lines in the table). And we see 

%We are still working on increasing of Shape GD's accuracy when applying it to the
%existing SIEM infrastructures, and also we are working on co-design of
%SIEM infrastructures and Shape GD to achieve the best possible detection rate.


%\begin{table}[htb]	
%	\resizebox{\columnwidth}{!}{%
%    \begin{tabular}{| l | l | l | l |}
%    \hline
%    Parameter & $\gamma$ = 97th prctile & $\gamma$ = 98th prctile &
%				$\gamma$ = 99th prctile \\ \hline
%	Flagged neighborhoods & 25 & 15 & 5 \\
%	Prevented incidents & 15 & 11 & 7 \\
% 	Shape GD's discriminative ability & 3x & 3.3x & 5.8x \\ \hline
%    \end{tabular}
%    }
%    \label{tbl:accenture_results}
%   	\caption{Running Shape GD in Accenture's SIEM infrastructure. 
%   	For each neighborhood, we show results for three values of the threshold
%   	$\gamma$ -- 97th, 98th, and 99th percentiles. The values in the corresponding
%   	column shows the number of infected user accounts whose infections could be 
%   	prevented if had Shape GD been deployed in the beginning of 2016.}
%\end{table}

%\begin{table}[htb]	
%	\resizebox{\columnwidth}{!}{%
%    \begin{tabular}{| l | l | l | l | l |}
%    \hline
%    Domain name & $\gamma$ = 97th & $\gamma$ = 98th &
%				$\gamma$ = 99th  & ShapeScore \\ \hline
%    j.maxmind.com & 7 & 7 & 7 & 67.74\\ 
%	grarhibck.com & 0 & 0 & 0 & 42.06\\ 
%	mashable.com & 0 & 0 & 0 & 36.42\\ 
%	delivery.adforgecdn.com & 0 & 0 & 0 & 29.50\\ 
%	beacon.securestudies.com & 0 & 0 & 0 & 28.81\\ 
%	tools.dvdvideosoft.com & 0 & 0 &  & 27.84\\ 
%	videolan.org & 0 & 0 &  & 26.91\\ 
%	euwfb.adsrvr.org & 1 & 1 &  & 26.25\\ 
%	t12.baidu.com & 1 & 1 &  & 25.98\\ 
%	creative.ad120m.com & 0 & 0 &  & 25.83\\ 
%	serve.popads.net & 1 & 1 &  & 25.48\\ 
%	yui.yahooapis.com & 0 & 0 &  & 25.44\\ 
%	sovrn-merge.openx.net & 0 & 0 &  & 25.30\\ 
%	cm.pos.baidu.com & 1 & 1 &  & 25.24\\ 
%	eclick.baidu.com & 0 & 0 &  & 25.09\\ 
%	bkrtx.com & 0 &  &  & 24.13\\ 
%	c.fqtag.com & 0 &  &  & 24.12\\ 
%	groupon.com & 0 &  &  & 24.03\\ 
%	xp.apple.com & 1 &  &  & 23.85\\ 
%	platform.stumbleupon.com & 0 &  &  & 23.71\\ 
%	cpro.baidu.com & 1 &  &  & 23.43\\ 
%	oz.cnzz.com & 0 &  &  & 23.19\\ 
%	go.oclasrv.com & 1 &  &  & 22.71\\ 
%	arcadeparlor.com & 0 &  &  & 22.70\\ 
%	letterboxd.com & 1 &  &  & 22.58\\ \hline \hline
%	Prevented incidents & 15 & 11 & 7 & \\ \hline
% 	Prevented incidents per nbd & 0.60 & 0.73 & 1.40 &  \\ \hline 
% 	Incidents per missed nbd & 0.20 & 0.22 & 0.24 &  \\ \hline 
%    \end{tabular}
%    }
%    \label{tbl:accenture_results}
%   	\caption{Running Shape GD in Accenture's SIEM infrastructure. 
%   	For each neighborhood, we show results for three values of the threshold
%   	$\gamma$ -- 97th, 98th, and 99th percentiles. The values in the corresponding
%   	column shows the number of infected user accounts whose infections could be 
%   	prevented if had Shape GD been deployed in the beginning of 2016.}
%\end{table}


==> algorithm_2.tex <==
\begin{figure}[tbp]
   \vspace{-0.0in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/algo_schema.pdf}\par
   \caption{\sysname{}'s implementation.}
   \vspace{-0.2in}
\label{fig:algo_schema}
\end{figure}

The algorithm consists of feature extraction, local detector (LD), and the
global detector (GD) (Figure~\ref{fig:algo_schema}). Our key innovations are in the GD, however, 
we also discuss feature extraction and LD design for completeness.
These steps differ across the case studies, therefore, when describing each of them,
first, we focus on their high-level overview, and after that we dive into details.


\subsection{Local Detectors}
\label{sec:local_detectors}
In both case studies local detectors (LDs) analyze executable files, 
however, they use different file abstractions -- static file analysis (Symantec Wine) 
because the original files are unavailable and
dynamic traces of executed system calls (waterhole case study).
In the Symantec Wine case study we use an additional local detector -- domain name classifier, 
which detects suspicious domains by analyzing their VirusTotal domain reports.

%In the Symantec Wine experiment LDs focus on static features of executable files because 
%the files are not available -- we have only an access to VirusTotal reports only that summarize them. Also we use an additional 
%local detector -- domain name classifier, which detects suspicious domains by analyzing
%their VirusTotal domain reports.
%And in the waterhole case study LDs extract features from 
%dynamic system call traces. 

%Even though particular feature extraction steps are dataset specific, both LDs use similar algorithms
%to spot suspicious feature vectors -- XGBoost~\cite{xgboost} and Random Forest~\cite{}.
Both LD algorithms leverage the state-of-the-art techniques in
automated malware detection. % to generate an sequence of {\em alerts} from the feature vector (FV) sequence. 
Specifically, the LD algorithm  uses both its internal state and the {\em current} feature vector (FV)
to generate an alert if it thinks that this FV corresponds to
malware.%, and produces no alert if it thinks that the current FV is benign. 
Henceforth, we define an {\bf alert-FV} to be an FV that
generates an LD alert (either true or false positive). 

Despite performing case study specific feature extraction, LDs employ similar algorithms 
as a binary classifier for malware detection: 
Boosted Decision Trees~\cite{xgboost} (Symantec Wine case study) and
Random Forest (waterhole case study).
These algorithms achieve the best performance on the training data set 
among the classifiers from a prior survey~\cite{Canali2012} 
and scale up well to process millions of FVs.
%they have been shown to be robust to adversarial inputs~\cite{},


\textbf{Symantec Wine.}
In the Symantec Wine цасе студы, we use two types of local detectors: 
a file-level LD and a domain name classifier. Both of them work with VirusTotal reports that
summarize the results of file analysis and domain analysis respectively.

\textbf{File-level LD.}
We adapt an LD from the prior work~\cite{vt_report_classification}.
It primarily relies on a lightweight file analysis, which scales well when processing millions of downloads per day.
Specifically, the LD extracts syntactic features from a file and applies a binary classification algorithm 
that labels a file as either malicious or benign.

The LD is designed to run existing commercial tools such as TRID, ClamAV, Symantec on a binary file, analyze statically imported libraries and functions, detect common packers, check whether a file is digitally signed or not, and collect its binary metadata. 
VirusTotal combines outputs of these tools into a single file report and makes it available online, which
we directly use as the LD's input.

\mikhail{REMOVE
The core LD's component is a feature extraction algorithm, i.e. an algorithm converting textual VirusTotal reports into
fixed-length feature vectors used as input by a classifier. Even though the original algorithm ~\cite{vt_report_classification}
allows the classifier to achieve high accuracy, it is inappropriate in our case because
it produces very high-dimensional feature
vectors that have limited usability due to the "curse of dimensionality" 
and due to high memory consumption.
We use a common method for dimensionality reduction -- feature hashing~\cite{feature_hashing}. 
Empirically we found that the output dimensionality of 1024 allows us to 
achieve the best trade-off between LD's accuracy and resource consumption. 
}
%Finally, the LD uses an xgboost classifier~\cite{xgboost}, which is trained using 10-fold cross-validation 
%and area-under-the-curve (AUC) as the classifier's objective to deal with class imbalance.
%It achieves 97.61\% AUC, and we chose the operating point of 5.0\% false
%positive rate and 90.47\% true positive rate.




\textbf{Domain name classifier.}
\begin{figure}[tbp]
   \vspace{-0.0in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/symantec/domain_name_classifier/domain_features.pdf}\par
   \caption{Domain name classifier's features.}
   \vspace{-0.2in}
\label{fig:domain_features}
\end{figure}
The domain name classifier analyzes VirusTotal domain reports and identifies domains that are likely to distribute malicious files.
It uses as input VirusTotal domain-level reports that aggregate domain classification produced by other commercial tools such as
Dr. Web, Websense ThreatSeeker, and VirusTotal and statistics computed by VirusTotal itself (Table~\ref{fig:domain_features}).
Each of those tools categorizes a domain based on its content. The number of categories ranges from 55 (Dr. Web) up to 451 (VirusTotal), and they include such classes as social networks, banking, ads, government and etc.

The domain-name classifier applies one-hot encoding schema to represent categorical data as a fixed length feature vectors.
Specifically, it creates a "zero" feature vector with the number of elements equal to the total number of categories (767-dimensional
feature vectors in our case) and sets "one" in the positions corresponding to the assigned categories, 
which are not necessarily mutually exclusive. The classifier uses numeric fields as is (without additional encoding).
%The classifier also uses VirusTotal domain-related statistics such as the number of malware samples distributed 
%by a particular domain, the number of samples that refer to a domain and the number of malicious URLs belonging to a domain. 
%These numeric values lie in the range from 0 to 100 (they seem to be capped at 100 level). 
The statistic is aggregated across the entire observation period, i.e. since the first time a domain name was submitted to VirusTotal service. 
%After extracting feature vectors from the raw data, we procced with training an xgboost binary classifier~\cite{xgboost} using 10-fold CV and AUC as an objective to address the class imbalance. In the training set each domain that has ever served at least one malware sample in the Wine dataset is labeled as malicious, otherwise it is considered as benign. 
%Domain name classifier achieves 83.80\% AUC and we choose the operating point of 19.03\% FP rate and 95.41\% TP rate.




\textbf{Waterhole.} In the waterhole case study, the LD analyzes system calls executed by a program.
It transforms continuously evolving 390-dimensional time-series of Windows system calls into
a discrete-time sequence of feature-vectors (FVs). 
This is accomplished by chunking the continuous time series into $r-$second
intervals, and representing the system call trace over each interval as a
single $L-$dimensional vector. 
$L$ is typically a low dimension, reduced down from 390 using PCA analysis, to (in
our experiments) $L=10$ and $r = 1$ second.
%We select the operating point of 92.4\% true positive rate and 6\% false positive rate.






\subsection{Neighborhood Instances from Attack-Templates}
\label{subsec:neighborhood_instantiation}
Within each neighborhood time window (NTW), \sysname generates neighborhood instances
based on statically defined attack vectors --
each attack vector is a ``Template'' to generate neighborhoods with.
%The $NTW$ parameter provides the trade-off between the time to detection and required computational resources. Thus, the lower $NTW$ parameter, the faster \sysname catches 
%malware entering the network, i.e. the lower detection time.
The goal of partitioning data into neighborhoods is to create predominantly benign and malicious neighborhoods.
The algorithm runs once per neighborhood time window (NTW).
Hence the partitioning algorithm is radically different across the case studies.
%Conceptually the algorithm partitions data into neighborhoods that are likely 
%to contain higher concentration of either benign or malicious files/machines than on average.
%However, the partitioning step is radically different across our case studies.


\begin{figure}
\removelatexerror
\begin{algorithm}[H] 
 \small
 \DontPrintSemicolon
 \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
 \SetCommentSty{mycommfont}
 \SetKwInOut{Input}{Input}
 \SetKwInOut{Output}{Output}
 \Input{Downloader graphs}
 \Output{Neighborhoods}
 \BlankLine
 \codecomm{Domain name classifier}\;
 \textbf{Let} DNC ($domain$): $domain$ is malicious\;
 \BlankLine
  
\codecomm{execute once per NTW}
 
\While{True}{
 \codecomm{create an empty list of neighborhoods}\;
 $nbds \leftarrow \emptyset$\;
 \BlankLine
 
 \codecomm{identify active domains within the current NTW}\;
 $D$ $\leftarrow$ domains accessed within the current NTW\;
 \codecomm{identify suspicious domains}\;
 $D'$ $\leftarrow$ \{d $\in$ $D$ $\vert$ DNC($d$)\}
 \BlankLine
  
 \ForEach{suspicious domain $d_i \in D'$}{
    \codecomm{identify files accessing the domain $d_i$}\;
	$F$ $\leftarrow$ files accessing the domain $d_i$

    \codecomm{initialize an empty neighborhood}\;
	$nbd$ $\leftarrow$ $\emptyset$
    \BlankLine
 	
	\ForEach{file $f_i \in F$}{	
	    \codecomm{search for transitively downloaded files}\;
		$F_i$ $\leftarrow$ files transitively downloaded by  $f_i$

	    \codecomm{retain suspicious files}\;
	    $F'_i$ $\leftarrow$ \{$file \in F_i$ $\vert$  $\exists d \in file.domains \quad DNC(d)\}$\;
    	$nbd \leftarrow N$ $\bigcup$ $F'_i$
	}
	$nbds \leftarrow nbds$ $\bigcup$ $nbd$\;
 }
}
 
 \caption{Symantec Wine: Neighborhoods from Attack-Vectors}
 \label{symantec_nbd_algo}
\end{algorithm}
 \vspace{-0.2in}
\end{figure}

%\begin{figure}[tbp]
%   \vspace{-0.0in}
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/symantec/downloader_graph.pdf}\par
%%   \caption{Example of a downloader graph.}
%   \vspace{-0.2in}
%\label{fig:downloader_graph}
%\end{figure}
\textbf{Symantec Wine.} The Algorithm~\ref{symantec_nbd_algo} partitions downloaded files into multiple neighborhoods.
It uses the following intuition: 
if a domain is malicious, then the files transitively downloaded from such a domain are likely to be malicious.

%The key idea of the partitioning algorithm (Algorithm~\ref{symantec_nbd_algo}) is to form neighborhoods around suspicious domains following the intuition 
%that if a domain is malicious, then the files transitively downloaded from such a domain are likely to be malicious.

%The algorithm uses a predefined 150-day long neighborhood time window (NTW) because we found in our experiments 
%that malicious domains distributing more than one malware sample have an average lifespan of 156 days (Section~\ref{}).
%Therefore, we consider downloads within a 150-day window to be correlated.

For ease of explanation, we treat the previously introduced domain name classifier as a predicate (line 1).
At each iteration the algorithm starts with identifying a set of suspicious domains within the current NTW (lines 4--5), which is done using the domain name classifier. Then the algorithm uses each suspicious domain as 
a seed to initiate the neighborhood formation process (lines  6 -- 12).
Next, for each suspicious domain it searches for the files within the current NTW that access 
that particular domain (either download other files from it or being downloaded from it) -- the set $F$ (line 7). 
By following downloader graph edges
the algorithm selects files transitively downloaded by the files in the set $F$ (line 10) and filters out
those that do not access any of the suspicious domains (line 11). The files that have not been excluded are
added to the current neighborhood (line 12).

%After mapping each suspicious domain to a set of suspicious files within a neighborhood (lines 6 -- 12), 
%the algorithm aggregates files that are transitively reachable in terms of the downloader graph abstraction 
%from suspicious domains.

Note that the algorithm formation process may generate many small neighborhoods. 
And an estimate of the conditional distribution using such feature vectors (Section~\ref{subsec:neighborhood_feature_extraction}) 
is usually susceptible to high variance, thus neighborhoods containing 
an insufficient number of files may have negative 
impact on the accuracy of the neighborhood classifier (Section~\ref{subsec:neighborhood_feature_extraction}).
To reduce variance and achieve robust classification of neighborhoods, the algorithm merges them such 
that final neighborhoods are greater than some predefined minimum size.
Empirical analysis of the accuracy of the neighborhood
classifier shows that it achieves robust classification of neighborhoods containing more than 1000 files.

In order to maintain neighborhood effect after merging, i.e. to have mostly homogeneous neighborhoods -- either benign or malicious, the merging algorithm ranks neighborhoods in terms of maliciousness, where malicious score is defined
as the relative number of LDs' alerts within a neighborhood. 
After that the algorithm sorts neighborhoods based on their malicious score and
proceeds merging them in a decreasing order of their malicious scores. 
Note that malicious score estimation may be incorrect if we incorrectly estimate the neighborhood size, 
but \sysname tolerates such errors.


\textbf{Waterhole.}
The algorithm (Algorithm~\ref{waterhole_nbd_algo}) to form a neighborhood to detect a waterhole attack significantly differs
from the one used in the Symantec Wine experiment.
It creates a neighborhood from client machines that access a server or a group of servers within a neighborhood
time window.

\begin{figure}
\removelatexerror
\begin{algorithm}[H] 
 \small
 \DontPrintSemicolon
 \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
 \SetCommentSty{mycommfont}
 \SetKwInOut{Input}{Input}
 \SetKwInOut{Output}{Output}
 \Input{Network flow data}
 \Output{Neighborhoods}
 \BlankLine
 \textbf{Let} predicate(A:Client, B:Servers) := $A$ accesses $B$\;
 \BlankLine
  
 \codecomm{execute once per NTW}\;
 
\While{True}{
 \codecomm{create an empty list of neighborhoods}\;
 $nbds \leftarrow \emptyset$\;
 \BlankLine
 
 $V$ := client machines\codecomm{*}\;
 $S$ := accessed servers\codecomm{*}\;
 \BlankLine

 \codecomm{partitioning a set into non-disjoint sets to incorporate}\;
 \vspace{-.03in}
 \codecomm{structural filtering}\;
  \vspace{-.03in}
 ${P_{1}, P_{2}, ..., P_{N}}$ $\leftarrow$ partition-set($S$), where $S$ = $\bigcup\limits_{i=1}^{N}    P_{i}$\;
 
 \ForEach{partition $P_i$}{
 	\codecomm{form neighborhoods $nbd_i$ using partitions $P_i$}\;
	 $nbd$ $\leftarrow$ $\{V |$ predicate($V$, $P_i$)$\}$\;
	 $nbds \leftarrow nbds$ $\bigcup$ $nbd$\;
 }
 }
 \BlankLine
 \codecomm{*active within the time window NTW}\;
 \caption{Neighborhoods from Attack-Vectors}
 \label{waterhole_nbd_algo}
\end{algorithm}
 \vspace{-0.2in}
%\label{NI_algorithm}
\end{figure}

%The partitioning algorithm (Algorithm~\ref{waterhole_nbd_algo}) executes once per NTW. 
%The best results achieved with \todo{6-second} long
%NTW (see Section~\ref{}).

To abstract away from technical details, we define the predicate (line 1) which is
true if a client $A$ accesses a server $B$.
Each iteration starts with defining the set $V$ of client machines that are active within the current NTW
and the set $S$ of servers that those clients access within the NTW (line 4 -- 5).
Then the algorithm proceeds with partitioning the set $S$
into one or more disjoint subsets $P_i$ (line 6). This is to incorporate
`structural filtering' into the algorithm, allowing an analyst to create
neighborhoods based on subsets of servers (instead of all servers in case of
waterhole).%, which are likely to be attacked. 
Structural filtering boosts detection under certain conditions (see
Appendix~\ref{sec:time-struct}).
The neighborhood instantiation algorithm builds a neighborhood for each partition
$P_i$ (line 8) and, finally, it adds the just formed neighborhoods to $nbds$ list (line 9). 



\subsection{Malware Detection in a Neighborhood}
\label{subsec:neighborhood_feature_extraction}
After having formed neighborhoods, the next logical step is to detect neighborhoods with high malware concentration. 
In order to accomplish this, we introduce \textit{a novel approach to extracting neighborhood features} 
that formalizes shape property.

The \textit{key algorithmic idea} is to map all alert-FVs within a neighborhood to a {\em single}
\textbf{vector-histogram} which robustly captures the neighborhood's statistical
properties. 
\textit{Such transformation allows us to analyze the joint properties of all alert-FVs generated
within a neighborhood without requiring FVs to be clustered or alerts to be
counted.}
After that, \sysname feeds neighborhood-level feature vectors into a binary classifier 
to identify malicious neighborhoods. 
We use two types of binary classifiers: boosted decision trees in the Symantec Wine case study 
and a Wasserstein distance-based threshold test in the waterhole experiment.


%The novelty of our approach lies in the  mapping alert-FVs from a neighborhood into a
%{\em single} vector-histogram and using it as an input to a binary classifier.
%Such transformation allows us to analyze the \textit{joint} properties of all alert-FVs generated
%within a neighborhood without requiring FVs to be clustered or alerts to be
%counted. We describe these steps in further detail.

%The goal of neighborhood processing is to detect neighborhoods with a high malware concentration
%(Algorithm~\ref{ShapeGD_algorithm}). The algorithm detects malware {\em per neighborhood}
%instead of individual nodes. 
%The input to the algorithm is a set of neighborhoods, each of them contains a set of 
%alert-FVs (different types of FVs in each case study).
%and its output is a global alert for the neighborhood.
%We now describe how the algorithm distinguishes 
%between {\em conditional distributions} of alert-FVs from true-positive and
%false positive neighborhoods.

%The threshold test, which acts as an anomaly detector, requires only benign data
%for training and it detects infected neighborhoods as anomalies.
%Even though the threshold test achieves high accuracy in the waterhole study,
%it is unable to approximate a complex classification function.
%As a result, we use a more flexible XGBoost algorithm 
%in the Symantec Wine experiment.

%As mentioned above, we use two different binary classifier -- an xgboost algorithm in 
%the Symantec Wine experiment and
%the simple threshold test for the waterhole experiment.
%The advantage of using xgboost is that it is able to approximate 
%a complex classification function, while the threshold test acts 
%as an anomaly detector, i.e. it separates abnormal looking
%neighborhood shapes from FP shapes.

%To train the threshold-based classifier 
%we only need a benign vector-histogram (built offline during training),
%which is constructed from a set of false
%positive alert-FVs -- thus, it captures the statistical shape of
%misclassifications (FPs) by the LDs but at a neighborhood scale.

% The classifier implicitly compares 
%this vector-histogram to a reference
%vector-histogram (built offline during training).
%The reference vector-histogram is constructed from a set of false
%positive alert-FVs -- thus, it captures the statistical shape of
%misclassifications (FPs) by the LDs but at a neighborhood scale. 





\noindent {\bf Generating a vector-histogram from alert-FVs.} 
The algorithm aggregates
$L$-dimensional projections of alert-FVs on per neighborhood basis into a set
$B$ (Algorithm \ref{ShapeGD_algorithm}, line 3).
%The algorithm processes each neighborhood separately: it aggregates alert-FVs
%on per neighborhood basis and projects them on an $L$-dimensional PCA basis to
%reduce dimensionality (Algorithm \ref{ShapeGD_algorithm}, lines 3--4).  Thus,
%the set $\mathcal{H}_{PCA}$ contains $L$-dimensional alert-FV vectors.
After that, \sysname converts low dimensional representation of alert-FVs, the
set $B$, into a single $(L, b)$-dimensional vector-histogram denoted by $H_B$
(line 4).  The conversion is performed by binning and normalizing $L$-dimensional vectors
within the set $B$ along each dimension.
%In each of the L-dimensions, the L-dimensions
%scalar-histogram of the corresponding component of the vectors is binned and
%normalized.  
Effectively, a vector-histogram is a matrix $L$x$b$, where $L$ is
the dimensionality of alert-FVs and $b$ is the number of bins per dimension. 


In the Symantec Wine case study, \sysname deals with two types of alert-FVs: file and domain alert-FVs.
Thus, it builds two separate vector histograms per neighborhood and then concatenates them into a single vector histogram.
The file-level vector histogram has dimensionality of 10x50, i.e. each file alert-FV is projected on 10-dimensional
basis and binned into 50 bins along each dimension.
Similarly, domain vector-histogram has dimensionality of 100x5, i.e. each domain alert-FV is projected on 100-dimensional
basis and binned into 5 bins along each dimension.
Then, the algorithm concatenates two matrix-shaped vector-histograms. To do that, it represents them 
as two 500 dimensional vectors by using a row-major order and appends the second one to the first one, 
thus, the resulting vector has 1000 dimensions.

And in the waterhole experiment, \sysname bins 10 dimensional file-level alert-FVs into 50 bins, 
thus a vector-histogram has dimensionality of 10x50.
%and \sysname uses a specially designed ShapeScore function to detect malicious activity.

%Because \sysname aggregates two types of alert-FVs: file-level and domain-level alert-FVs, 
%it builds two vector histograms -- one out of file alert-FVs and the other one out of 
%domain alert-FVs -- and after that it concatenates them into a single vector histogram.
%The file-level vector histogram has dimensionality of 10x50, i.e. each file alert-FV is projected on 10-dimensional
%basis and binned into 50 bins along each dimension.
%Similarly, domain vector-histogram has dimensionality of 100x5, i.e. each domain alert-FV is projected on 100-dimensional
%basis and binned into 5 bins along each dimension.

%Next, the algorithm concatenates two matrix-shaped vector-histograms. To do that, it represents them 
%as two 500 dimensional vectors by using a row-major order and appends the second one to the first one, 
%thus, the resulting vector has 1000 dimensions.

We use standard methods to determine the size and number of bins. % and note that
%the choice of Wasserstein distance in the next step makes \sysname robust
%against variations due to binning.  
In particular, we tried square-root choice,
Rice rule, and Doane's formula~\cite{binning} to estimate the number of bins,
and we found that 20--100 bins yielded separable histograms (as in Figure
\ref{fig:windows-hist}).% for the Windows dataset and fixed it at 50 for our
%experiments. 

%As mentioned above, we use two different binary classifier -- an xgboost algorithm in 
%the Symantec Wine experiment and
%the simple threshold test for the waterhole experiment.
%The advantage of using xgboost is that it is able to approximate 
%a complex classification function, while the threshold test acts 
%as an anomaly detector, i.e. it separates abnormal looking
%neighborhood shapes from FP shapes.

%\mikhail{Skip it ???
%Both classifier estimate how much a current vector-histogram, $H_B$, differs from 
%a {\em reference histogram}, $H_{{\rm ref}}$,
%which is generated during the training phase
%using only the false positive FVs of the LDs.  
%We run LDs on the VirusTotal reports and system-call
%traces generated by benign apps respectively -- the FVs corresponding to the alerts from the
%LD (i.e., the false positives) are then used to construct the reference
%histogram $H_{{\rm ref}}.$
%}

%To collect known benign traces, a straightforward approach is to
%use test inputs on benign apps or use record-and-replay tools to re-run
%real user inputs in a malware-free system.  Or, like any anomaly detector, an
%enterprise can train \sysname using applications deployed currently and recompute
%$H_{ref}$ periodically. 


%\textbf{Symantec Wine.}
%In comparison to the waterhole case study, we use a more powerful classifier -- XGBoost -- 
%and enhance the way of representing a neighborhood as a vector histogram.
%Because \sysname aggregates two types of alert-FVs: file-level and domain-level alert-FVs, 
%it builds two vector histograms -- one out of file alert-FVs and the other one out of 
%domain alert-FVs -- and after that it concatenates them into a single vector histogram.
%The file-level vector histogram has dimensionality of 10x50, i.e. each file alert-FV is projected on 10-dimensional
%basis and binned into 50 bins along each dimension.
%Similarly, domain vector-histogram has dimensionality of 100x5, i.e. each domain alert-FV is projected on 100-dimensional
%basis and binned into 5 bins along each dimension.
%
%Next, the algorithm concatenates two matrix-shaped vector-histograms. To do that, it represents them 
%as two 500 dimensional vectors by using a row-major order and appends the second one to the first one, 
%thus, the resulting vector has 1000 dimensions.

\textbf{Binary classifier.}
Originally, \sysname was designed to serve as an anomaly detector, therefore it used Wasserstein distance-based threshold test 
(Appendix~\ref{sec:shape-score-function}) to detect malicious neighborhoods. And this approach works reliably 
in the waterhole case study. 
However, we found that the threshold test does not achieve high accuracy in the Symantec Wine case study, and 
we replaced it with a a binary classifier based on boosted decision trees (XGBoost).
In either case a classifier accepts a neighborhood-level feature vector as input and make a prediction whether a neighborhood 
is malicious or benign.

To train the binary classifier in the Symantec Wine experiment, we can use plenty of benign and malicious files
together with the neighborhood instantiation algorithm (Section~\ref{subsec:neighborhood_instantiation}) to
generate benign/malicious neighborhoods given ground truth file-level data.
In comparison to the binary classifier, training the threshold test 
in the waterhole case study requires only benign data, which can be collected
using test inputs on benign apps or using record-and-replay tools to re-run
real user inputs in a malware-free system.  

Note like any machine learning detector, \sysname needs to be retrained periodically
to account for constantly evolving statistical software properties, which can
negatively impact false positive/negative rate.


%And finally the binary classifier -- xgboost~\cite{xgboost} -- estimates probability of a neighborhood being malicious, 
%which the algorithm turns into a binary label (either malicious or benign).


%\textbf{Waterhole.}
%In the waterhole experiment, \sysname bins 10 dimensional file-level alert-FVs into 50 bins, 
%thus a vector-histogram has dimensionality of 10x50, 
%and \sysname uses a specially designed ShapeScore function to detect malicious activity.

%%\noindent {\bf ShapeScore.} 
%For completeness, we describe here the Wasserstein-based distance -- \textit{ShapeScore} function -- that we developed to
%detect malicious neighborhoods in the waterhole case study.
%\sysname computes the ShapeScore by comparing this histogram, $H_B$, to a {\em reference
%histogram}, $H_{{\rm ref}}$.  ShapeScore is thus the distance of a neighborhood
%from a benign reference histogram -- a high score indicates potential malware.
%
%The ShapeScore of the accumulated set of FVs, $B$,
%is given by the sum of the coordinate-wise Wasserstein distances
%\cite{vallender1974calculation} between 
%$$H_B =
%(H_{B}(1) \ H_{B}(2) \ \ldots \ H_{B}(L))$$ 
%and 
%%$$\mathcal{H}_{{\rm ref}} =
%%(\mathcal{H}_{{\rm ref}}(1) \ \mathcal{H}_{{\rm ref}}(2) \ \ldots \
%%\mathcal{H}_{{\rm ref}}(L)).$$ 
%$$H_{{\rm ref}} = (H_{{\rm ref}}(1) \ H_{{\rm ref}}(2) \ \ldots \
%H_{{\rm ref}}(L)).$$ 
%In other words,
%%$$
%%{\rm ShapeScore} = \sum_{l=1}^L d_W(\mathcal{H}_{\mathcal{B}}(l),\mathcal{H}_{{\rm ref}}(l)),
%%$$
%$$
%{\rm ShapeScore} = \sum_{l=1}^L d_W(H_{B}(l),H_{{\rm ref}}(l)),
%$$
%where for two scalar distributions $p, q,$ the Wasserstein distance
%\cite{vallender1974calculation,wasser-wiki} is given by
%$$
%d_W(p, q) = \sum_{i=1}^b \left |\sum_{j=1}^i \left(p(j) - q(j) \right) \right |.
%$$
%
%This Wasserstein distance serves as an efficiently computable one dimensional
%projection, that gives us a discriminatively powerful metric of distance
%\cite{vallender1974calculation,benbre00}. Because the Wasserstein distance
%computes a metric between distributions -- for us, histograms normalized to
%have total area equal to 1 -- it is invariant to the number of samples that
%make up each histogram. Thus, unlike count-based algorithms, {\em it is robust
%to estimation errors in community size}. Figure~\ref{fig:windows-hist} verifies
%this intuition, and shows that true positives and false positive feature
%vectors separate well when viewed through the ShapeScore. 
%
%Finally, to determine whether a neighborhood has malware present \sysname performs
%hypothesis testing. If ShapeScore is greater than a threshold $\gamma$, \sysname
%declares a global alert, i.e., the algorithm predicts that there is malware in
%the neighborhood.  The robustness threshold $\gamma$ is computed
%via standard confidence interval or cross-validation methods with multiple sets
%of false-positive FVs (see Section \ref{sec:power-shape}).







\begin{figure}
\removelatexerror
\begin{algorithm}[H]
\small
 \DontPrintSemicolon
 \SetKwInOut{Input}{Input}
 \SetKwInOut{Output}{Output}
 \Input{Suspicious neighborhoods $nbds$}
 \Output{Malicious neighborhoods}

 \For{each nbd in nbds}{
   %// collect alert-FVs from the nodes in the neighborhood\;
   \codecomm{aggregate L-dim projections of alert-FVs on per neighborhood basis}\;
%   $\mathcal{B}$ 
  $B$ $\leftarrow$ $\{alert-FVs$  $|$ $alert-FV$ $\subset$ $nbd\}$\;
   %\BlankLine

   %// reduce dimensionality\;
%   $\mathcal{B}_{PCA}$ $\leftarrow$ project $\mathcal{B}_{FVs}$ on $L$-dim PCA basis\;
   %\BlankLine

   %// perform binning with \textit{b} bins along each dimension\;
   \codecomm{build an $(L, b)$-dim. vector-histogram}\;
%   $\mathcal{H}_{\mathcal{B}}$ 
   $H_B \leftarrow$ bin \& normalize $B$ along each dimension\;
	
   \codecomm{classify the neighborhood}\;
   \If{Binary Classifier($nbd$)} {
     label $nbd$ as \textit{malicious}\;
   }
 }
 \caption{Neighborhood Classification}
 \label{ShapeGD_algorithm}
\end{algorithm}
 \vspace{-0.2in}
%\label{ShapeGD_algorithm}
\end{figure}


==> algorithm_symantec.tex <==


We adapt local detectors from the prior work~\cite{vt_report_classification} because they can efficiently scale up to processing a large number of files. Such LDs primarily rely on a lightweight file analysis. 
Specifically, an LD extracts syntactic features from a file and applies a binary classification algorithm 
that labels a file as either malicious or benign.

First, an LD runs existing commercial tools such as TRID, ClamAV, Symantec on a binary file, analyzes statically imported libraries and functions, detects common packers, checks whether a file is digitally signed or not, and collects its binary metadata. The output of all these analyses is aggregated into a single report.
Rather than actually running all these tools, we query an online VT service to download reports 
for the files in the WINE dataset. 
The benign files lacking corresponding VT reports are assigned VT reports of other benign files at random.

Second, an LD extracts features from VT reports using a state-of-the-art feature extraction 
algorithm~\cite{vt_report_classification}, which outputs very high-dimensional feature
vectors. Such feature vectors have limited usability due to "curse of dimensionality" 
and due to memory overhead, which often results in program crashes.
To overcome such an issue, we use a common method for dimensionality reduction -- feature hashing~\cite{}. 
Empirically we found that the output dimensionality of 1024 allows us to 
achieve the best trade-off between classifier's performance and resource consumption. 

Finally, an LD uses an xgboost classifier~\cite{xgboost}, which is pretrained using 10-fold cross-validation 
and area-under-the-curve (AUC) as classifier's objective to deal with class imbalance. 
%Finally, an LD uses an xgboost classifier~\cite{xgboost}, which is pretrained using 10-fold cross-validation 
%and area-under-the-curve (AUC) as classifier's objective to deal with class imbalance. 
%Following the parameter tuning approach outlined in the Section~\ref{}, we trained an xgboost classifier
%achieving 97.61\% AUC, and we choose the operating point with 5.0\% false positive rate and 90.47\% true positive rate. Due to the high number of benign files in the dataset, 5.0\% false positive rate corresponds to more than 1 million  misclassified files.
%We use out-of-fold predictions made by such classifier throughout the rest experiments.


\textbf{Domain name classifier.}
\label{algo:domain_classifier}
 
\begin{figure}[tbp]
   \vspace{-0.0in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/symantec/domain_name_classifier/domain_features.pdf}\par
   \caption{Domain features.}
   \vspace{-0.2in}
\label{fig:domain_features}
\end{figure}


We build a domain name classifier that analyzes VT domain reports~\ref{fig:domain_features} and identifies domains that are likely to distribute malicious files. The classifier extracts feature vectors from the data provided by commercial tools such as Dr. Web, Websense ThreatSeeker, and VT and from the statistics computed by VT itself~\ref{fig:domain_features}.
Dr. Web, Websense ThreatSeeker and VT categorize each domain based on its content. The number of categories ranges from 55 (Dr. Web) up to 451 (VT), and they include such classes as social networks, banking, ads, government and etc.

The classifier applies one-hot encoding schema to convert domain categories into feature vectors. Specifically, it
creates a "zero" feature vector with the number of elements equal to the total number of categories (767-dimensional
feature vectors in our case) and sets "one" in the positions corresponding to the assigned categories.
The classifier also uses VT domain related statistics such as the number of malware samples distributed 
by a particular domain, the number of samples that refer to a domain and the number of malicious URLs belonging to a domain. The statistic is aggregated across the entire observation period, i.e. since the first time a URL was submitted to VT service. Those numeric values lie in
the range from 0 to 100, and they seem to be capped by VT at 100 level. And the classifier uses numeric fields as is without further conversion.

VT provides domain reports for 301,323 domains out of 353,267.
We could submit missing URLs to the VT service, however, the WINE dataset lacks complete URL, it only provides domain names, therefore we conservatively treat 51,944 missing VT reports as benign. It means that in our experiments \sysname
may demonstrate lower detection rate than if it had access to the missing VT reports.
In practice, the issue of missing domain reports can be addressed by running domain analyzers periodically in order
to have a complete set of domain reports.

After extracting feature vectors from the raw data, we procced with training an xgboost binary classifier~\cite{xgboost} using 10-fold CV and AUC as an objective to deal with the class imbalance. In the training set each domain that has ever served at least one malware sample in the Wine dataset is labeled as malicious, otherwise it's considered as benign. Thus, we deal with 33,886 malicious domains and 267,437 benign domains.

%threshold 0.03 fp 0.505977108627 tp 0.960249070413 alerts 167,856 fp_file 0.164228272619 tp_file 0.98171754106
In our experiments, we use out-of-fold predictions made by the domain name classifier to approximate its behavior in the
deployment scenario. Specifically, in each fold the classifier uses 90\% of the data for training, and it makes a prediction for each domain name within the rest 10\% of the dataset. In the next iteration of 10-fold CV, it detects
suspicious domain names within the another fold -- another group of 10\% domain names.



%-- running experiments: NBD time window
%\textbf{Experiment parameters.}
%We use a neighborhood time window of 150 days and run a detector algorithm every 30 days.

\textbf{Online detection algorithm.}

\begin{figure}
\removelatexerror
\begin{algorithm}[H] 
 \small
 \DontPrintSemicolon
 \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
 \SetCommentSty{mycommfont}
 \SetKwInOut{Input}{Input}
 \SetKwInOut{Output}{Output}
 \Input{Downloader graphs}
 \Output{$Malicious$ files}
 \BlankLine
 \textbf{Let} DNC ($domain$): $domain$ is malicious\;
 \textbf{Let} NC ($neighborhood$): $neighborhood$ is malicious\;
 \textbf{Let} LD ($file$): $file$ is malicious\;
 \BlankLine
  
\While{True}{
 \codecomm{[\textit{time-NTW, time}] \textit{defines the current time window}}\;
 $time \leftarrow$ $current$ $time$
 \BlankLine

 \codecomm{1. Create Neighborhoods}\; 
 \codecomm{create an empty list of neighborhoods}\;
 $nbds \leftarrow \emptyset$\;
 \BlankLine
 
 \codecomm{identify active domains within the current NTW}\;
 $D$ $\leftarrow$ domains accessed within the current NTW\;
 \codecomm{identify suspicious domains}\;
 $D'$ $\leftarrow$ \{d $\in$ $D$ s.t. DNC($d$)\}
 \BlankLine
  
 \ForEach{suspicious domain $d_i \in D'$}{
    \codecomm{identify files accessing the domain $d_i$}\;
	$F$ $\leftarrow$ files accessing the domain $d_i$

    \codecomm{initialize an empty neighborhood}\;
	$N$ $\leftarrow$ $\emptyset$
    \BlankLine
 	
	\ForEach{file $f_i \in F$}{	
	    \codecomm{search for transitively downloaded files}\;
		$F_i$ $\leftarrow$ files transitively downloaded by  $f_i$

	    \codecomm{filter out likely benign files}\;
	    $F'_i$ $\leftarrow$ \{$file \in F_i$ $\vert$  $\exists d \in file.domains \rightarrow DNC(d)\}$\;
    	$N \leftarrow N$ $\bigcup$ $F'_i$
	}
	$nbds \leftarrow nbds$ $\bigcup$ $N$\;
 }
 \BlankLine
     
 \codecomm{2. Merge Neighborhoods}\;
 \codecomm{compute relative number of alerts within neighborhoods}\;
  $(n, score) \leftarrow (n, |$\{$file \in n |$ LD($file$)\}$\vert/|n|$)\;
 \codecomm{sort neighborhoods in descending order of their scores}\;  
 \BlankLine
     
 \codecomm{create an empty list of neighborhoods}\;
 $nbds' \leftarrow \emptyset$\;
 $n \leftarrow \emptyset$\;
 
  \ForEach{neighborhood $n_i \in nbds'$}{
	$n \leftarrow n \bigcup n_i$\;
  \BlankLine
 	
	\If{$|n| > minimum$ $neighborhood$ $size$}{
	    \codecomm{add a neighborhood to the neighborhood list}\;
		 $nbds' \leftarrow nbds'$ $\bigcup n$ \;
		 $n \leftarrow \emptyset$\;
	}
  }
  \BlankLine
  
  $nbds''$ $\leftarrow$ \{$n \in nbds' |$ NC($n$)\}\;
  $F'$ $\leftarrow$ \{$file \in n |$ $n \in nbds''$\}\;
  \codecomm{output malicious files for deeper analysis}\;
  $malicious files$ $\leftarrow$ \{$file \in F' |$ LD($file$)\}\;
    
  \codecomm{sleep for the time interval $delay$}\;
 }
 
 \caption{Online detection algorithm}
 \label{online_detection_algo}
\end{algorithm}
 \vspace{-0.2in}
\end{figure}

\begin{figure}[tbp]
   \vspace{-0.0in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/symantec/downloader_graph.pdf}\par
   \caption{Example of a downloader graph.}
   \vspace{-0.2in}
\label{fig:downloader_graph}
\end{figure}

\textbf{Example.}
We start this subsection with an example of how the detection algorithm actually operates.
For such purpose, we illustrate it using an example of a downloader graph on the Figure~\ref{fig:downloader_graph}.
The two colors -- blue and red -- represent benign and malicious entities (ground truth) -- both files and domains.

Let's assume the domain name classifier truly identifies globaldl.net as a malicious domain (a domain prone to distributing malware),
then the algorithm starts forming a neighborhood with respect to globaldl.net domain name. First, \sysname searches for the files directly accessing or being downloaded from
globaldl.net domain -- chrome.exe and antivirus.exe respectively. 
However, chrome.exe is white-listed based on its digital signature (Section~\ref{}).
Thus, \sysname starts aggregating all the files that antivirus.exe transitively downloads F, G, H, I, i.e. the files  setupnew.exe, netids.dll, webguard.exe, and rexpert.exe. It keeps only the files that have at least one of their edges 
-- incoming or outgoing -- predicted as malicious. 
We can think that the algorithm originally includes in a neighborhood all the nodes transitively reached from antivirus.exe including antivirus.exe itself, i.e. the nodes E,F,G,H,I. Then it traverses the nodes in the neighborhood
once again and removes the nodes whose edges are predicted to be benign by the domain name classifier.

For example, if the algorithm correctly predicts that gravic.com is a benign domain and mistakenly predicts that dtsusuk.org is also benign, then it prunes the node H (webguard.exe). However, if the algorithm correctly predicts 
dtsusuk.org label (malicious domain), then it keeps the node H in the neighborhood.
In practice the algorithm makes two type of errors: it either includes
benign nodes into a neighborhood or removes malicious ones. We adjust algorithm's parameters to make it conservative, i.e. to retain as many malicious nodes within a neighborhood as possible while avoiding inclusion of benign nodes.


\textbf{Algorithm.}
Now we proceed formally describing the detection algorithm. After introducing the high-level concept, we focus on its  core part -- neighborhood level classification.

Our system periodically executes the online detection algorithm~\cite{online_detection_algo} within a loop.
The algorithm runs every $delay$ hours, and we assume that $delay$ hours are enough for 
executing a single iteration of the algorithm. The $delay$ parameter provides the trade-off between the time to detection and required computational resources. Thus, the lower $delay$ parameter, the faster \sysname catches 
malware entering the network, i.e. the lower detection time.

Conceptually the algorithm comprises two logical parts -- partitioning data into neighborhoods that are likely 
to contain higher concentration of either malicious or benign files than on average (lines 4 -- 23) and detecting infected neighborhoods (lines 24 -- 26).
For the ease of explanation we treat previously described machine learning classifiers as logical predicates 
(lines 1 -- 3), whose output is a single boolean value -- true corresponds to raising an alert, and false signifies a no-alert situation. We use such predicates to concisely delineate data partitioning process.

Each iteration of the algorithm operates on the data within the neighborhood time window (NTW), 
which has a predefined length of 150 days in our experiments. 
In our experiments we found that malicious domains distributing more than one malware sample have an average lifespan of 156 days~\ref{}.

The algorithm forms neighborhoods around suspicious domains following the intuition that if a domain is truly malicious 
than it is likely that the large number of files transitively downloaded from such a domain is malicious.
The lines 7 -- 8 define the set of suspicious domains within the current time window, and each such domain is used as 
a seed to initialize neighborhood formation process (lines 9-- 15).

While partitioning the data into a set of neighborhoods, the algorithm iterates over the set of suspicious domains (line 9),
maps each such domain to the files that either access the domain or being downloaded from the domain. 
These two cases correspond to the source and target nodes associated with a domain edge.
We intentionally consider both cases. Though the former case logically follows from malware distribution process, 
the latter is an artifact of whitelisting browser executables, which may leave malicious files downloaded by users using 
benign browsers. After whitelisting, there may be left incoming edges in the downloader graphs leading to maliciious files.

After mapping each suspicious domain to a set of files that access it or being downloaded from it, 
the algorithm aggregates files that are transitively reachable in terms of the downloader graph abstraction 
from those file seeds or, in other words, the files that are transitively downloaded by file seeds (lines 15 -- 16).

The algorithm formation process may generate many small neighborhoods. And the feature vectors extracted from such
neighborhoods are usually susceptible to high variance may have negative impact on 
the accuracy of the neighborhood classifier (Section~\ref{}).
To reduce variance and achieve robust classification of neighborhoods, we merge them such that the final neighborhood
has at least a predefined minimum number of files. Empirical analysis of the accuracy of the neighborhood
classifier shows that it achieves robust classification on neighborhoods containing more than 1000 files.
Thus, we adjust the neighborhood merging algorithm such that it outputs neighborhoods with at least 100 files.

In order to maintain neighborhood effect after merging, i.e. to have mostly homogeneous neighborhoods -- either benign or malicious, the merging algorithm ranks neighborhoods in terms of maliciousness, where malicious score is defined
as the relative number of Local Detector's alerts within a neighborhood. 
After that the algorithm performs sorting neighborhoods based on their malicious score (line 17) and
proceeds merging them in a decreasing order of their malicious scores (lines 20 -- 24). 
%It merges neighborhoods together such that the total number of files within them is above the minimum threshold.

%When merging the neighborhoods, the algorithm prioritizes merging highly infected neighborhoods. 
%To estimate the infection rate within a neighborhood, the algorithm counts the relative number of 
%Local Detector's alerts within a neighborhood, and then it sorts all the neighborhoods based on those parameters.
%Therefore, the algorithm first starts merging highly infected neighborhoods and than it continues merging together
%less contaminated neighborhoods (lines 20 -- 24). It groups N neighborhoods together such that the total number of files
%within them is higher the minimum threshold.

The next step after merging neighborhoods is to detect the neighborhoods with high concentration of malicious files (line 25). To do that, the neighborhood classifier extract neighborhood level features and uses a machine learning classifier to identify highly contaminated neighborhoods (Section~\ref{}). 
The goal of this process is to filter out neighborhoods that are likely to contain less than 5\% of malicious files. 
We intentionally set the threshold to 5\% because lower value of this parameter would result in selecting not only 
highly infected neighborhoods, but also predominantly benign neighborhoods. And the latter would significantly
reduce the neighborhood effect.Finally, \sysname aggregates files across all neighborhoods labeled as malicious and performs deep file inspection (line 26). 

The key aspect of the entire data processing pipeline is to increase malware concentration within the suspicious file set in comparison to the random file-level sampling. Thus, computationally intensive deep file
analysis deals with fewer files than the total number of files in the system and thus produces the fewer absolute number of false positives.
An example of the deep file introspection could be dynamic behavioral analysis within
virtual machines~\cite{}. However, due to the lack of the original executable files and due to the fact that VT
does not have dynamic behavioral reports for the most of the files in the Wine dataset, we employ Local Detectors
on top of suspicious neighborhoods. Therefore, we propose to analyze LDs' alerts raised only within suspicious neighborhoods (line 27) and compare the results against Local Detectors running on the data set
without neighborhood level preprocessing and with previously presented approach~\cite{downloader_graphs}.



\textbf{Neighborhood classification algorithm.}

\begin{figure}
\removelatexerror
\begin{algorithm}[H] 
 \small
 \DontPrintSemicolon
 \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
 \SetCommentSty{mycommfont}
 \SetKwInOut{Input}{Input}
 \SetKwInOut{Output}{Output}
 \Input{Neighborhood nbd}
 \Output{Is neighborhood malicious}

 \textbf{Let} FFE($file$) := $file$'s feature vector\;
 \textbf{Let} LD($file$): $file$ is malicious\;
 \textbf{Let} DFE($domain$) := $domain$'s feature vector\;
 \textbf{Let} DNC($domain$): $domain$ is malicious\;
 \BlankLine

 \codecomm{aggregate L-dim projections of file-alert FVs on per neighborhood basis}\; 
 $FVs_{File}$ $\leftarrow$ \{$FFE(file) \in nbd |$ LD($file$) \}\;
 $file_H$ $\leftarrow$ bin \& normalize $FVs_{File}$\;
 \BlankLine
 
 \codecomm{aggregate K-dim projections of alert-domain FVs on per neighborhood basis}\;  
 $FVs_{Domain}$ $\leftarrow$ \{$DFE (domain) \in nbd |$ DNC($domain$) \}\;
 $domain_H$ $\leftarrow$ bin \& normalize $FVs_{Domain}$\;
 \BlankLine

 \codecomm{Concatenate file- and domain-histograms}\; 
 $H$ $\leftarrow$ $file_H || domain_H$\;
 $output$ $\leftarrow$ Binary Classifier($H$) $> threshold$\;
 
 \caption{Neighborhood classifier}
 \label{algo:nbd_algorithm}
\end{algorithm}
 \vspace{-0.2in}
\end{figure}

\mikhail{copy paste from the original paper??}
The neighborhood classification algorithm lies at the heart of the entire malware detection framework.
It analyzes both files and domains within a neighborhood. From high-level point of view, it performs two 
identical steps for each neighborhood: it aggregates file FVs leading to LDs' alerts into a file vector-histogram (line 5) and
it aggregates domain FVs leading to LDs' alerts into a domain vector-histogram (line 7). After that it bins each histogram 
independently (lines 6 and 8).

The $file_H$ has dimensionality of 10x50 (line 6), i.e. each file-alert FV is projected on 10-dimensional
basis and binned into 50 bins along each dimension.
Similarly, $domain_H$ has dimensionality of 100x5 (line 8), i.e. each domain-alert FV is projected on 100-dimensional
basis and binned into 5 bins along each dimension. \mikhail{retains N \% variance}

Next, the algorithm concatenates two matrix-shaped histograms. To do that, it represents them 
as two 500 dimensional FVs by using a row-major order and appends the second one to the first one, 
thus, the resulting FV has 1000 dimensions.

And finally a binary classifier (xgboost algorithm in our case) estimates probability of a neighborhood being malicious (line 10),
which the algorithm turns into a binary label (either malicious or benign) if it exceeds a threshold.

%It also performs similar action on domains -- it aggregates domain FVs leading to domain name classifier alerts within
%a neighborhood into a domain vector-histogram. After that, it concatenates both histograms and applies
%a binary classifier (xgboost algorithm in our case), which outputs the probability of a domain being suspicious.
%
%It aggregates file-level alert-FVs across all the files within a neighborhood and domain-level alert-FVs across
%all domains accessed within the neighborhood, bins and normalizes them separately. After that it concatenates two
%vector histograms.
%\mikhail{explain the algorithm in more details}



%We define neighborhoods using a slightly modified watering hole template. Specifically, a neighborhood is 
%a collection of files transitively downloaded from a suspicious domain within a neighborhood time window.
%As in the case of the watering hole attack, the intuition behind such a neighborhood definition is
%that if a process contacts a suspicious domain, it is likely to download malicious files and it's likely that
%the original file is malicious also. By traversing downloader graphs, we recursively apply such intuition to
%other files.
%
%Technically the algorithm performs the following steps (Figure~\ref{downloader_graph}).
%For each domain name the domain classifier outputs the probability of being malicious. If a domain is considered
%malicious (globaldl.net), we start forming a neighborhood by identifying all files that access that domain within a NTW (chrome.exe on the figure) and
%for each of them we perform a breadth-first search on the downloader graph.
%While traversing downloader graphs in the BFS manner, we use domain name predictions of our domain name
%classifier to discard files downloaded from likely benign domains (gravic.com).
%Had the domain name classifier correctly identified all suspicious domains, then the neighborhood would include the following malicious files -- E, F, G, I. However, due to high false positive rate of the classifier, 
%neighborhoods contain only 30\% malicious files.
%%At the end of this step, a neighborhood includes files transitively
%reachable from a suspicious domain.





1. Local Detectors

2. Neighborhood (nbd) algorithm

3. NBD-level feature extraction

4. Detecting suspicious NBDs


==> deployment.tex <==

%\noindent \textbf{Implementation.} Shape GD is an enterprise-level malware
%detector.  Currently, enterprises use SIEM tools (like HP Arcsight and Splunk)
%to monitor network traffic and system/application logs, malware analysis
%sandboxes that scan emails for malicious links and attachments, in addition to
%host-based malware detectors (LDs) from Symantec, McAfee, Lookout, etc. We use
%exactly these side-information -- from network logs (client-IP, server IP,
%timestamp) and email monitoring tools -- to construct neighborhoods and filter
%alert-FVs using LDs (Algorithm \ref{NI_algorithm}).
%
%%Here we describe a deployment scenario for early detection of waterhole and
%%phishing attacks. In these scenarios, Shape GD needs to monitor the
%%outgoing connections and email communication within an enterprise. We
%%suggest implementing Shape GD as an addition to a network firewall and
%%allowing it to collect necessary information from an email server.
%%Such information is sufficient to dynamically instantiate
%%neighborhoods 
%
%%Observing outbound network connections and monitoring email activity
%%within a corporate network are enough to be able dynamically form
%%neighborhoods (Algorithm \ref{NI_algorithm}). Shape GD can store
%%membership information for each active node over a neighborhood time
%%window (NTW) and discard it shortly after a current NTW expires.
%
%Upon receiving alert-FVs, Shape GD runs its malware detection algorithm
%(Algorithm \ref{ShapeGD_algorithm}) for all neighborhoods the alert-FVs belong
%to. If a particular neighborhood is suspicious, then Shape GD will notify a
%downstream analysis (deeper static/dynamic analyses or human analysts) and
%forward relevant information in the incident report. 


%\noindent \textbf{Computing Shape GD's parameters.} 
%>> How to choose parameters such as histogram+PCA, neighborhood time window
%(NTW), size of neighborhoods in feature vectors (FVs), ShapeScore threshold,
%etc. in a real deployment?
Here we elaborate on the steps that should be taken in a real world environment
to choose parameters. The steps discussed here are generic and are applicable
to other attacks beyond waterhole and phishing -- the following results section
quantifies each of these steps.
%In the rest of the paper, we show only the final detection results for
%brevity.

First, an analyst should start with designing an appropriate algorithm
to run on local detectors (LDs).% (Appendix \ref{sec:LDs}). 
To achieve
this, an analyst needs to compare the performance of multiple feature
extraction (FE) algorithms combined with a diverse set of machine
learning classifiers. One way to choose the best pair of a FE
algorithm and a classifier is to build ROC curves for each pair, and
select the pair that meets the desired detection rate to 
computation/training effort for the LD.

%false positive and true positive rates from the LD.

% Second, an analyst needs to obtain an independent set of labeled data
% to evaluate Shape GD's ability to distinguish between false positives
% and true positives (Section \ref{sec:power-shape}). 

Second, the analyst needs to determine 
whether even a purely malicious neighborhood can be separated from
benign ones, and 
the minimum number of
FVs per neighborhood to do so (Sections~\ref{sec:power-shape}.% and
%Appendix~\ref{sec:nbd-size}). 
This
number depends on the false positive rate of LDs ( e.g., in our
experiments, we determined that a neighborhood should generate at
least 15K FVs).%, see Figure \ref{fig:windows-hist-stability}).

Third, we need to choose an NTW based on the false positive rate (FP)
and the desired time-to-detection (Section~\ref{sec:time-nf}. 
A small NTW means more frequent
transfers of FVs from LD to GD, whereas a long NTW means that more
nodes can get compromised before the GD makes a decision and/or FPs
can drown out TPs. Similarly, structural filtering can improve 
detection rate if the true positive alert-FVs are not deluged
by the rate of false-positive alert-FVs -- Section~\ref{sec:time-struct}
quantifies how this trade-off differs for waterhole and phishing.


% \textbf{Third, to choose an appropriate NTW window, the following two factors
% need to be taken into consideration: an average number of nodes in a
% dynamic neighborhood, and side information about an attack. 
% The former determines the minimum NTW size as the ratio of a minimum
% number of FVs generated within a neighborhood (this number has been
% estimated in the previous step) and the average number of nodes.

% Side information about an attack provides an insight whether an
% analyst should minimize the size of an NTW or maximize it. For
% example, due to uncertainty of user behavior in a phishing attack,
% i.e. it is not known whether a potential victim will ever open a
% malicious attachment and if yes, when this happens, it is better to
% use large NTWs in order not to miss actual exploitation of user
% machines (Section \ref{sec:time-nf}).

% On the contrary, side information about a waterhole attack says that
% if a machine could get infected due to vising a compromised website,
% this happens right after visiting it, and there is no human factor
% involved in exploiting a physical machine. Therefore, an analyst needs
% to minimize an NTW (Section \ref{sec:time-nf}) and stick to the
% minimum NTW size, which is the minimum number of FVs generated within
% a neighborhood divided by the average number of nodes.}

% Finally, an analyst may experiment with adding structural filtering.
% Effects of structural information depend on attack against which an
% analyst protects a corporate network and on a concrete setting such as
% the number of observed nodes, available computation resources to Shape
% GD and etc (Section \ref{sec:time-struct}).

%\noindent \textbf{Reference histogram.} 
%%As explained in the Section
%%\ref{sec:model}, a reference histogram lies at the heart of Shape GD.  To
%To construct reference histograms, we need to obtain the LD's false positive vectors (FPs).
%This requires running benign applications similar to any anomaly detector.
%%% Ideally we need to run an LD in an uninfected system and collect FPs.
%%% however, this may be hard or even impossible. 
%A straightforward approach is to collect FPs in a lab environment using test
%inputs on benign apps or using record-and-replay
%tools to re-run real user inputs in a malware-free system. 
%Or, an enterprise can 
%train using applications deployed currently and recompute $H_{ref}$ periodically -- 
%this is similar to anomaly detectors where the goal is to detect
%anomalous behaviors as (potentially) malicious.


%The reference
%histogram may be affected by new types of installed benign software, thus it

%needs to be recomputed periodically similar to any anomaly detection system
%(spam-detection, etc 

%which is not a problem because enterprises
%usually have an internal repository of approved for installation software
%products, and such centralized management of available software products makes
%it easy to keep track of software updates and to update the reference histogram
%periodically.  }

% The other way of collecting
% FPs is to run LDs in a production system and treat generated alert-FVs
% as FPs. This will require to leverage achievements in the field of
% robust machine learning because alert-FVs may include TPs. However,
% their portion is expected to be tiny because only a small portion of
% machines is usually compromised (if any). In this paper we assume that
% a reference histogram is learned in a lab environment.




%and learn a reference histogram while admitting tiny portion of TPs intermixed with FPs. Such method would work because only a small portion of machines is usually compromised (if any).
%However, in this paper we assume that a reference histogram is learned in a lab environment.

%We follow these steps; analogous steps would be followed 
%in a real deployment. In the paper, we only show final detection 
%results for one representative set of LD techniques for brevity.

%-- start with a feature extraction and LD algorithm. Output: FVs 
%that lead to a local alert. (Fig. 3 shows example LDs).

%-- determine minimum number of FVs required to model 
%neighborhoods in benign programs. This is determined using 
%only benign past (e.g., test)  data -- see Fig. 5; requires about 
%15K FVs from our experiments.

%--  choose an NTW based on the false positive rate (FP) and the 
%desired time-to-detection.
%Figs 8, 9 show this trade-off for phishing and waterhole attacks 
%respectively. Small NTW means more work to transfer FVs from LD to
% GD, whereas long NTW means that more nodes can get compromised 
%before GD makes a decision or FPs can drown out TPs. 
%
%We have experimented with several choices of feature extraction 
%and LD algorithms (Fig 3), and NTW settings (Fig. 8,9) with 
%qualitatively similar results. 


==> discussion.tex <==

\noindent \textbf{Global FPs vs LD FPs.} As remarked in the Introduction, an FP
of 1\% at the global level means that we will see one alert every 100 - 300
hours (for the phishing scenario) and 100 seconds (for waterhole scenario 
the neighborhood time window slides by 1 second). This reduces work to 
be performed by the deeper, second-level analysis considerably.

Specifically, LDs operating at 6\% false positive rate generate 23.5M -- 70M
FPs within 100--300 hours time interval in a network of 1086 nodes (phishing)
and 300K alerts within every 100 sec interval where neighborhoods include
$\sim$50K nodes on average (waterhole). Shape GD filters these alerts.  When
using 1--3 hours (phishing) and 6 sec (waterhole) time-based neighborhood
filtering, Shape GD will report to a system running a deeper analysis
approximately 234.5K -- 703.7K FPs raised by LDs (phishing) and approximately
1.4K FPs (waterhole).  Adding structural filtering brings these numbers down to
21.6K -- 64.8K FPs (phishing) and 360 FPs (waterhole).

Compared to a neighborhood of LDs, Shape GD thus reduces  the number of FPs
reported to deeper analyses by $\sim$100$\times$ and $\sim$200$\times$ when
employing time-based filtering only (for phishing and waterhole scenarios
respectively), while structural filtering reduces alert-FVs for deeper analysis
to $\sim$1000$\times$ and $\sim$830$\times$.
%by $\sim10\times$ and $\sim4\times$ correspondingly Shape GD reports 
%Note that the waterhole scenario gains less from structural filtering than
%phishing because structural filtering leads to an increase in neighborhood time
%window (in waterhole scenario) from 6 second up to 25 second, adding many more
%benign FVs per neighborhood.  
In both scenarios, analysts can choose to reduce
number of alert-FVs to be analyzed by sliding neighborhood windows by a larger
interval; however, this will increase the time to detect malware infection.




\noindent \textbf{Shape property across LDs and platforms.} \sysname relies on conditional
separability of FPs and TPs, and we use only one LD type for evaluation -- a
system call histogram-based LD.  However, we have experimentally determined
that FPs and TPs are separable for other LD types as well -- an n-gram-based
LD~\cite{mutant_x} and an LD that uses VirusTotal~\cite{virustotal} reports for
malware detection~\cite{vt_report_classification}.  Further, we can classify
malicious neighborhoods on the Android platform -- using malware binaries
obtained from the NCSU dataset and contagio dump website, and using benign
applications that we drive using real human user input -- in addition to the
Windows setup that we describe here. We have left out the details due to lack
of space but can produce an anonymous report if requested.

Though the local detectors we built have a 6\% FP rate, \sysname can work well
work with better LDs. \sysname only requires LD's FPs and TPs to be separable
and to be able to aggregate enough alert-FVs across the nodes within a
neighborhood.  We deliberately do not consider rule-based LDs that are commonly
used within enterprise networks because, even though their FP rate is very low,
they suffer from a high false negative rate, and they can be easily evaded with
simple malware transformations.

% \noindent \textbf{Templates for unknown attacks.}  \mikhail{We make an
%   assumption that for each known network-level attack it is possible
%   to define a neighborhood formation template based on the semantics
%   of an
%   attack.%, i.e. the rules to aggregate nodes into a neighborhood.
%   Since the number of network-level attacks (e.g. waterhole, phishing
%   and etc) is reasonable, then development of an individual template
%   for each attack is a feasible process that is performed only once.
%   Once a new attack is detected, a corresponding template needs to be
%   developed, however, new attack types do not emerge frequently.  }

% \noindent \textbf{What if FPs and TPs are indistinguishable?}
% \mikhail{
% One may challenge the main assumption about distinguishability of FP and TP distributions, 
% which forms the basis for Shape GD.
% They can be indistinguishable only if LDs are perfect, i.e. they extract all useful 
% information from the data. However, machine learning algorithms often involve solving NP-hard 
% problems, and to accomplish this they fall back on using various heuristics. 
% Therefore, it is very unlikely for practical machine learning algorithms to retrieve all the 
% information from the underlying data. As a consequence, their FPs and TPs bear information 
% allowing Shape GD to separate them.
% }




%\section{Discussion}
%\label{sec:discussion}
%\mikhail{
%\noindent \textbf{Why is Shape GD an anomaly detector?}
%We deliberately design Shape GD as an anomaly detector because we want to exclude malware from the training process. Malware authors are antagonistic to defenders and thus they continuously modify malware to evade detection. Consequently, relying on incomplete estimation of malware statistical properties might make Shape GD vulnerable to evasion attacks (cite Laskov). 
%On the contrary, developers of benign software are either cooperative or neutral to Shape GD. Therefore,  statistical properties of benign apps are more stable and are less likely subject to abrupt behavioral changes or changes due to the deployment of ShapeGD.
%}
%
%\noindent \textbf{Mimicry attacks on Shape GD}
%\mikhail{We do not analyze how hard or how easy it would be to mount a mimicry attack on Shape GD. Though, it is a valid research question, it lies outside the scope of the current paper.}
%
% How to detect malware when community has mixed devices or LDs
% basically, the idea we discussed was if the distribution doesn't
% change much then training set should capture it

% On applying to more fuzzy communities and neighborhoods.

% On malware that is not always generating malicious FVs. Constants
% will stretch. Also, currently malicious FVs include benign activity.

%\noindent {\bf \todo{Is Shape GD fundamentally sound?}}
%\todo{Nbd reduces dimensions. Squeeze more signal from set of alert-FVs
%once they have been grouped. Cite theory/sigmetrics paper?}



%%%%%%%%%%%%%%%%%
\input{overhead.tex}



\noindent{\bf Detailed Shape-GD Pipeline.}
As an extension to the description in Section 4, 
Figure~\ref{fig:shape-gd-pipeline} shows the 
detailed machine learning pipeline for extracting 
one neighborhood's shape into a ShapeScore.

\begin{figure}[t]
\includegraphics[width=0.48\textwidth]{figs/FE_pipeline.pdf}\par
\caption{(Overview) Shape-GD machine learning pipeline.}
\vspace{-0.2in}
\label{fig:shape-gd-pipeline}
\end{figure}



\ignore {
\mikhail{Drop it?!}
\noindent {\bf Applying Shape GD to real-world, heterogeneous enterprise
datasets.} Our current experiments rely on a homogeneous CIDS where 
%(similar to Facebook's {\tt osquery} based analysis) 
each node runs the same LD. 
%the same set of LDs are deployed on each node.
Our future work includes deploying Shape GD in a heterogeneous system with
several LDs, each with its own set of features and time-scales of analysis, that
pool data into SIEM tools with arbitrary delays --
%Appendix~\ref{sec:accenture} 
Appendix~B
describes our initial results in this
direction.

In summary, we apply Shape GD to 5.5 Billion security log entries (from 20 LD types) in an
enterprise with over 150K devices. Starting with 700K unique domain names
visited by the enterprise devices, we first use SecureRank~\cite{secure_rank}
and VirusTotal~\cite{virustotal} to rank the domains in order from benign to
potentially malicious. The key result is that even if we start with the 100
most suspicious domains generated by SecureRank and VirusTotal -- that led to 30
unique security incidents -- Shape GD (set to 97 percentile $\gamma$ threshold)
is able to identify the top 25 domains as malicious before they generate a
confirmed signature-based LD alert (and thus pre-empt 15 confirmed exploits).
At 98 and 99 percentiles, Shape GD can pre-empt 11 and 7 of the 30 exploits
respectively -- flagging only 15 and 5 neighborhoods (domains) respectively
from the top 100 domains {\em already filtered} using SecureRank and
VirusTotal.  This suggests that Shape GD can act as a prioritization scheme
when applied to a heterogeneous system -- a deeper study of this challenge
forms part of our future work.
}

\ignore{ % Replaced by Accenture
\noindent \textbf{Heterogeneous neighborhoods.}
We have evaluated Shape GD for the case of homogeneous neighborhoods, i.e. all
the nodes run the same operating system (Windows) and LDs of the same type
(Random Forest). The shape idea may apply to heterogeneous neighborhoods
comprising of heterogeneous devices (e.g. mobile, desktop), and with
heterogeneity among the LDs (e.g. operating at different levels of the
hardware/software stack, different versions).

An extension of our work to this setting is plausible by constructing a
vector-histogram (Section~\ref{sec:model}) of higher dimensionality (in the
worst case, number of LD types times the number of system types). This would
potentially work if there are sufficient numbers of nodes of each type, so that
the higher dimension vector-histogram exhibits `typical' statistics. Such a
setting might be particularly interesting for security providers who are
monitoring large networks, where there would be a sufficiency of nodes in a
neighborhood for such statistical concentrations to occur. Finally, a
particularly interesting scenario would be to deploy multiple lightweight
heterogeneous LDs on each system and perform intra-system statistical shape
analysis. We leave these directions for future work.


% Shape GD identifies truly
%malicious neighborhoods from false positives -- i.e., detects anomalies -- by
%comparing a neighborhood's ShapeScore against the reference histogram trained
%on false positive alert-FVs. Shape GD thus only requires the training stage
%(when reference histogram is computed) to be a good representation of the
%neighborhood at test stage -- the neighborhood machines and LDs themselves can
%be heterogeneous (a mix of Windows and Linux machines in an enterprise, for
%example) even if our experiments in this paper are not (for artifactual
%reasons). 

%\noindent{\bf Statistiscal distinguishability of LD TPs and FPs.}
%In practice, system call traces from malware exploits and payloads (i.e TPs)



\noindent \textbf{Deep Learning.} Behavioral analysis using machine
learning approaches are becoming increasingly popular in industry,
thanks to the vast amount of data and new ``high dimensional''
algorithms that are becoming prevalent (e.g. deep nets). With their
ability to extract highly effective features, deep nets may provide a
new way forward for creating novel behavioral detectors. At the global
level, however, what is needed is a data-light approach for global
detection by composing local detectors, tailored to be agile enough to
do global detection in a fast-changing (non-stationary) environment.

Our work addresses precisely this problem.  We believe that our
approach effectively serves as a lens for dimensionality reduction and
is thus complementary to the state-of-the-art behavioral analyses
approaches.


}

\section{How fragile is Count GD to errors in estimating neighborhood size? (Phishing)}
\label{sec:phishing-countgd}

\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/windows/enron/noisy_count.eps}\par
\caption{{\em(Phishing attack) An error in estimating neighborhood size dramatically affects Count GD's performance. 
It can tolerate at most 2\% underestimation errors and 6.3\% overestimation errors to achieve comparable with Shape GD performance.}
\vspace{-0.2in}
\label{fig:windows-noisy_count}}
\end{figure}

Due to space considerations, we have placed the results for Count GD's 
fragility to mis-estimated neighborhood sizes in the appendix in Figure~\ref{fig:windows-noisy_count}.
The key trends are similar to waterhole attack presented in the main paper -- 
even a slight under- or over-estimate of dynamic neighborhoods' sizes
can yield completely inaccurate results.



==> exp_justification.tex <==
\sysname experiments require datasets where the global detector can acquire
alert-FVs from local detectors, similar to {\tt osquery}-based systems where
the LD and GD are co-designed. We describe our experience with three existing
methodologies and datasets -- none of them allow alert-FVs to be acquired,
provide complete ground truth infection information, or allow the infection
rate to be varied. This motivates the methodology we use to systematically
evaluate \sysname. 

\noindent{\bf Analysis of existing datasets.}
Prior work has used enterprise logs~\cite{mining_log_data_alina_oprea} that are
unavailable publicly.  We have acquired similar security logs from a Fortune 500
company with a 200K machine network -- the logs average 250M entries per day
over a 2 year period, arise from  20 closed-source endpoint local detectors
such as Symantec, McAfee, Blue Coat, etc, have almost 500 sparsely populated
dimensions per log entry, and about 75\% of the log entries lack important
identity and event-timestamp information and are delayed by up to 60 days.
Commercial (black-box) LDs do not expose feature vectors for external analysis.

We have also acquired network {\tt pcap} traces from our university network,
emulating prior work~\cite{network_intrusion_detection} in network-only global detectors.
University security groups (like ours) are only allowed to collect
network-layer {\tt pcap} information for a rolling 2-week period and cannot
instrument host machines (that are owned by students and visitors) -- i.e., our
4TB/day dataset from 150K machines is unsuitable to evaluate \sysname because
it doesn't have LDs. Extending this dataset with a weak LD -- the ability to
inspect executables in a sandbox downloaded by hosts (e.g., as pursued by
Lastline~\cite{lastline}) -- would be an appropriate experimental setup but
sensitive data issues make such datasets hard to get. Hence, we model this
extended setup in our methodology. 

We have analyzed Symantec's WINE dataset~\cite{downloader_graphs} and found it inadequate to
evaluate \sysname even after layering VirusTotal information on it.
Specifically, the WINE dataset includes downloader
graphs~\cite{downloader_graphs} -- the nodes are executables and the edges
represent whether the source downloaded the destination executable -- and
represent downloader trojans (`droppers') in malware distribution
networks~\cite{malware_distribution_net} that download payloads to steal
information, encrypt the disk, etc on to the host.  This dataset covers 5 years
of data with 25M files (specifically, hashes that represent files) on over 1M
machines -- however, only 1.5M of the 25M hashes have reports on VirusTotal.
Hence, one cannot reconstruct (alert) feature vectors for the hashes stored in
the downloader graph.

\sysname re-analyzes (local) alert feature vectors in the global detector --
filtering alert-FVs into neighborhoods and then computing the neighborhoods'
shapes.  
%\sysname evaluations require quantifying the short-lived and unpredictable
%correlations that are created due to attack vectors -- 
%\sysname algorithms thus directly apply to 
Hence we model {\tt osquery}-like
deployments as used in enterprises like Facebook and Google where the LDs and
GDs are co-designed and GDs can acquire alert-FVs. 

\noindent{\bf Simulating malware propagation in a network.} Methodologies that
use existing datasets with malware propagation (like the ones above) have an
inherent weakness. Such datasets have one sequence of malware propagation
events ``hardwired'' into the dataset and do not allow us to analyze how a
detection mechanism reacts to variations of malware propagation dynamics,
especially when malware can adapt these dynamics.  Instead, we propose to vary
the rate of infection (which changes the neighborhood formation) and determine
\sysname's detection performance across different infection rates.

%Methodologies that use existing infection traces have a larger fundamental
%weakness. Each dataset is a single (network-level) trace, which  
%%that represents an actual malware infection trace is 
%is meaningless when malware is dynamic and adapts to proposed defenses. 
%%instead of detection results for one malware infection trace, 
%Instead, we propose to vary the rate of infection (which changes the
%neighborhood formation) and determine \sysname's detection performance across
%different infection rates.

Further, none of the above datasets provide ground truth information about the
true extent of infections, 
%making it hard to determine false negatives and
incentivizing a design that minimizes false positives at the expense of false
negatives. In a controlled setting where host-level malware and benignware traces 
are overlaid onto a trace of web-service/email communication, we can maintain
ground truth information and determine false positives and negatives precisely.

To this end, we use a malware and benignware dataset from a recent related
work~\cite{kruegel-bare-metal}, 
%to run malware and benignware on host machines,
train an LD with histogram-based feature vectors and a Random Forest detector
based on a recent survey on host-level malware detection~\cite{Canali2012},
%(Appendix~\ref{} shows that we achieve equivalent detection results on our
%dataset), 
and overlay these host-level results on web-service (network) and email traces
using two standard (and publicly available) datasets from Yahoo data centers
and Enron respectively. We describe this methodology in detail next.


%
%In this section we justify our experimental setup, show that it extends
%a state-of-the-art SIEM infrastructure by adding the missing features that are 
%vital for Shape-GD, and demonstrate that simulated attacks closely resemble
%the attacks that Sednit hackers group~\cite{eset_sednit_fancy_bear}
%has been extensively using over more than ten years for cyberespionage.
%
%%We deliberately choose a white-box methodology for ShapeGD's evaluation
%%and in this section we outline the reasons for such a choice.
%
%\noindent {\bf Local detectors and network traces.}
%As described in Section~\ref{}, Shape GD requires both homogeneous local 
%detectors being deployed on endpoint machines, which can send alert-FVs 
%to Shape GD, and network-related data (accessed websites and received emails) 
%to appropriately form neighborhoods.
%Initially, we were trying to prototype the entire system on top of 
%an existing SIEM data collection framework within a Fortune-500 company and within an 
%information security office at a university. The former infrastructure 
%collects data across 200,000 machines, while the later monitors 100,000
%machines.
%
%The main obstacle that we faced is the lack of suitable endpoint malware detectors 
%that can transmit alert-FVs back to ShapeGD. Usually commercial detectors 
%output one bit of information (alert or no-alert). Even if some detectors 
%output additional information in the case of raising an alert, it's not the
%data that was actually analyzed by the detector before raising an alert.
%In other words, it's simply the data derived from the original alert-FV.
%
%The other challenge for the proposed Shape GD algorithm was 
%a missing or inaccurate "device ID" field in the incoming data sent by
%local detectors, which is supposed to uniquely identify an endpoint device.
%Quite often malware detectors use local device IP as an identifier ("device ID"), 
%which is very unreliable way of identifying devices due to IP collision across 
%multiple local networks. Sometimes, when a malicious activity is detected
%during a signature scan of the file system, malware detectors do not report
%machine's IP at all. In such cases, they are supposed to report a MAC address, 
%but due to privacy concerns they are configured not to do that.
%Likely, approximate device IDs can be retrieved from the data sets, however,
%this problem is orthogonal to our paper because we assume device IDs 
%are available.
%
%We also found that those two data sets contain a lot of corrupted and
%missing data due to periodic infrastructure failures, network shortages, and
%misconfiguration of endpoint malware detectors reporting the data.
%
%Finally, after multiple rounds of interacting with the incidence response teams
%within those two organizations, we found out that ground truth 
%(e.g. attack vectors, the exact number of infected machines) is unavailable.
%Thus, it was impossible to estimate how quickly Shape GD could catch malware 
%and what percentage of infected machines it could detect.
%
%We closely collaborating with those two organizations and developing an infrastructure
%from ground up that includes virtual machines with custom local detectors and
%network-level tools for monitoring the communication between them. 
%However, we leave this to future work.

%\noindent {\bf Sensitivity study.}
%%We believe that any protection mechanism based on machine learning needs to undergo
%%a thorough evaluation to understand how sensitive a system is to modified attacks.
%%It's a well-known fact that machine learning algorithms are susceptible to evasion 
%%attacks~\cite{evade-ml,evade-pdf,practical_black_box_attacks}.
%
%Though the real data sets that would allow to evaluate ShapeGD don't exist, but 
%if they existed, they would not let us perform a sensitivity study due to inability 
%to adjust parameters of malware spread (Section~\ref{}).
%Thus, this served as an additional reason for evaluating ShapeGD in a simulated environment.

%\noindent {\bf .} 
%We propose a new methodology for evaluating collaborative intrusion
%detection systems, which combines the best practices from the previous work.

%Note that simulated phishing and waterhole attacks match the similar
%attacks deployed by Sednit hacker group~\cite{eset_sednit_fancy_bear}, which presumably stands
%behind DNC hack in 2016 and other notorious campaigns.
%Sednit group primarily relies on phishing and waterhole attacks to fulfill their cyberespionage
%goals. For example, the Eset report~\cite{eset_sednit_fancy_bear} describes
%a phishing attack against the targets in Ukraine that took place in May 2016.
%Had those targets belonged to a single neighborhood, Shape GD would have discovered such an attack,
%especially, given high (more than 50\%) click rate on malicious links and given hackers'
%persistence to phish a victim (at most 7 times) until success.
%
%The other way of attacking victims that is widely used by Sedkit hackers is to impersonate
%legitimate domains. For example, they created stratforglobal.net that looks like the official website
%of an Austin-based intelligence company Stratfor, whose official domain name is
%stratfor.com. The hackers lure innocent victims with fake emails to visit the websites under their 
%control that automatically exploit victims' machines and plant persistent malware.
%As in the previous case, if Shape GD used per website neighborhoods (Section~\ref{}),
%then it would likely to identify the malware campaign at an early stage.


==> experimental-setup/app-table.tex <==
\begin{table}[t]
\centering
\begin{tabular}{ l  p{5cm} }
  % \label{table:app-table}
  \multicolumn{2}{c}{User Traces} \\
  \hline
  App & Description of User Activity \\ \hline
  Wikipedia & Browse and search multiple articles  \\            %\hline
  Allrecipes & Search for recipes, scroll through recipe photos \\               %\hline
  Yelp & Browse local catering, read reviews \\                       %\hline
  HTML5 Reference & Repeatedly open and read documentation \\  %\hline
  Sana & fill out medical survey \\
  \hline
  & \\                                          %\hline
  \multicolumn{2}{c}{Monkey} \\                \hline
  App & Description \\ \hline  
  Walmart & Online shopping \\                  %\hline
  AVG & Free antivirus \\                       %\hline
  Buzzfeed & Social news \\                     %\hline
  eBay & Online Auction \\                      %\hline
  Zedge & Wallpaper and Ringtones \\            %\hline
  The Holy Bible & Holy Text \\                 %\hline
  \hline
\end{tabular}
\end{table}

==> experimental-setup/appStatsTableProcessed.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{p{1.3cm} p{1.5cm} c c c c c c c c c c}
\multicolumn{2}{c}{} & \multicolumn{2}{c}{File Ops} & \multicolumn{2}{c}{Network Ops} & \multicolumn{2}{c}{Process Ctrl} & \multicolumn{2}{c}{System Wide} &\multicolumn{2}{c}{Misc} \\
App & Config & $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$\\\hline
Allrecipes&Benign&8.08e+02&3.78e+02&1.97e+00&1.56e+02&0.00e+00&1.77e+03&3.53e+02&1.06e+01&2.05e+02&0.00e+00\\
Allrecipes&File stealer&3.12e+03&2.12e+00&7.76e+02&2.37e+02&1.97e+02&6.26e+03&5.17e+00&1.63e+03&4.93e+02&5.81e+02\\
Allrecipes&Contacts stealer&3.29e+03&2.47e+00&8.67e+02&2.69e+02&2.31e+02&6.39e+03&5.74e+00&1.81e+03&5.40e+02&6.89e+02\\
Allrecipes&SMS stealer&3.12e+03&2.14e+00&7.49e+02&2.29e+02&2.05e+02&6.76e+03&5.24e+00&1.54e+03&4.69e+02&6.34e+02\\
Allrecipes&Other stealer&3.34e+03&2.40e+00&8.97e+02&2.73e+02&2.49e+02&6.30e+03&5.40e+00&1.76e+03&5.19e+02&7.79e+02\\
Allrecipes&Click fraud&3.32e+03&2.30e+00&8.21e+02&2.52e+02&2.19e+02&6.30e+03&5.29e+00&1.62e+03&4.78e+02&6.62e+02\\
Allrecipes&GET flood&3.13e+03&2.26e+00&7.85e+02&2.44e+02&1.91e+02&6.14e+03&5.41e+00&1.47e+03&4.73e+02&5.35e+02\\
Allrecipes&SHA1- cracker&3.08e+03&2.29e+00&8.27e+02&2.48e+02&2.20e+02&6.31e+03&5.43e+00&1.74e+03&5.00e+02&6.88e+02\\ 
\hline
AVG&Benign&3.39e+02&1.71e+01&5.10e+00&1.72e+02&1.31e-02&7.51e+02&5.57e+01&4.31e+01&1.49e+02&1.84e-01\\
AVG&File stealer&2.79e+03&2.93e+01&1.40e+03&3.91e+02&3.18e+02&3.99e+03&2.01e+01&1.20e+03&4.18e+02&1.04e+03\\
AVG&Contacts stealer&3.01e+03&2.91e+01&1.25e+03&3.99e+02&3.24e+02&4.22e+03&1.96e+01&1.37e+03&4.52e+02&1.01e+03\\
AVG&SMS stealer&3.03e+03&2.88e+01&1.30e+03&3.96e+02&3.68e+02&3.95e+03&1.96e+01&1.20e+03&4.10e+02&1.26e+03\\
AVG&Other stealer&2.68e+03&2.76e+01&1.62e+03&3.89e+02&3.58e+02&4.76e+03&2.03e+01&1.53e+03&6.02e+02&1.16e+03\\
AVG&Click fraud&3.13e+03&2.95e+01&1.07e+03&4.06e+02&2.78e+02&4.03e+03&2.17e+01&1.16e+03&4.52e+02&9.58e+02\\
AVG&GET flood&3.26e+03&3.04e+01&1.03e+03&4.01e+02&3.14e+02&3.82e+03&1.95e+01&9.16e+02&3.69e+02&1.04e+03\\
AVG&SHA1- cracker&2.80e+03&2.79e+01&1.49e+03&4.03e+02&3.28e+02&3.89e+03&1.87e+01&1.34e+03&3.95e+02&1.12e+03\\
\hline
The Bible&Benign&2.22e+02&1.51e+01&1.92e+00&2.12e+02&1.98e-04&1.88e+02&1.43e+01&5.21e+00&1.31e+02&2.67e-02\\
The Bible&File stealer&1.08e+03&4.00e+01&1.02e+03&3.11e+02&2.62e+02&9.19e+02&2.37e+01&6.87e+02&2.55e+02&4.63e+02\\
The Bible&Contacts stealer&1.26e+03&4.21e+01&8.84e+02&3.13e+02&2.49e+02&9.59e+02&5.90e+01&7.25e+02&2.46e+02&3.86e+02\\
The Bible&SMS stealer&1.27e+03&4.18e+01&8.71e+02&3.09e+02&2.45e+02&1.12e+03&2.91e+01&7.54e+02&3.03e+02&4.50e+02\\
The Bible&Other stealer&1.08e+03&3.95e+01&1.14e+03&3.20e+02&2.77e+02&1.16e+03&2.75e+01&7.78e+02&3.13e+02&4.74e+02\\
The Bible&Click fraud&1.45e+03&4.27e+01&7.41e+02&3.23e+02&2.52e+02&1.07e+03&3.15e+01&7.40e+02&2.92e+02&4.84e+02\\
The Bible&GET flood&1.38e+03&4.20e+01&7.38e+02&3.11e+02&2.27e+02&8.12e+02&2.07e+01&6.32e+02&1.89e+02&4.27e+02\\
The Bible&SHA1- cracker&1.16e+03&4.06e+01&9.77e+02&3.09e+02&2.50e+02&9.44e+02&5.51e+01&7.09e+02&2.43e+02&4.27e+02\\
\hline
Buzzfeed&Benign&5.04e+02&3.52e+01&4.93e+00&3.00e+02&0.00e+00&4.71e+02&3.71e+01&8.19e+00&5.91e+02&0.00e+00\\
Buzzfeed&File stealer&3.92e+03&2.58e+01&1.26e+03&3.49e+02&2.06e+02&4.39e+03&1.52e+01&1.31e+03&2.53e+02&3.96e+02\\
Buzzfeed&Contacts stealer&3.83e+03&2.38e+01&1.48e+03&3.84e+02&2.65e+02&4.29e+03&1.45e+01&1.34e+03&2.99e+02&4.62e+02\\
Buzzfeed&SMS stealer&3.65e+03&2.41e+01&1.64e+03&3.51e+02&2.95e+02&4.23e+03&1.45e+01&1.56e+03&2.85e+02&6.88e+02\\
Buzzfeed&Other stealer&3.16e+03&2.26e+01&2.03e+03&3.21e+02&4.33e+02&3.60e+03&1.37e+01&1.74e+03&2.11e+02&1.01e+03\\
Buzzfeed&Click fraud&3.62e+03&1.95e+01&1.73e+03&4.24e+02&3.17e+02&4.33e+03&1.31e+01&1.32e+03&3.44e+02&5.02e+02\\
Buzzfeed&GET flood&4.31e+03&2.43e+01&1.24e+03&3.70e+02&1.77e+02&4.75e+03&1.45e+01&1.17e+03&3.10e+02&3.58e+02\\
Buzzfeed&SHA1- cracker&3.56e+03&2.22e+01&1.64e+03&3.57e+02&2.12e+02&4.04e+03&1.36e+01&1.42e+03&2.89e+02&3.51e+02\\
\hline
eBay&Benign&7.12e+01&1.00e+01&1.93e+00&1.54e+02&0.00e+00&6.73e+01&1.11e+01&7.55e+00&1.12e+02&0.00e+00\\
eBay&File stealer&1.77e+03&5.36e+01&9.12e+02&6.97e+02&1.85e+02&1.35e+03&3.27e+01&7.89e+02&4.83e+02&1.61e+02\\
eBay&Contacts stealer&1.75e+03&5.15e+01&9.67e+02&6.76e+02&1.85e+02&1.31e+03&2.96e+01&8.27e+02&4.30e+02&1.69e+02\\
eBay&SMS stealer&1.86e+03&5.12e+01&9.29e+02&6.70e+02&1.76e+02&1.56e+03&3.56e+01&8.96e+02&5.20e+02&1.89e+02\\
eBay&Other stealer&1.71e+03&5.24e+01&9.88e+02&6.84e+02&1.84e+02&1.46e+03&3.28e+01&8.96e+02&4.96e+02&1.60e+02\\
eBay&Click fraud&1.78e+03&5.16e+01&9.16e+02&6.83e+02&1.81e+02&1.23e+03&2.99e+01&8.03e+02&4.40e+02&1.78e+02\\
eBay&GET flood&1.74e+03&5.26e+01&9.78e+02&7.02e+02&1.99e+02&1.44e+03&3.36e+01&9.18e+02&5.26e+02&2.29e+02\\
eBay&SHA1- cracker&1.84e+03&5.31e+01&9.41e+02&6.92e+02&1.88e+02&1.44e+03&3.08e+01&8.53e+02&4.57e+02&2.22e+02\\
\hline
Html5 Ref.&Benign&5.19e+01&7.87e+00&3.30e+00&1.25e+02&1.94e-02&6.77e+01&1.05e+01&3.18e+01&2.04e+02&1.90e-01\\
Html5 Ref.&File stealer&1.06e+03&2.00e+00&6.53e+02&9.64e+01&1.01e+02&2.07e+03&6.81e+00&1.03e+03&3.46e+02&2.18e+02\\
Html5 Ref.&Contacts stealer&7.32e+02&1.85e+00&4.44e+02&5.81e+01&1.01e+02&1.06e+03&6.39e+00&6.57e+02&1.59e+02&1.97e+02\\
Html5 Ref.&SMS stealer&7.63e+02&2.08e+00&4.67e+02&6.53e+01&1.14e+02&1.04e+03&6.63e+00&5.70e+02&1.70e+02&2.28e+02\\
Html5 Ref.&Other stealer&7.95e+02&2.22e+00&4.64e+02&6.21e+01&1.14e+02&1.08e+03&6.81e+00&5.27e+02&1.65e+02&2.11e+02\\
Html5 Ref.&Click fraud&7.44e+02&1.69e+00&4.54e+02&6.56e+01&1.04e+02&1.07e+03&6.05e+00&5.47e+02&1.66e+02&2.10e+02\\
Html5 Ref.&GET flood&6.18e+02&1.32e+00&4.25e+02&6.70e+01&9.64e+01&9.15e+02&5.32e+00&5.88e+02&1.61e+02&1.93e+02\\
Html5 Ref.&SHA1- cracker&7.64e+02&1.71e+00&4.52e+02&6.10e+01&1.01e+02&1.10e+03&6.10e+00&5.73e+02&1.66e+02&2.05e+02\\
\hline
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{p{1.3cm} p{1.5cm} c c c c c c c c c c}
\multicolumn{2}{c}{} & \multicolumn{2}{c}{File Ops} & \multicolumn{2}{c}{Network Ops} & \multicolumn{2}{c}{Process Ctrl} & \multicolumn{2}{c}{System Wide} &\multicolumn{2}{c}{Misc} \\
App & Config & $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$\\\hline
Walmart&Benign&1.34e+02&9.97e+00&1.56e+00&1.21e+02&0.00e+00&1.34e+02&1.31e+01&6.50e+00&1.01e+02&0.00e+00\\
Walmart&File stealer&1.94e+03&3.14e+01&1.31e+03&2.97e+02&3.09e+02&1.41e+03&2.26e+01&1.14e+03&1.86e+02&5.83e+02\\
Walmart&Contacts stealer&1.95e+03&3.15e+01&1.26e+03&3.00e+02&3.06e+02&1.40e+03&2.29e+01&1.09e+03&2.28e+02&4.79e+02\\
Walmart&SMS stealer&2.19e+03&3.23e+01&1.11e+03&3.01e+02&2.72e+02&1.42e+03&2.24e+01&1.10e+03&1.81e+02&4.48e+02\\
Walmart&Other stealer&1.86e+03&3.14e+01&1.49e+03&2.96e+02&3.36e+02&1.58e+03&2.39e+01&1.11e+03&2.18e+02&5.96e+02\\
Walmart&Click fraud&2.23e+03&3.33e+01&1.09e+03&3.11e+02&2.96e+02&1.48e+03&2.34e+01&1.10e+03&2.15e+02&4.88e+02\\
Walmart&GET flood&1.96e+03&3.08e+01&1.24e+03&2.94e+02&3.04e+02&1.58e+03&2.20e+01&1.08e+03&1.91e+02&5.25e+02\\
Walmart&SHA1- cracker&2.07e+03&3.18e+01&1.19e+03&2.96e+02&2.87e+02&1.43e+03&2.37e+01&1.22e+03&1.90e+02&4.54e+02\\
\hline
Wikipedia&Benign&5.97e+01&4.30e+00&1.27e+00&5.23e+01&1.73e-04&1.81e+02&1.25e+01&1.10e+01&1.49e+02&1.56e-02\\
Wikipedia&File stealer&1.16e+02&4.66e-02&1.15e+02&9.86e+00&7.49e+01&1.38e+02&7.63e-01&1.20e+02&2.35e+01&1.09e+02\\
Wikipedia&Contacts stealer&1.16e+02&3.83e-02&1.15e+02&9.57e+00&7.54e+01&1.35e+02&6.71e-01&1.17e+02&2.25e+01&1.12e+02\\
Wikipedia&SMS stealer&1.15e+02&4.62e-02&1.15e+02&9.39e+00&7.66e+01&1.34e+02&7.50e-01&1.23e+02&1.96e+01&1.22e+02\\
Wikipedia&Other stealer&1.15e+02&3.84e-02&1.14e+02&9.36e+00&7.47e+01&1.33e+02&6.69e-01&1.20e+02&1.77e+01&1.06e+02\\
Wikipedia&Click fraud&1.18e+02&4.35e-02&1.17e+02&9.66e+00&7.57e+01&1.46e+02&7.16e-01&1.21e+02&2.19e+01&1.10e+02\\
Wikipedia&GET flood&1.18e+02&4.14e-02&1.16e+02&1.01e+01&7.65e+01&1.41e+02&6.57e-01&1.19e+02&2.43e+01&1.21e+02\\
Wikipedia&SHA1- cracker&1.15e+02&4.82e-02&1.15e+02&9.57e+00&7.48e+01&1.35e+02&7.44e-01&1.19e+02&2.21e+01&1.12e+02\\
\hline
Yelp&Benign&1.43e+02&3.17e+01&5.95e+00&1.56e+02&9.35e-04&1.50e+02&3.89e+01&4.04e+01&1.48e+02&5.36e-02\\
Yelp&File stealer&3.54e+02&1.63e+00&2.55e+02&9.10e+01&1.78e+02&9.30e+02&2.09e+01&7.25e+02&2.62e+02&4.08e+02\\
Yelp&Contacts stealer&1.76e+02&7.23e-01&1.28e+02&4.58e+01&9.76e+01&7.15e+02&4.19e+00&4.91e+02&1.77e+02&2.94e+02\\
Yelp&SMS stealer&1.87e+02&7.70e-01&1.34e+02&4.73e+01&1.01e+02&6.81e+02&4.18e+00&4.74e+02&1.64e+02&2.99e+02\\
Yelp&Other stealer&1.66e+02&6.90e-01&1.29e+02&4.69e+01&1.02e+02&5.02e+02&3.92e+00&4.81e+02&1.62e+02&2.99e+02\\
Yelp&Click fraud&1.87e+02&7.82e-01&1.38e+02&4.82e+01&1.01e+02&8.92e+02&4.39e+00&5.05e+02&1.84e+02&2.96e+02\\
Yelp&GET flood&1.91e+02&7.57e-01&1.37e+02&4.84e+01&1.06e+02&6.71e+02&4.27e+00&4.66e+02&1.69e+02&3.19e+02\\
Yelp&SHA1- cracker&1.70e+02&6.91e-01&1.27e+02&4.37e+01&9.41e+01&6.82e+02&3.90e+00&4.84e+02&1.64e+02&2.88e+02\\
\hline
Zedge&Benign&9.33e+01&3.40e+00&1.97e+00&1.50e+02&7.41e-05&8.92e+01&6.59e+00&9.67e+00&1.15e+02&8.61e-03\\
Zedge&File stealer&1.48e+03&4.73e+01&1.10e+03&2.97e+02&2.20e+02&1.96e+03&2.59e+01&7.06e+02&2.61e+02&3.26e+02\\
Zedge&Contacts stealer&1.65e+03&4.58e+01&9.78e+02&3.09e+02&2.54e+02&2.00e+03&2.30e+01&7.77e+02&2.40e+02&4.60e+02\\
Zedge&SMS stealer&1.64e+03&4.61e+01&9.43e+02&2.93e+02&2.13e+02&1.89e+03&2.32e+01&7.18e+02&2.06e+02&3.52e+02\\
Zedge&Other stealer&1.39e+03&4.50e+01&1.27e+03&2.90e+02&2.47e+02&2.28e+03&2.39e+01&9.45e+02&2.61e+02&4.21e+02\\
Zedge&Click fraud&1.97e+03&4.61e+01&7.84e+02&3.16e+02&2.05e+02&2.20e+03&3.01e+01&8.27e+02&3.05e+02&3.81e+02\\
Zedge&GET flood&1.88e+03&4.66e+01&7.94e+02&3.00e+02&1.94e+02&2.19e+03&2.78e+01&7.11e+02&2.70e+02&3.14e+02\\
Zedge&SHA1- cracker&1.53e+03&4.55e+01&1.10e+03&3.04e+02&2.20e+02&1.85e+03&2.20e+01&7.62e+02&2.19e+02&3.48e+02\\
\hline
\end{tabular}
\end{table*}


==> experimental-setup/appStatsTableProcessed2.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{p{1.3cm} p{1.7cm} c c c c c c c c c c}
\multicolumn{2}{c}{} & \multicolumn{2}{c}{Info Ops} & \multicolumn{2}{c}{Network Ops} & \multicolumn{2}{c}{Process Ctrl} & \multicolumn{2}{c}{System Wide} &\multicolumn{2}{c}{Misc} \\
App & Config & $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$\\\hline
Allrecipes&Benign&807.63&378.09&1.97&156.20&0.00&1769.43&352.52&10.59&204.89&0.00\\
Allrecipes&Info Stealers&3178.85&2.23&800.42&245.51&211.39&6425.50&5.35&1662.49&501.25&638.63\\
Allrecipes&Click fraud&3318.07&2.30&821.33&252.16&218.89&6304.90&5.29&1615.40&477.94&662.00\\
Allrecipes&GET flood&3134.57&2.26&785.05&243.75&190.60&6135.10&5.41&1467.49&472.75&534.95\\
Allrecipes&SHA1 cracker&3075.08&2.29&827.06&247.84&220.24&6308.22&5.43&1741.13&499.81&687.64\\
\hline
AVG&Benign&338.76&17.14&5.10&172.43&0.01&751.44&55.70&43.11&149.18&0.18\\
AVG&Info Stealers&2896.67&28.99&1355.95&393.83&335.33&4111.68&19.86&1280.97&443.21&1103.83\\
AVG&Click fraud&3133.62&29.52&1069.81&406.28&277.86&4026.85&21.69&1163.93&451.92&958.07\\
AVG&GET flood&3262.63&30.41&1032.88&400.91&314.46&3817.12&19.54&916.25&369.20&1037.31\\
AVG&SHA1 cracker&2801.21&27.94&1486.22&402.53&327.56&3891.16&18.71&1337.88&395.46&1118.08\\
\hline
The Bible&Benign&222.07&15.05&1.92&211.67&0.00&187.52&14.34&5.21&131.44&0.03\\
The Bible&Info Stealers&1174.72&40.93&959.81&312.12&255.48&1008.98&37.60&727.33&270.56&442.15\\
The Bible&Click fraud&1445.97&42.70&740.60&322.89&252.10&1070.40&31.50&740.38&292.06&484.37\\
The Bible&GET flood&1384.36&42.04&738.36&311.23&226.70&812.16&20.67&632.14&189.40&427.20\\
The Bible&SHA1 cracker&1156.08&40.58&976.95&308.67&249.81&944.07&55.07&709.14&242.69&427.04\\
\hline
Buzzfeed&Benign&503.53&35.21&4.93&300.23&0.00&470.75&37.08&8.19&590.84&0.00\\
Buzzfeed&Info Stealers&3746.29&24.55&1487.21&353.92&266.82&4249.37&14.76&1455.20&267.37&591.31\\
Buzzfeed&Click fraud&3622.02&19.49&1731.58&424.10&317.23&4329.06&13.13&1316.29&343.91&502.08\\
Buzzfeed&GET flood&4312.83&24.30&1235.48&370.39&176.64&4753.77&14.46&1170.37&310.07&358.01\\
Buzzfeed&SHA1 cracker&3555.33&22.16&1640.07&357.31&211.90&4039.72&13.57&1423.65&289.22&351.29\\
\hline
eBay&Benign&71.20&10.04&1.93&154.16&0.00&67.30&11.13&7.55&112.19&0.00\\
eBay&Info Stealers&1784.51&52.32&935.80&683.49&182.76&1413.48&32.86&837.43&482.22&170.77\\
eBay&Click fraud&1782.21&51.57&916.41&683.32&180.77&1232.32&29.89&803.20&440.19&178.15\\
eBay&GET flood&1742.85&52.59&977.55&701.85&198.78&1438.88&33.61&918.20&526.44&229.09\\
eBay&SHA1 cracker&1836.04&53.06&940.86&692.20&187.92&1437.56&30.77&852.52&457.24&222.36\\
\hline
Html5 Ref.&Benign&51.87&7.87&3.30&125.07&0.02&67.74&10.50&31.80&204.46&0.19\\
Html5 Ref.&Info Stealers&1009.54&2.00&618.80&90.41&102.42&1938.86&6.77&973.80&321.83&217.16\\
Html5 Ref.&Click fraud&743.86&1.69&454.14&65.64&104.34&1068.09&6.05&546.56&166.04&209.80\\
Html5 Ref.&GET flood&617.56&1.32&424.71&67.00&96.42&914.87&5.32&588.45&160.95&193.38\\
Html5 Ref.&SHA1 cracker&763.65&1.71&452.21&60.98&101.19&1104.86&6.10&573.21&165.91&205.48\\
\hline
Walmart&Benign&134.10&9.97&1.56&121.04&0.00&133.74&13.05&6.50&100.98&0.00\\
Walmart&Info Stealers&1999.18&31.67&1262.06&298.76&301.18&1430.67&22.76&1119.04&199.53&527.00\\
Walmart&Click fraud&2229.72&33.28&1092.56&310.69&295.99&1479.60&23.36&1096.63&215.25&487.80\\
Walmart&GET flood&1959.11&30.80&1241.82&293.67&303.67&1582.72&22.01&1084.04&190.90&525.16\\
Walmart&SHA1 cracker&2069.16&31.80&1185.04&296.22&287.45&1434.59&23.72&1215.58&190.38&453.51\\
\hline
Wikipedia&Benign&59.71&4.30&1.27&52.27&0.00&181.11&12.49&10.96&148.95&0.02\\
Wikipedia&Info Stealers&115.88&0.04&115.10&9.61&75.48&135.56&0.73&120.09&21.74&113.02\\
Wikipedia&Click fraud&118.18&0.04&116.65&9.66&75.66&145.88&0.72&120.79&21.91&109.86\\
Wikipedia&GET flood&117.90&0.04&116.38&10.08&76.51&140.62&0.66&119.14&24.29&121.10\\
Wikipedia&SHA1 cracker&115.47&0.05&115.00&9.57&74.81&135.24&0.74&118.96&22.11&111.52\\
\hline
Yelp&Benign&142.71&31.71&5.95&156.44&0.00&150.31&38.91&40.37&148.35&0.05\\
Yelp&Info Stealers&246.35&1.08&178.53&63.70&129.87&787.28&13.37&590.97&210.95&345.86\\
Yelp&Click fraud&186.80&0.78&137.90&48.21&100.56&891.92&4.39&504.53&183.96&296.34\\
Yelp&GET flood&190.54&0.76&136.63&48.37&105.58&671.18&4.27&465.84&168.69&319.15\\
Yelp&SHA1 cracker&169.80&0.69&126.89&43.68&94.08&681.62&3.90&484.41&163.90&288.38\\
\hline
Zedge&Benign&93.34&3.40&1.97&149.50&0.00&89.23&6.59&9.67&114.70&0.01\\
Zedge&Info Stealers&1555.80&46.45&1043.32&298.34&229.11&1984.82&24.37&755.74&243.52&378.27\\
Zedge&Click fraud&1969.47&46.08&784.39&316.30&205.36&2197.14&30.05&826.79&305.11&380.56\\
Zedge&GET flood&1880.25&46.57&793.67&300.48&193.63&2191.07&27.84&711.39&270.40&313.79\\
Zedge&SHA1 cracker&1528.01&45.52&1097.38&304.17&219.51&1851.26&22.01&761.71&219.38&347.92\\
\hline
\end{tabular}
\end{table*}

==> experimental-setup/malware-propogation-model.tex <==
The malware propogation model follows an exponential distrub ...

This is similar to some tuberculosis infection models \sanjay{PLEASE CITE}

==> experimental-setup/small-stats-table.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{p{1.3cm} p{1.7cm} c c c c c c c c c c}
\multicolumn{2}{c}{} & \multicolumn{2}{c}{File Ops} & \multicolumn{2}{c}{Network Ops} & \multicolumn{2}{c}{Process Ctrl} & \multicolumn{2}{c}{System Wide} &\multicolumn{2}{c}{Misc} \\
App & Config & $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$\\\hline
Wikipedia&Benign&59.71&4.30&1.27&52.27&0.00&181.11&12.49&10.96&148.95&0.02\\
Wikipedia&Info Stealers&115.88&0.04&115.10&9.61&75.48&135.56&0.73&120.09&21.74&113.02\\
Wikipedia&Click fraud&118.18&0.04&116.65&9.66&75.66&145.88&0.72&120.79&21.91&109.86\\
Wikipedia&GET flood&117.90&0.04&116.38&10.08&76.51&140.62&0.66&119.14&24.29&121.10\\
Wikipedia&SHA1 cracker&115.47&0.05&115.00&9.57&74.81&135.24&0.74&118.96&22.11&111.52\\
\hline
Yelp&Benign&142.71&31.71&5.95&156.44&0.00&150.31&38.91&40.37&148.35&0.05\\
Yelp&Info Stealers&246.35&1.08&178.53&63.70&129.87&787.28&13.37&590.97&210.95&345.86\\
Yelp&Click fraud&186.80&0.78&137.90&48.21&100.56&891.92&4.39&504.53&183.96&296.34\\
Yelp&GET flood&190.54&0.76&136.63&48.37&105.58&671.18&4.27&465.84&168.69&319.15\\
Yelp&SHA1 cracker&169.80&0.69&126.89&43.68&94.08&681.62&3.90&484.41&163.90&288.38\\
\hline \\
\end{tabular}
\caption{Mean, $\mu$, and standard deviation, $\sigma$, of system call intensities per second per logical group of system calls.}
\end{table*}


==> experimental-setup/synthetic-malware-gen.tex <==
% Synthetic Malware Generation 
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/tables/synthetic_malware.pdf}\par
\caption{\textit{(Synthetic malware payloads used in our experiments: 4 info stealers, 2 networked nodes, and 1 compute node. The settings represent a small fraction, but computationally diverse, set of malware behaviors.}}
\label{fig:synthetic-malware}
\end{figure}
%After many unsuccessful attempts to run real malware in our experimental setup, we reimplemented malicious functionality in the form of synthetic malware and use it throughout the paper. Carefully crafted synthetic malware benchmark is designed to closely resemble real-world malware and to provide precise control over its parameters. Also, synthetic malware includes a futuristic feature not seen in the wild -- it can lower its intensity to remain unnoticed by local detectors.

%After in-depth analysis of hundreds of mobile malware samples in the wild, we
%have come up with a new methodology that is a few steps ahead of the current
%approach to evaluation of malware detectors -- this is the most crucial
%component of our experimental setup.

We evaluate our GD algorithms not against off-the-shelf malware
whose ,
but also against advanced malware that tries to escape detection by
diversifying its payloads' executions. We describe the scope of malware behaviors
and our process to construct a state-of-the-art malware sample that is
guaranteed to execute correctly.

%hiding behind the variations of benign executions.
%Instead of testing the \sysname against old malware, we have developed a
%We begin with an off-the-shelf malware sample -- Geinimi.a
%benchmark that extends existing malicious behaviors by including the new ones
%-- not seen in the wild -- in order to be more powerful in breaking the
%detection schema.

\noindent {\bf Limitations of off-the-shelf malware.} Most malware samples
available
online~\cite{dissect_malware_2012,contagiodump,malware.lu,virusshare.com} do
not execute correctly. This is because malware often require older, vulnerable
versions of Android OS; they are designed to run only in a specific
geographical location; they include anti-emulation
defenses~\cite{anti_emulation_android_vidas}; they passively wait for commands
from command and control (C\&C) servers that are temporarily or permanently
down; or are programmed to react to specific user actions.  Another challenge
of using off-the-shelf malware is that
%understand malicious behavior that stands behind 
malware code-names assigned by anti-virus (AV) companies -- like
\textit{CruseWin} and \textit{AngryBirds-LeNa.C} -- do not inform an analyst
what payload the malware actually executes. 

Hence we evaluate our detector against malware that we have reverse-engineered
and ensured to work correctly (on both the device and C\&C server sides); whose
payloads we understand in behavioral terms (such as stealing files or
Contacts); and whose payloads we actively diversify to stress our detector.

%Moreover, sticking to a handful of malware samples that are able to
%run in a lab environment is likely to introduce bias into the experimental
%results because such malware samples usually do not exhibit complex behavioral
%patterns due to being trivially simple.
%\mohit{rephrase, please}
%After in-depth analysis of hundreds of mobile malware samples in the wild, we have come up with a new methodology that is a few steps ahead of the current approach to evaluation of malware detectors -- this is the most crucial component of our experimental setup.
%
%We have performed rigorous evaluation of our system not only against existing malicious behaviors, but also against advanced malware trying to escape from the local detectors by hiding behind the variations of benign executions.  Instead of testing the \sysname against old malware, we have developed a benchmark that extends existing malicious behaviors by including the new ones -- not seen in the wild -- in order to be more powerful in breaking the detection schema.
%
%\noindent {\bf Off-the-shelf malware.}
%Plenty of malware samples available online~\cite{dissect_malware_2012,contagiodump,malware.lu,virusshare.com} do not execute 'properly'. Malware may require older, vulnerable versions of Android OS, run only in a specific geographical location, include anti-emulation defenses~\cite{anti_emulation_android_vidas}, passively wait for commands from command and control (C\&C) servers that are temporarily or permanently have been brought down, react to specific user actions. Moreover, sticking to a handful of malware samples that are able to run in a lab environment is likely to introduce bias into the experimental results because such malware samples usually do not exhibit complex behavioral patterns due to being trivially simple.

%The main issue with malware samples available online~\cite{dissect_malware_2012,contagiodump,malware.lu,virusshare.com} is that they often do not execute 'properly'. Malware may require older, vulnerable versions of Android OS, run only in a specific geographical location, include anti-emulation defenses~\cite{anti_emulation_android_vidas}, passively wait for commands from command and control (C\&C) servers that are temporarily or permanently have been brought down, react to specific user actions. Moreover, sticking to a handful of malware samples that are able to run in a lab environment is likely to skew the resulting data set because such malware samples usually do not perform complex actions, thus we would not be able to observe complex malicious behaviors.

Another challenge coming from the blind use of off-the-shelf malware is to understand malicious behavior that stands behind obfuscated malware names assigned by an anti-virus (AV) company. For example, malware names like \textit{CruseWin} and \textit{AngryBirds-LeNa.C} do not inform an analyst what an expected malicious behavior is. 
%they should expect from those samples. 
Finally, inconsistency between naming conventions used by different AV companies aggravates the problem.

\noindent {\bf Malware design pattern.}
When designing synthetic malware, we have applied client-server paradigm that is common across all real-world malware samples. Malware running on a device performs malicious actions in response to the commands that it receives from its C\&C server and communicates back to the server to confirm successful completion. Synthetic malware allows numerous network-related parameters to be fine-tuned: frequency of communication with C\&C, network bandwidth, the size of data packets sent by client side, interpacket delays between them, device-level intensity of malicious actions.

The client-side code is organized using delegation software design pattern together with Android message passing interface. When a client receives a notification from C\&C in the form of an xml file, it parses server's request, configures itself and launches one or more Android services responsible for carrying out a malicious task. Depending on C\&C's request, malware may run those services sequentially or concurrently. Some services act as an intermediate dispatcher -- they perform initialization and then spawn parallel threads to conduct actual malicious activity asynchronously. For example, the service performing click fraud activity creates a thread pool and supplies a list of URL links to the workers in the pool that they must access.

It is worth noting that most Android apps (both benign and malicious) are obfuscated using standard Android tool -- Proguard~\cite{proguard}. It renames classes, fields, and methods with obscure names. We have applied Progaurd to the synthetic malware as well.

\noindent {\bf Variety of malicious behaviors.}
As a starting point for modeling diversity of malicious behaviors, we have analyzed 229 malware samples in 126 families, which cover prevailing mobile malware over last three years, that we have downloaded from the public repositories~\cite{contagiodump,malware.lu,virusshare.com}. We have identified common malicious behaviors and trends and reimplemented them closely following design of a reverse-engineered Geinimi sample~\cite{geinimi}.

%\noindent {\bf Malware design pattern.}
%When designing our synthetic malware, we have applied client-server paradigm that is common across all real-world malware samples. Malware running on a device performs malicious actions in response to the commands that it receives from its C\&C server and communicates back to the server to confirm successful completion. Synthetic malware allows numerous network-related parameters to be fine-tuned: frequency of communication with C\&C, network bandwidth, the size of data packets sent by client side, interpacket delays between them, device-level intensity of malicious actions.
%
%The client-side code is organized using delegation software design pattern together with Android message passing interface. When a client receives a notification from C\&C in the form of an xml file, it parses server's request, configures itself and launches one or more Android services responsible for carrying out a malicious task. Depending on C\&C's request, malware may run those services sequentially or concurrently. Some services act as an intermediate dispatcher -- they perform initialization and then spawn parallel threads to conduct actual malicious activity asynchronously. For example, the service performing click fraud activity creates a thread pool and supplies a list of URL links to the workers in the pool that they must access.
%\input{experimental-setup/malware-table}%

At a high level, client-side malicious code can perform several independent tasks that fall into one of the three behavioral categories that we have found when analyzing real malware samples: information stealers, networked nodes, and compute nodes. C\&C server may instruct client-side code to execute any combination of these basic tasks. Their implementation is described later in this section.

\noindent {\bf Information stealers.}
Malware stealing personal information usually focuses on accessing the following data: contacts for spamming purposes, text messages for breaking two-factor authentication (e.g. bank trojans), location and files on device for spying on users, phone IDs for legitimizing stolen devices. Our synthetic malware can easily model all these behaviors.

Contact stealing service is mainly governed by two parameters: the number of contacts being exfiltrated and delay between sending queries to the contact provider. 

As for SMS stealing behavior, real malware samples come in two flavors: batch and intelligent stealers (e.g. bank trojans). The former transmit all the text messages to their C\&C server, while the latter register an Android listener to intercept incoming SMS messages and scan them for the presence of authentication codes, alternatively they can perform intelligent text search within the database of already received messages and upload to the C\&C server only interesting ones.

As mentioned earlier, for spying purposes malware frequently accesses location information and steal files from a device, mostly photos. Following Android programming model, synthetic malware can obtain location by registering an Android listener that receives location updates or directly from Android middleware. In the latter case, OS returns a previously cached location that may have been determined using cellular network (approximate mode) or GPS (precise mode) if it is available on a device.

Our malware supports all basic file operations: it can send directory content, upload a particular file or several files to the C\&C server or store a file received from a server on a device. The latter functionality is widely used by malware developers to install new (likely malicious) apps.

The last type of malware steals device IDs such as IMEI and IMSI codes, OS info available via the static class android.os.Build and other miscellaneous device specific data such as browsing history and bookmarks, description of installed apps, call logs. Generally this information -- especially IMEI and IMSI -- can be used for impersonating purposes, in particular, to legitimize stolen devices before selling them on a black market, or for targeted advertising.

Our implementation of these functional blocks allows to specify the following parameters: amount of data being read (e.g. 1 or 10 contacts/SMSs/files), intensity of data accessing operations (e.g. read a file by 1K chunks), delay between successive reading operations (e.g. sleep for 100 ms between retrieving subsequent contacts/SMSs).

\noindent {\bf Networked nodes.}
The other behavioral malware category -- networked nodes -- includes mobile malware that exploits phone's network resources. It is getting more and more widespread as network bandwidth keeps rising up. Malware developers are lured by frequently changing device's IP and the ease of distributing malicious activity across many network nodes (devices) that are unlikely to be blacklisted. 

We have identified two types of an abuse of phone's network capabilities: click fraud and DDoS attacks~\cite{malware_blackhat_15, prolexic_q4_2013, android_ddos_2012}. Click fraud is one of the most popular ways of generating revenue out of having access to compromised hosts. Malicious service receives a list of URLs from a C\&C, periodically fetches webpages specified in the URL list and traverses their DOM structure. To speed up the process, our malware may launch several parallel threads.

The other type -- DDoS attacks from compromised mobile devices -- are getting more popular. Vast majority of DDoS attacks abuse HTTP protocol (e.g. 80\% according to \cite{ddos_threat_spectrum_2012}). Our malware is able to mount two attacks: GET flood and SlowLoris~\cite{slowloris_ddos}. GET flood comprises a series of GET requests sent by compromised network nodes. As opposed to GET flood, SlowLoris attack is far less computationally expensive because it tries to exhaust server pool of available connections by opening numerous connections and sending data very slowly to keep connections alive over a long time period. In our experiments, synthetic malware establishes 500 connections. If some connections fail, they are automatically reopened to keep the total number of active connections constant.

\noindent {\bf Compute nodes.}
The last category of malicious behaviors includes computationally intensive malware. Unlike the previous two, it may or may not leave distinguishable fingerprint at system call interface. A typical example of such malware is a bitcoin miner \cite{mobile-bitcoin-miner}. We approximate this category by the code cracking SHA1 passwords.

\noindent {\bf Realistic user data.}
In addition to careful modeling of malicious behaviors, we have invested a lot of efforts into populating our emulators with synthetic data that is statistically close to the real user data. For these purposes, we have followed the guidelines from the following empirical study~\cite{morpheus-hasp}. Without user data even a perfectly working malware may not perform anything malicious if, for example, it is designed to steal  data (e.g. photos, contacts, text messages and etc).

\noindent {\bf Repackaging Android apps.}
We have embedded synthetic malware into benign underlying apps using the same methods as malware developers: disassembled an apk using \textit{apktool}, copied malicious code into the apk, modified \textit{Manifest.xml} to extend the list of required permissions and to statically register malicious components. Finally, we have reassembled the decompiled app with \textit{apktool} and signed with \textit{jarsigner}.

\noindent {\bf Check for correctness.}
One of the key design decisions that we have made is to augment malware with capability to  notify data collection system when certain events happen (e.g. C\&C request has been successfully parsed, malware starts/finishes execution). This is very important because android emulators often crash, thus we can identify and rerun failed experiments. We also use malware start and stop time stamps to start and stop collecting malicious feature vectors.  We also make sure that the notification mechanism does not pollute the collected data.

\mikhail{we need a table with malware parameters + one paragraph to describe them}





==> intro/behavioral-analysis.tex <==
% Behavioral Analysis
\subsection{Behavioral Analysis}

\comment{

* Crowdroid Anomaly Detector
* Andromaly Anomaly Detector
* pBMDS: Anomaly Detector
* Behavioral Detection of Malware on Mobile Handsets: Anomaly Detector
* SmartSiren: Anomaly Detector: CIDS: network based
* Monitoring Smartphones for Anomaly Detection: Symbian: Features sent to remote server: Features == amount of free RAM, user inactivity, number of running processes, CPU utilization, SMS sent count

* A Layered Architecture for Detecting Malicious Behaviors: Behavioral Signature mining
* Synthesizing Near-Optimal Malware Specifications from Suspicious Behaviors: Behavioral Signature Mining
* Automated Classification and Analysis of Internet Malware: Behavioral Signature Mining

Anomaly Detection
Power based

In \cite{Schmidt2008}, Schmidt et al proposed an anomaly detection system based on Symbian. Due to mobile phone requirements, the authors sent the feature vectors to a remote server for processing. The features included amount of free RAM, a user inactive boolean, the number of running processes, the current CPU utilization, and the number of sent SMS messages.  

% Early Work
In \cite{Jacoby2004} authors monitored instantaneous current of a battery


Anomalous behavior detection systems attempt to statistically distinguish malicious activity from \emph{normal} benign execution. Once trained, behavioral classification engines determine whether a given feature vector is benign or suspicious, and emits a label accordingly. This implies that the feature set captures some abstract notion of program execution. For example, a commonly chosen, and relatively low level, feature is the system call trace\todo{DO THE LIST CITATIONS HERE}. System calls are provided by the OS and enable general programs to request OS services (open/close files, process management, etc.). For instance, Crowdroid, an early Android CIDS, treated system calls as a bag of words where each feature vector is simply a system call histogram per appli.   

Dynamic behavioral analysis techniques monitor program execution... 

Signals
System Calls + w params / API Calls \cite{Wagner:2002:MAH:586110.586145,Christodorescu:2008:MSM:1342211.1342215,kruegel2007,Fredrikson2010,Canali2012,Burguera2011,Kolbitsch:2009:EEM:1855768.1855790,Xie2010, rieck2008} 
Network Info \cite{Cheng2007,Roesch1999,staniford-chen1996,porras1997}
Battery/CPU\cite{Schmidt2008}/MEM\cite{Schmidt2008}/etc \cite{Buennemeyer2008,Jacoby2004,Kim2008}
Power\cite{clark2013}

Features:
N-Grams \cite{Gu2008,Canali2012}
Tuple \cite{Shabtai2012,Canali2012}
Bag \cite{Burguera2011,Canali2012, rieck2008}
Graph (Probably Dependency Graph or Approx) \cite{Christodorescu:2008:MSM:1342211.1342215,Kolbitsch:2009:EEM:1855768.1855790,Lippmann2008,Xie2010,kruegel2007}

Algorithms:
Histogram Comparison: \cite{Shabtai2012}
Classification (SVM, Clustering, etc) 
- kMeans: \cite{Burguera2011,Shabtai2012}
- kNN: \cite{Demme2013}
- ANN: \cite{Demme2013}
- SVM: \cite{rieck2008}
- Logistic Regression \cite{Shabtai2012}
- Decision Trees + Bayesian Networks \cite{Shabtai2012,Demme2013} 
HMMs \cite{Xie2010}
Graph Comparison \cite{Lippmann2008,kruegel2007}
Results

\begin{itemize}
% Classification (SVM, Clustering, etc) 
\item kMeans: \cite{Burguera2011,Shabtai2012}
\item kNN: \cite{Demme2013}
\item ANN: \cite{Demme2013}
\item SVM: \cite{rieck2008}
\item Logistic Regression \cite{Shabtai2012}
\item Decision Trees + Bayesian Networks \cite{Shabtai2012,Demme2013} 
\end{itemize}
}


Behavioral analysis refers to statistical methods that monitor signals from
program execution, extract features and build models from these signals, and
then use these models to classify processes as malicious.  Importantly, as we
discuss in this section, all known behavioral detectors have a high false
positive and negative rate (especially when zero-day and mimicry
attacks are factored in). 

%such as system calls, network traffic, instruction-level
%behavior etc, 

% System calls and parameters have been studied extensively
%Signals for behavioral analysis include
System-calls and middleware API calls have been studied extensively 
as a signal 
%are very commonly used signals 
for behavioral detectors~\cite{Wagner2002,Christodorescu:2008:MSM:1342211.1342215,kruegel2007,Fredrikson2010,Canali2012,Burguera2011,Kolbitsch:2009:EEM:1855768.1855790,Xie2010,
rieck2008,bose2008,Mutz2006,Forrest1996,Hofmeyr1998,Warrender1999,Somayaji2000}.
%Specifically for Android, Crowdroid\cite{Burguera2011} 
%uses system call traces sourced from
%several devices as the sole signal in its anomaly detection.  
Network intrusion 
detection systems like Snort, Bro~\cite{paxson1999}
HIDE~\cite{zhang2001}, EMERALD~\cite{porras1997}, BotSniffer~\cite{Gu2008}, and 
NetBiotic \cite{vlachos2004} analyze network traffic to detect known malicious
or anomalous behaviors.
More recently, behavioral detectors use signals such as power
consumption\cite{clark2013,Buennemeyer2008,Kim2008}, CPU
utilization\cite{Schmidt2008}, memory footprint\cite{Schmidt2008}, and hardware
performance counters\cite{Demme2013,Tang2014}. Specifically on 
Android, Andromaly\cite{Shabtai2012}
uses power consumption and CPU utilization, in addition to syscalls,
network flow, and control flow, as signals that are
tracked at runtime.


%Features go Here Rather than just saying whats popular, lets talk about how
%these features are useful in the statistical model building process Up the
%citation count
Detectors then extract {\em features} from these raw signals.  For example, an
n-gram is a contiguous sequence of n items that 
%is useful for their simplicity and their ability to 
captures total order relations~\cite{Gu2008,Canali2012}, n-tuples are ordered
events that do not require contiguity, and bags are simply histograms.
%Note, the dimensionality of the feature space is directly proportional to the
%value of n, however this comes at the expense of increased complexity and
%memory requirements. Dimensionality these features to compress the feature
%space into a smaller form that remains representative.  N-tuples are a strict
%relational ordering of n-grams, without requiring contiguity. n-tuples are
%useful in non-trivial combinations of
These can be combined to create bags of tuples, tuples of bags, and tuples of
n-grams~\cite{Shabtai2012,Canali2012,Forrest1996,Hofmeyr1998,Warrender1999}
often using principal component analysis to reduce dimensions.
%Bags are simply an unordered count of their contents. For example, bags may
%contain n-grams, tuples, or simply the original signal. Bags are useful
%because they describe the data in terms of its frequency
%distribution~\cite{Canali2012}. %Notable examples To reduce dimensions,
%analysts uses techniques such as include~\cite{Burguera2011,Canali2012,
%rieck2008,Warrender1999}. Rieck et al.~\cite{rieck2008} proposed a framework
%for automatically classifying malware samples into groups with similar
%behaviors.  
Further, system calls with their arguments form a dependency graph structure 
%spatio-temporal relations among features.  As~\cite{Canali2012} pointed out,
%complex combinations of N-grams, Tuples, and Bags can approximate these
%graphs. However, there are algorithms from graph
that can be compared to sub-graphs that represent malicious
behaviors~\cite{Christodorescu:2008:MSM:1342211.1342215,Kolbitsch:2009:EEM:1855768.1855790,Lippmann2008,Xie2010,kruegel2007}.
%theory that are useful for comparing graphs and subgraphs



% Anomaly start by listing overlapping methods Talk about hardware performance
% counters in the signals section
%Anomaly detection research use many different algorithms to extract alerts
%from
Finally, detectors train models to classify executions into malware/benignware
using supervised (signature-based) or unsupervised (anomaly-based) learning.
These models range from distance metrics~\cite{Forrest1996, Hofmeyr1998}, histogram
comparison~\cite{Kind2009}, hidden markov
models(HMM)~\cite{Xie2010,Warrender1999}, and neural networks (artificial neural
networks, fuzzy neural networks, etc. )~\cite{Demme2013,Wei2014}, to 
more common classifiers such as
%classification 
kNN\cite{Demme2013}, one-class SVMs~\cite{Tang2014},
decision trees\cite{Demme2013}, and ensembles thereof. 
%Andromaly evaluates histogram comparison, k-Means, logistic regression,
%decision trees, and baysian networks algorithms for its anomaly detection. 
\ignore{
pBMDS\cite{Xie2010} use HMMs to correlate
%probabilistic approach to anomaly detection by 
user inputs with system calls, whereas Xu et al.~\cite{Xu2004} apply sequence
alignment techniques to known and unknown malicious binaries to detect
polymorphic strains.
}

%Results
%Mobile platforms face resource limitations not evident in their PC
%counterparts. Although smartphones have become more powerful in recent years,
%minimizing analysis and detection overheads is still a top priority. Host-based

Such machine learning models, however, result in high false positives and
negatives.  
Anomaly detectors can be circumvented by mimicry attacks where
malware mimics system-calls of benign applications~\cite{Wagner2002} or
hides within the diversity of benign network traffic\cite{Sommer2010}.
Sommer et al.~\cite{Sommer2010} additionally highlights 
several problems that can arise due
to overfitting a model to a non-representative training set, suggesting signature-based
detectors as the primary choice for real deployments. Unfortunately, 
signature-based detectors cannot detect new (zero-day) attacks.
%show how mimicry attacks can circumvent system-call based detectors.
%Similarly, 
Specific to Android, both system
calls~\cite{Burguera2011} and hardware-counter based
detectors~\cite{Demme2013} 
%results for hardware performance counters to detect
yield $\sim$20\% false positives and $\sim$80\% true positives.

Our work {\em assumes} that each individual {\em local detector} (LD) is weak
and presents (a) a new property -- the different shapes of true- and
false-positive feature vectors -- and (b) a new censorship algorithm to
concentrate the weak signal in LDs' outputs.

%Our work can use any of the above detectors as {\em local detectors} (LDs)
%and 

%demonstrate that network traffic models are not robust to benign variations --
%leading to high false positives and `real' deployments working only with
%signature based detectors. 

%Intrusion detection systems such as Andromaly have managed to keep processing
%overheads at around 10\% with reasonable detection rates; Best case detection
%rates for Andromaly changed per experiment with TP/FP rates ranging from
%99.9\%/0.00\% to 85.3\%/16.2\%. Note, however, the Andromaly experiments use a
%few simple custom-written Android malware since no known Android malware
%existed. Alternatively, systems like Crowdroid choose to extract system call
%features locally, which is a lightweight task, and perform analysis in the
%cloud. The server computes a bag of system calls per execution trace and
%distinguishes malicious activity from benign activity using 2 cluster k-Means.
%The authors evaluate Crowdroid with a combination of 3 in-house apps and real
%malware samples; namely the Steamy Window app with PJApps Malware and Monkey
%Jump 2 with HongTouTou Malware. Given 60 execution traces per app, 50 benign
%and 10 malicious, the Crowdroid engine achieved 100\% TP and 0\% FP rates for
%all apps except Monkey Jump 2 which achieved 85\% detection with 3 false
%positives. The contrast between PJApps and HongTouTou detection rates is a
%byproduct of their intended malicious activities. PJApps launches a background
%application with many functions whereas HongTouTou just browses web pages and
%leaks phone information to a remote entity. In a sense, HongTouTou is stealthy
%compared to PJApps strains.        
        


%Discussion
%Talk about intended activity of malware and how this relates to intelligent malware. Talk about how sufficient data is needed to prevent overfitting in data mining pipeline.



==> intro/cids.tex <==
\subsection{Collaborative Intrusion Detection Systems (CIDS)}
\label{sec:cids}

% Can You infect me now?
% Malware Propagation in Large Scale Networks
% Smartphone Malware and Its Propagation Models: A Survey
% Modeling Malware Propagation in Smartphone Social Networks
% Why mobile-to-mobile Malware wont cause a storm
% BIG: Modeling and Restraining Mobile Virus Propagation


%Intrusion detection systems (IDS) monitor local or network operations for
%suspicious activities. 
Collaborative intrusion detection systems (CIDS) provide an architecture where
LDs' alerts are aggregated by a {\em global detector} (GD).
%correlate information across many per-device local detectors of these
%intrusion \emph{monitors}, improving the detection of intelligent local
%attacks. In particular, local detectors emit a stream of alerts and network
%overlays allow the system to determine neighborhoods.  The global detector
%takes the local detector streams and the neighborhoods from the network
%overlays and correlates the local detectors' alerts, considering only a
%neighborhood at a time.  Local Detector
GDs can use either signature-based\cite{kannadiga2005, snapp1991, cuppens2002,
yegneswaran2004, ramachandran2004, duma2006},
anomaly-based\cite{zhang2001,staniford-chen1996,vlachos2004}, or a combination
of the two~\cite{porras1997,krugel2001,paxson1999} to generate global alerts.
%Signature-based detectors are similar to malware detectors in that ther are
%unable to address unknown attacks. Anomaly detectors, however, are able to
%handle unknown attacks but usually suffer from a high false positive rate.
%Simple local detectors such as those in DIDS\cite{snapp1991} and
%DIDMA\cite{kannadiga2005} throw labeled flags for all suspicious activity
%(e.g. failed login attempts, modification of system files, telnet usage,
%rlogin usage, etc.). On the other hand, systems like HIDE\cite{zhang2001} emit
%statistical alerts in the form of random variables.
Additionally, the CIDS architecture can be centralized~\cite{porras1997},
hierarchical~\cite{zhang2001}, or distributed (using a peer-to-peer overlay
network)~\cite{yegneswaran2004,ramachandran2004,vlachos2004,duma2006,ZhouCV2005}.

%% Network Overlays
%\ignore{
%CIDSs use network overlays to determine inclusion or non-inclusion of specific
%nodes in the correlation analysis. Therefore, the networks are defined
%\emph{virtually} as a set of nodes logically connected via edges, for example a
%virtual graph may be constructed from the edges of a social network of friends
%and an email contact graph.
%}
%
%\ignore{
%The HIDE\cite{zhang2001} system assigns static network overlays
%hierarchically based on network locality. Global detectors in HIDE monitor machines on
%their local area network for suspicious activity and generate statistical
%reports based on their findings. These summaries are forwarded to, and aggregated
%at a global detector in the next level of the hierarchy. Note that this global
%detector is also monitoring its \emph{local} network for suspicious activity.
%
%Distributed CIDSs, which have neither a central processing component nor a strict
%hierarchical ordering, use network overlays to locate a neighborhood of nearby
%peers for alert correlation.
% Oftentimes, this mapping takes form as P2P
%networks~\cite{yegneswaran2004,ramachandran2004,vlachos2004,duma2006}.
%INDRA\cite{Janakiraman2003} uses a distributed hash table for organizing their
%global detectors in its P2P network overlays. In the LarSID
%system\cite{ZhouCV2005}, nodes \emph{subscribe} to network overlays, where they
%\emph{publish} suspicious findings. Therefore, all nodes serve as both local and
%global detectors.
%}


%Global detectors act as \emph{correlation engines} for a neighborhood of local
%detectors. One common paradigm for global detectors 

In all cases, existing GDs use some variant of count-based algorithms to
aggregate LDs' alerts \cite{Dash2006,Seurat2004}: once the number of alerts
exceeds a threshold within a space-time window, the GD raises an intrusion
alert. In HIDE~\cite{zhang2001}, 
%uses a multi-tiered system where 
the global detector at each hierarchical-tier is a neural network trained on
network traffic information.  Worminator\cite{Locasto2005} additionally uses
bloom filters to compact LDs' outputs and schedules LDs to form groups in order
to spread alert information quickly through a distributed system.  
All count based algorithms are fragile when the noise is high (in the early 
stages of an infection) and when the network size is uncertain.
%Our GD uses shape information and dynamically censors the output
In contrast, our shape and censoring based GD is robust against 
such uncertainty.

%We focus on early stage detection of zero-day infections and on
%aggregating alerts in 
%a network where the membership information is unreliable. 

Note that distributed CIDSs are vulnerable to probe-response attacks, where the
attacker probes the network to find the location and defensive capabilities of
an LD~\cite{Shmatikov2007,Bethencourt2005,Shinoda2005}. These attacks are orthogonal to our
setting since we do not have fixed LDs (i.e. all nodes act as LDs). 
 
%and generate global
%a network scheduling approach, implemented as
%a bloom filter, 
%to ensure that neighboring nodes with access to complementary
%pieces of information can communicate at approximately the same time.  
%This
%allows the system to determine if a local alert is simply noise or part of a
%distributed alert.


==> intro/global-d.tex <==
\subsection{Global Detectors}

\noindent \textbf{Count:} {\em Count} refers to the simple yet natural
idea that the number of alerts when there truly is a new malware in
the community differs from the baseline number of alerts. As our
results show, count provides statistical separation, but {\em only
  once the malware spread becomes large enough}; in the early stages,
the number of true alerts is drowned in the (comparatively) vast
number of false positive alerts. Thus, for early stage detection, we
seek something more powerful than count alone.

% For example, if the false positive rate is
% $0.3,$ and the true positive rate is $0.7,$

% To illustrate these, consider for concreteness, a
% community of 1000 nodes connected according to a typical social graph
% \cite{}. Assume that the local detectors at the individual nodes have
% false positive (misclassifies benign as malware) and false negative
% (misclassifies malware as benign) rates of $0.3.$

% \noindent \textbf{Count:} Count simply means that that number of
% alerts when there truly a malware in the community differs from the
% baseline count. Indeed, in our example, due to false positives, even
% when thereis no malware in the network, we expect $300 \pm 43$ (for
% $3 \sigma$ confidence). On the other hand, suppose that 10\% of the
% community had malware (a significant fraction), we would expect
% about $400 \pm 45$ alerts, which statistically separates from the
% benign baseline count. 

% However, if there is noise in the community
% structure knowledge or the local detector is more noisy, the fraction
% of nodes that need to have malware can easily rise to 20 - 25 \%,
% which in practice is huge (and thus, not very useful). Thus, count
% alone is of marginal utility if we want to detect malware in its early
% stages.

\noindent \textbf{Space-time Geometry:} The {\em location of alerts}
on the graph is informative -- it is clear that if we observe 100
alerts randomly spread out over the network, then there is not much
cause of worry (likely false positives). However, if we see 100 alerts
all of which are clustered within a few hops of each other (spatial
geometry), then this is much more indicative of a true
malware. Similarly if we first observe an alert at a single node, a
short time later we observe alerts at several of its neighbors, and a
further short time later alerts from their neighbors. This is
evocative of a malware spread (temporal correlation with graph
structure), despite the fact that the total number (count) of alerts
is still very low (and below the false positive uncertainty
threshold).

% Thus, the
% hypothesis testing engine needs to formally incorporate not just
% counts, but also graph space-geometry when making inferences.

\noindent \textbf{Shape of the Distribution:} The third, and perhaps
most subtle effect, is that looking at the {\em inputs to the local
  detectors that send an alert} is informative. That is, instead of
simply counting alerts, {\em we need to exploit the actual
  feature-vectors generating the alerts} (these are eigenvalues if the
feature extraction from the OS trace is based on PCA
\cite{jolliffe2002principal,hearst1998support,scholkopf1998support}). Indeed,
from an information theoretic perspective, this is the right thing to
do because the entropy at the input (feature vector space) to the
(noisy) local detector is greater than that at its output (binary
space).


==> intro/malware-class.tex <==
\subsection{Identifying Malware Classes}


\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.5\textwidth]{synthetic-malware.pdf}
\caption{
Modeling adaptive malware. We 
synthesize
4 information stealers, 2 networked nodes, and 1 compute node, 
in addition to
%The settings represent a small fraction but computationally diverse set of malware behaviors. 
%We also repackage
4 existing malware -- Geinimi, Roidsec, click fraud, and md5 cracker. 
All synthesized malware include the best known obfuscation and 
evasion techniques.
%and use Geinimi which comes repackaged into the MonkeyJump game.
%*Most, but not all, of the workload requires only 100ms.
}
\label{fig:synthetic-malware}
\end{figure}



==> intro/malware-detection.tex <==
\subsubsection{Malware Detection}
\comment{They look at A,B, C on alpha, beta, gamma using blah and saw this. And here is the take away}


Quantitative Study of Accuracy in System Call-Based Malware detection
comparing relative strength of the behavioral detectors
Look at atoms (system calls, syscalls w args, actions (bag of syscalls), actions w args) combined into structures (ngrams, tuples, and bags)
Large scale empirical analysis: approximately 7200 malware samples + 36 benign applications  


Crowdroid:
Analyze the behavior of android applications, providing framework to distinguish between applications that, having the same name and version, behave differently. The aim is to detect anomalously behaving applications. Main contribution is use of crowd sourcing system to obtain system call traces. detected all self written malware with 100\% detection rate. NOTE: IN RELATED WORK Schmidt et al. proposed a solution based on monitoring events occuring on Linux-kernel level. They reviewed Linux based tools for enhancing security, and extracting features such as system calls, modified files, etc. Security tools and mechanisms used in computers are not feasible for applying on smartphones due to the excessive resource consumption and battery depletion. Hence, authors perform whole analysis process on a dedicated remote server. Crowdroid client downloaded from Google app store. Crowdroid monitors syscalls, preprocesses them, and sends them to the centralized server. Server extracts syscall histogram for each execution of each app on a device. Use two cluster k-means as the classifier? Three baseline apps (calculator, countdown, and money converter) written and modified to include malware (NOT SPECIFIED WHAT THIS MALWARE DOES). 60 execution traces collected: 50 Benign + 10 malicious per app. Also tested on Steamy Window + PJApps Malware (100\% detection) and Monkey Jump 2 + HongTouTou Malware (85\% Detection / 3 False Positives). The reason for obtaining a worse detection rate on monkey jump 2 is the simpler nature of the actions performed by the malware. HongTouTou sends information and browses internet while PJApps starts a background application and has more functions programmed. 



A survey on automated dynamic malware-analysis techniques and tools:

Automatic analysis of malware can be performed in two ways. Dynamic analysis refers to techniques that executes a sample and verify the actions this sample performs in practice, while static analysis performs its task without actually executing the sample. The inability to detect unknown threats is an inherent problem of signature based detection techniques. EXTREMELY LONG PAPER, WILL CONTINUE LATER


Andromaly:
Generic and modular framework for detecting malware on Android devices. Host Based. Accomplished by continuously monitoring mobile devices to detect suspicious/abnormal activities using a supervised anomaly detection technique. Light weight application monitors the device for CPU utilization, number of packets sent over Wi-Fi, number of running processes, battery level, average touch pressure, etc. After collection and preprocessing, the system metrics are sent for analysis by various detection units, namely processors, each employing its own expertise to detect malicious behaviour and generate a threat assessment (TA) accordingly. the pending TAs are weighted to produce an integrated alert. The weighting process is per threat type (worms, torgans, etc all have different weights). Weighting process includes a smoothing phase to avoid instantaneous false alarms. Evaluated k-Means, Logistic Regression, Histograms, Decision Tree, Bayesian Networks, and Naive Bayes as classifiers. (MICHAEL NOTE, WTF only a few of these are true classifiers). Used the filter approach for feature selection due to its fast execution time and generalization ability. Under the Filter approach, an objective function evaluates features by their information content and estimates their expected contribution to the classification task. Three feature selection methods were applied: Chi-square, Fisher Score, Information Gain. All 3 follow the Feature Ranking approach. Ranked 88 different features. Developed 4 malicious applications that perform DoS attacks and information theft attacks. First, a Tip Calculator malicious application to unobtrusively perform a DoS attack. When a user clicks the calculate button, the application starts a background service that waits for some time then launches several hundereds of CPU-consuming threads. Schedule SMS, an app to send delayed SMS messages to people. in addition to these malicious apps, 20 benign games and 20 benign tool apps were used. 10\% Overhead when running malware detector at 5s sampling intervals. Best case results changed per experiment with TP/FP ranging from 0.999/0.00 to 0.853/0.162. At time of experiment, no known android malware existed. Second limitation is in small variety of malware applications used.


A Layered Architecture for Detecting Malicious Behaviors:
Build representations of these high-level actions (For example bot actions include proxying, keystroke logging, data leaking, and program download and execute) hierachically, taking care to identify only the essential components of each action. Lowest level even in behavioral specifications are system call invocations. The difference between the low level events and the high level aggregate effect of those events is reffered to as the \emph{semantic gap}. Contributions include a behavior-specification language, a detector for high level actions including distinguishing malicious execution of high-level behaviors from benign. A behavior graph is a directed graph of the form that is adapted from and extends AND/OR graphs. A behavior graph may have AND-edge set and OR-edge sets specifying requirements for actions. Annilhilator nodes are used to represent the destruction of an object or event. replicators duplicate objects. All graphs in this paper were developed manually and iteratively through domain knowledge. Implemented on Qemu emulators. Tainting overhead is 7x-23x wall clock.


Synthesizing Near-Optimal Malware Specifications from Suspicious Behaviors:
This technique, based on graph mining and concept analysis, scales to large classes of programs due to probabilistic sampling of the specification space. HOLMES can synthesize discriminative specifications that accurately distinguish between programs, sustaining an 86\% detection rate on new, unknown malware, with 0 false positives. Behavior based techniques are promising because it is harder for an attacker to radically change the behavior of a malware than to morph its syntactic structure. Constructing behavioral specifications that have a low false positive rate and at the same time are general enough to detect variants of malware is a major challenge. An automatic technique for building these specifications is desirable, both to reduce the AV vendors' response time to new threats and to guarantee precise behavioral specifications. Given a set of \emph{behavior graphs} that describe the semantics exhibited by malicious and benign applications, the graph mining operation extracts \emph{significant behaviors} that can be used to distinguish the malware from the benignware. Wish to find a set of behavioral specifications that describe a given set of programs (the positive set) but not any program  in the second set (the negative set). The first step of the behavior mining algorithm extracts the portions of the dependence graphs of programs from the positive set that correspond to behavior that is significant to the programs intent. I.e. find the subgraphs that give the maximum contrast between the positive and negative sets. (Note mining algorithm determines the notion of significance). Discriminative specification algorithm can guarantee that specifications are optimal with respect to the true and false positive rates over a target sample distribution. Use simulated annealing, probabilistic sampling technique, to efficiently search for a subset of clusters that can be used to construct a close approximation to the optimal specification. Used real Windows malware samples and ran in Qemu. Real world benign apps (putty, FileZilla, Skype, Visual Studio, etc). Able to detect unknown malware with 86.56 percent TP and 0 percent FP. Issue: Can take a while to extract behaviors and these dependence graphs can be big. 


pBMDS: A Behavior-based Malware Detection System for Cellphone Devices:

pBMDS adopts probabilistic approach to malware detection by correlating user inputs with system calls to detect anomalous activities. Leverages HMMS to learn application and user behaviours from two major aspects: process state transitions and user operational patterns. Consider malware such as Commwarrior adopting MMS/SMS and/or Bluetooth as its major infection vector, scanning contacts, randomly choosing some contacts and sending malicious messages to these new victims. Authors assume that malware always launch attacks from the application software (i.e. cannot break the kernel). Once a process deviates from its expected normal behavior(reflected through GUI interactions) to a certain degree, it is considered suspicious and teh access to the system resources should be denied. After learning the user operational patterns and the state transition rules, the engine encodes the learning result by hashing it to the kernel, where it can be safely saved as a user profile. To test whether a running process is malware or a compromised by malware, the run-time detection engine authenticates at key system call points. Runs on Qtopia, a linux based smart phone. After sanitizing the user inputs the next step is to generate a behavior graph which reflects the intermediate process states towards each key system call.


Automated Classification and Analysis of Internet Malware:
The signatures used by IDS and AV often focus on a specific exploit behavior, an approach increasingly complicated by the emergence of multi-vector attacks. As a result, IDS and AV products characterize malware in ways that are incosistent across products, incomplete across malware, and that fail to be consise in their semantics. The reduced collection of user visible system state changes (files r/w, processes created) in a virtualized enviornment is used to create a fingerprint of the malware's behavior. AV systems rarely use dhte exact same labels for a threat, and users of these systems have come to expect simple naming differences. Three key design goals of a label ing system, Consistency, Completeness, and Conciseness. Existing AV solutions fail to meet these metrics. To address these limitations, the authors propose an approach based on the actual execution of the malware samples and observation of their persistent state chagens. Individual system calls may be at a level that is too low for abstacting semantically meaningful information: a higher level abstraction is needed to effectively describe the behavior of malware. State changes are at a higher level than individual syscalls and the avoid many common obfuscation techniques that foil static analysis and low-level signatures. Authors approach to generating meaningful labels is achieved through clustering of the behavioral fingerprints. Initial naive approach to defining similarity was based on the concept of edit distance. Two drawbacks to this approach, it overemphasizes size and behavioral polymorphism (e.g random file names). Instead used normalized compression distance. To combine various pieces of malware based on their similarity, authors constuct a tree structure based on the well-known hierachical clustering algorithm. To extract meaningful groups, the authors adopt an \emph{inconsitency} measure that computes the difference in magnitude between distances of clusters so the tree can be cut into distinct clusters. Evaluate on large and small datasets taken from 2006-2007 including 3698 and 893 unique MD5s respectively. Algorithm created 403 clusters from the 3698 individual malware.  


A Semantics-Based approach to malware detection:
This paper takes the position that the key to malware identification lies in their semantics. It proposes a semantics based framework for reasoning about malware detectors and proving properties such as soundness and completeness of these detectors. Goal of this paper is to provide a formal semantics-based framework that can be used by security researchers to reason about and evaluate the resilience of malware detectors to various kinds of obfuscation transformations. 


DroidMat: Android Malware Detection through Manifest and API Calls Tracing: LOOK AT THEIR RELATED WORK SECTION
Authors propose a static feature-based Android malware detector. Static information includes permissions, deployment of components, Intent messages passing and API calls for characterizing the android applications behavior. Uses k-Means to enhance the malware modeling capability and uses SVD on the low rank approx to determine the number of clusters. Finally, uses kNN algorithm to classify the app as benign or malicious. Dyanamic features often used in literature include logged behavior sequences, system calls, tainting and control flow, and power consumption. Static features used in literature include requested permissions, imported package, API calls, instruction (opcode), data flow, and control flow. Use k-Means and EM in functional behavior recognition. Use spectral analysis to find top singular values covering 95\% of spectral energy. 238 malware samples from 34 malware families collected from Contagio mobile. 50 Benign applications from 30 categories on the Google Play store verified benign using VirusTotal. Accuracy is 97\% with 87\% Recall rate and 96\% Precision.


Semantics Aware Malware Detection:


 Static Analysis?
Authors propose RiskRanker, a scalable automated system to analyze wheter a particular app exhibits dangerous behavior (e.g. launching a rot exploit or sending background SMS). Able to examine 118,318 apps from various Android markets in less than 4 days. Of these, successfully uncovered 718 malware samples in 29 families; 322 of which are zero-day (in 11 families). This is a proactive scheme to spot zero-day Android malware by scalably and accurately sifiting through a large number of untrusted apps without relying on malware specimin. Divide potential risk into high-risk, medium-risk, and low-risk. High risk apps can compromise the phone integrity without authorization, medium risk apps do not exploit software vulnerabilities but can cause users finacial loss/disclose sensitive info. low risk apps may collect device specific, or generic, readily available personal info. For high risk, first scan apps for native code, those with native code are scanned for vulnerability signatures. For medium risk, use symbolic execution to determine which callbacks result in a call to a method of interest. Our first-order analysis modules are mainly designed to handle non-obfuscated apps and may fall short for stealthy malware that intensively encrypts or dynamically changes its payload. To mitigate these weaknesses, we accordingly develop second-order analysis modules to collect and corre-
late various signs or patterns of behavior common among malware yet not among legitimate apps. To evaluate false negatives, authors downloaded 12 malware samples from contagio dump to use as ground truth. System fails to detect social engineering attacks like FakeNetflix. Also fails to detect BatteryDoctor, Gone60, and TapSnake spyware that collect personal info. Also failed to detect ADRD click fraud app. The second reason for failure is taht missed samples do not share the same walicious payload as others in the same family. Finally, some apps are missed because they are guilty by association (e.g. droppers).  


Behavioral Detection of Malware on Mobile Handsets:

Novel behavioral based detector where normal behavior learned from classifier based on SVMs. Also find that the time and resource overheads of constructing the behavior signatures from low level api calls are acceptably low for their deployment on mobile devices. At the time able to detect current mobile viruses and worms with 96\% accuracy. Run on Symbian OS using malware strains gathered from 25 distinct families. Authors reconstruct higher level behavior signatures from lower level API calls. Train SVMs with both normal and malicious behaviors so that partial signatures for malicious behavior can be classified correctly. Behavior signatures are best specified using temporal logic instead of classical propositional logic. Monitor a subset of symbian API calls using temporal logic of causal knowledge (temporal logic TLCK). Authors manually generated propositional variables and TLCK operators to create the behavior signatures for each family. Plan on exploring automated feature extraction methods. Construct the behavior signatures of a program at runtime by generating, pruning, and aggregating, dependency graphs. Use Gaussian radial basis as kernel method in SVM.

% http://ieeexplore.ieee.org/xpls/abs_all.jsp?arnumber=6170530&tag=1

==> intro/malware-propagation.tex <==
% Malware propagation
\subsection{Network Malware Propagation}
\label{sec:malware-prop}

% \comment{
% Spatial-Temporal Modeling of Malware Propagation in Networks:

% Due to huge potential damages that may be caused by malware, researchers have proposed many models to describe the dynamic process of malware propagation. The goals of the these propagation models can be classified into the following categories: (1) gain a deep understanding of the propagation mechanisms of malware. (2) predict the scale of the malware outbreak before it actually occurs; (3) evaluate how network provisioning impacts the propagation and how propagation impacts the network; (4) characterize the infection dynamics of malware; and (5) design countermeasures to restrain malware propagation.

% Infection vectors:
% - SMS/MMS:  ComWar worm browses hosts phonebook then spreads via SMS/MMS

% - Bluetooth\cite{Yan4268196,Yan4624266,rhodes2008,carettoni2007}: Device to device malware spreading: Limited attack vector because devices generally not in discovery mode, discovery period is limited, and file transfer requires user confirmation. 

% - Internet Access: Similar to PC enviornment

% - Compromised USB: for example if the programs used to synchronize smartphones were compromised.

% A representative unified and integrated propagation model remains unknown to the cyber security community. 
% Yan and Eidenbenz built an analytical model to study the spread of Bluetooth worms\cite{Yan4268196,Yan4624266}. They describe the impact of mobility patterns by investigating input parameters, such as average node degree, average node meeting rate, and link duration distribution.

% Rhodes and Nekovee \cite{rhodes2008} invesitaged the effect of population characteristics and device behavior on the outbreak dynamics of Bluetooth worms using SIP model. They assumed there is a single infected device capable of infecting any nearby device with probability p. Did not characterize the spatial-temporal characteristics of the propagation dynamics of Bluetooth worms, and also did not consider the impact of individual difference on the propagation dynamics of different worms. 

% (Superimposed graphs) Gao and Liu\cite{Gao2011,Gao2013} proposed a two layer model to simulate the propagation process of Bluetooth-based and SMS-based viruses. They modeled bluetooth propagation as a geographical overlay on a 2-dimensional grid. They modeled SMS-based virus propagation as a logical contacts graph where each node is a cell phone and the links are derived from address books. This evaluates the effects of human operations on SMS-based virus propagation and the effects of human mobility on geographic networks.

% Ramachandran and Sikdar\cite{Ramachandran2006,Ramachandran2007} presented analytical models to explore the impact of spreading mechanisms such as downloads from the Internet or P2P networks, WLAN and infrared interfaces and through MMS or SMS messages on the dynamics of malware propagation in smartphone networks. 

% most of the discussed models do not consider all possible input parameters. For example, most models have neither considered the impact of individual differences on malware propagation, nor considered the impact of human behavior on malware propagation. Nor did any describe the impact of random mobility on smartphone users. 

% Peng et al. \cite{Peng2013}
% }


% \comment{
% Mickens and Noble\cite{Mickens2005} proposed a probabilistic queuing framework to model the propagation of mobile malware over short-range wireless interfaces. This model emphasizes node mobility, a key factor in the non-homogeniety of near-proximity based mobile networks, as the node speed effects the steady state infection level of the network. \comment{This model accounted for movement and traffic patterns over various time durations(Not seen in previous analytical models)}

% Yan and Eidenbenz\cite{Yan4268196,Yan4624266} built an analytical model to study Bluetooth worm propagation. According to this model, the impact of mobility patterns on Bluetooth worm propagation can be investigated by introducing input parameters (e.g. link duration distribution, average node meeting rate, and average node degree). 

% Rhodes and Nekovee \cite{rhodes2008} invesitaged the effect of population characteristics and device behavior on the outbreak dynamics of Bluetooth worms using a susceptible-infected-removed (SIR) model. They assumed there is a single infected device capable of infecting any nearby device with probability p. Infected devices are removed, for example, if they become innoculated by an exploit patch. 

% Martin et al. \cite{Martin2010} predicted the spread of mobile platform viruses using the susceptible-infected-susceptible (SIS) model from mathematical epidemiology. In this model a node may be cured of infection but is still susceptible to a new infection. 


% Peng and Wang \cite{Peng2011, Peng2013} proposed a worm propagation modeling scheme (WPM) which simulates the dynamics of worm propagation process from a single node to the entire network using 2D cellular automata. This model takes into consideration the spread of of infected nodes in a network and offers a resistance factor to the susceptible nodes. 
% }
%\subsubsection{Proximity Attacks}%: e.g. modeling Bluetooth worms


To evaluate our GD algorithms, we use a grid, a random graph, and a
social network to connect the LDs. Indeed, there has much recent study
on network based malware/virus spread including propagation models
(e.g. SI, SIR, SIS), graph properties, and simulation/empirical
results
\cite{Mickens2005,Yan4268196,badusb,Fan2010ANSONAM,Yan4624266,suetal06:blueworm,Mickens2005,Cheng2007,wang09:spreading,kleinberg07:wlessepi,massganesh05:epidemics,kepwhite91:viruses}.
We highlight the work in \cite{massganesh05:epidemics}, where the
effects of graph structure on spread dynamics was characterized for a
variety of graphs. The spread can occur in various ways, e.g. over
geographical networks, online networks, call contact graphs,
proximity, etc. Further, the spread can be explicit (i.e., over the
contact graph itself) or implicit (i.e., the word-of-mouth contact
graph popularizes a malicious app, but the actual download is from a
app store).

We abstract these into three archetypical graphs: grid, random and
social. The grid graph, with small cycles and large diameter, captures
proximal networks for the spread (e.g. word-of-mouth, USB drives,
bluetooth). The random graph and social graph capture online networks
which have small degree but also a small diameter (i.e. things spread
rapidly). Phone contact graphs, Facebook graph, and email contact
graphs are illustrative of this class.


%models for how malware propagates across each LD-graph. 

% Malware often spreads through short-range wireless interfaces like
% Bluetooth~\cite{Mickens2005,Yan4268196,Yan4624266} or physical devices such as
% malicious USB drives~\cite{badusb}. Such proximity-based malware propagation
% can be modeled using a grid network of LDs.  In addition, we also study random
% graphs which are widely used as crude first-order model of networks with low
% diameter and small degree.

% Malware also spreads over contact graphs. For instance, Fan et al.
% \cite{Fan2010ANSONAM} discuss a model of computer viruses that transmit through
% Facebook and email, finding that the worm spreads through the contact graph and
% that Facebook worms spread faster than email worms. Further, Xin et al.
% \cite{Xin2009} examined the propagation of worms through a lens of game theory,
% concluding that camouflaged worms play better than naive worm and consequently
% propagate faster. 



%Much of the early research in modeling mobile malware propagation was
%spurred on by the worms Commwarrior and Cabir. 

%The Cabir worm propagated over Bluetooth, and CommWarrior over both Bluetooth
%and SMS/MMS \comment{(it picked contacts at random to send to)}.  For example,
%Mickens and Noble\cite{Mickens2005} proposed a probabilistic queuing framework
%to model the propagation of mobile malware over short-range wireless
%interfaces. Their model emphasizes node mobility, and determined it to be a key
%factor in the non-homogeneity of near-proximity based mobile networks, as the
%node speed affects the steady state infection level of the network. This model
%accounted for movement and traffic patterns over various time durations, a
%contribution not seen in previous analytical models.  Similarly, Yan and
%Eidenbenz\cite{Yan4268196,Yan4624266} continued studying Bluetooth worm
%propagation, determining that the impact of mobility patterns on Bluetooth worm
%propagation can be investigated by introducing input parameters to the model
%(e.g. link duration distribution, average node meeting rate, and average node
%degree).

% \ignore{
% Malware propagation models also borrow from mathematical epidemiology.  Rhodes
% and Nekovee \cite{rhodes2008} investigate the effect of population
% characteristics and device behavior on the outbreak dynamics of Bluetooth worms
% using a susceptible-infected-removed (SIR) model. They assumed there is a
% single infected device capable of infecting any nearby device with probability
% p, but where infected devices can be inoculated by a security patch. Later,
% Martin et al. \cite{Martin2010} described the spread of mobile malware using a
% susceptible-infected-susceptible (SIS) model.  In this model a node may be
% cured of infection but is still susceptible to a new infection.  Peng and Wang
% \cite{Peng2011, Peng2013} proposed a worm propagation modeling scheme (WPM)
% which simulates the dynamics of worm propagation process from a single node to
% the entire network using 2D cellular automata. 
% }

%This model takes
%into consideration the spread of of infected nodes in a network and offers a
%resistance factor to the susceptible nodes.



%Unlike proximity-based infections, malware that propagates through the internet
%has the potential to do significantly more damage\cite{morris-worm, storm-worm, conficker-worm}\comment{\todo{CITE} \michael{Morris
%Worm, Storm Worm, Conficker Worm}

% https://tools.ietf.org/html/rfc1135 Morris Worm,
% https://www.f-secure.com/v-descs/small_dam.shtml Storm Worm,
% http://www.microsoft.com/security/portal/threat/encyclopedia/entry.aspx?Name=Worm:Win32/Conficker.E#tab=2
% Conficker} 

%[Morris Worm, Storm Worm, Conficker]} and smartphones offer a mobile platform
%for such worms 
%Previous work models the spread of these internet worm through


% Ultimately, mobile platforms suffer from a multi-vector attack scenario. As
% such, researchers have proposed hybrid propagation proximity-based and
% internet-based models. In general, this is captured via Bluetooth and SMS/MMS
% models. Cheng et al.~\cite{Cheng2011MalProp} proposed the first hybrid
% analytical model based on the propagation of the CommWarrior worm, measuring
% the speed and severity of its propagation.  Ramachandran and
% Sikdar~\cite{Ramachandran2006,Ramachandran2007} explored the impact of
% spreading mechanisms such as downloads from the Internet and P2P networks,
% infrared interfaces, and through MMS and SMS on the dynamics of malware
% propagation in smartphone networks. Xia et al.~\cite{Xia2008} further
% considered the situation where an infected device may be in a dormant state.
% Fan \cite{Fan2010:5601326} built a hybrid model based on preventative immunity,
% and virus mutation that takes mobility of the actors into account. Gao and
% Liu\cite{Gao2011,Gao2013} proposed a two-layer hybrid model using superimposed
% graphs. They model bluetooth propagation as a geographical overlay on a
% two-dimensional grid and  SMS-based propagation as a logical contacts graph
% where each node is a cell phone and the links are derived from address books.
% Therefore, their work considers both the effects of human operations on
% SMS-based propagation and the effects of human mobility on geographic networks.






==> intro/related-work.tex <==
% \subsection{Related Work}

\comment{
\mohit{from proposal}
Inference on networks has seen a lot of
interest recently, with research on determining epidemic source aka rumor
source) \cite{infectionsource,zash11,karam13,luo12,luo13,zhuyin}, learning
network structure from observations \cite{gomez2012,netrapalli12}, and
inferring for causation (work by PIs)
\cite{milling12,allerton2012,mobihoc2013,meirom14}. Beyond the epidemic
context, statistical models for parameter learning
\cite{dene05a,dene05b,streftaris02,demiris05b,bane04} and anomaly learning
\cite{acd08,acd11} have seen much progress over the last decade. Our approach
-- dynamic learning from weak signals for reducing false positives/negatives
using the network -- is a new direction. Tangentially related are works with
active detection techniques where one considers optimal sensor placement for
epidemic detection, e.g., \cite{LeskovecKDD2007}.
%
From a systems perspective, such network based approaches have been studied in
the context of collaborative IDS \cite{dash06,seurat,IDS-survey15} (also see
related works in Section~\ref{sec:arch}).  Most relevant is \cite{dash06} where
the authors use a variety of count methods (analysis of the time series of
cumulative alert counts) at a global level by aggregating all the local
detector counts. As discussed earlier, the space-time geometry emerging from
the community structure and shape distributions of true and false positives
provide a more nuanced lens for detecting zero-day exploits.
% Thus, the key innovation in our approach is that we use the fine-grained
% community space-time structure as a lens to filter and bias alert samples --
As we will see in Figure~\ref{fig:eigen} and Question~4, these insights provide
a powerful boost for early stage malware detection.
}

\input{intro/behavioral-analysis}
\input{intro/cids}
\input{intro/malware-propagation}


==> intro/threat.tex <==
\subsection{Threat Model and Assumptions}
\label{sec:threat}

%Mobile app ecosystems are complex and we minimally consider a system
%with six principals -- users, benign and malware app developers,
%mobile platform providers, hardware manufacturers, malware analysts,
%and finally \sysname itself.  

We assume that a large fraction of our
users and developers are benign and can provide data to build robust
models.  \sysname is thus best suited for early stage malware
detection -- if the majority of devices are compromised, behavioral
analysis is useless.  Malware developers are untrusted and can exploit
apps, the underlying operating system and hardware, and even trick
users into installing overprivileged apps.  The end result is that
malware turns a fraction of the devices on a network into active
adversaries that attempt to evade detection while executing malicious
payloads.
%
%
The remaining principals function similar to traditional Collaborative IDSs.
Platform providers like Google and Samsung are trusted and can open up
important operating system and hardware-level signals for malware detection.
We trust hardware manufacturers like Intel and Qualcomm to implement their
instruction sets without hardware backdoors.  Malware analysts are trusted but
only to provide malware detection results and are not trusted to view or infer
users' private data.  Finally, we trust \sysname as a platform to collect,
seal, and declassify user data.


==> local_detectors.tex <==
%\subsection{Local Detectors}
%\label{sec:LDs}

Our first step is to establish a good local detector (LD) for desktop systems
running Windows OS.  In particular, we choose system call based LDs since the
system call interface has visibility into an app's intercation with core OS
components -- file system, Windows registry, network -- and
%file, device, and network activity and 
can thus capture signals relevant to malware executions.

We experiment with an extensive set of system-call LDs -- our takeaway is that
even the best LD we could construct operates at a true- and false-positive
ratio of 92.4\%:6\% and is not deployable by itself (i.e.,
will create $\sim$30 false positives every 10 minutes without a GD). 

%These LDs and 
%detection rates are representative of prior findings against similar malware -- 
%we could improve both the LDs and model adaptive malware but

%\mikhail{Should we mention an optimal point: FP=5.5\% and TP=92.4\% ? 95:10 is not optimal.}

Each LD comprises of a feature extraction (FE) algorithm and a machine learning
(ML) classifier.  Our FE algorithm partitions the time-series of system calls
into 1-sec chunks and represents each chunk as a histogram (where each bin
contains frequency of a particular system call).  Then it projects all feature
vectors onto 10-dimensional subspace spanned by top 10 principal components
generated by PCA algorithm.  We choose ML
%LD candidates from general machine
classifiers (used throughout prior work 
because these are computationally efficient to train) such as SVMs, random
forest, k-Nearest Neighbors, etc, and do not include complex alternatives such
as artificial neural networks or deep learning algorithms.  We also
deliberately avoid handcrafted ML algorithms and hardcoded detection rules.

%because such custom models usually overfit a specific dataset, and because
%they require humans to continuously adjust the detector to new types of
%malware.

%To extract features, we experiment with histograms, n-grams, and also using a human-understandable system call basis.
%When using histograms and n-grams, we compute the (top ten) principal
%components using PCA analysis to reduce dimensionality of the data. 
%For the human-understandable \intbasis, we group system calls into
%33 dimensions each related to file access, networking, process control, etc.
%We use \intbasis as a candidate because it enables malware analysts to 
%map malware payloads back to intuitive tasks such as stealing SMSs or snooping
%on location data.

Figure~\ref{fig:windows-LD-roc} plots the true positive v. false positive rates
(i.e. the ROC curves) of the seven ML algorithms we evaluate.  The area under
the ROC curve (AUC) is a quantitative measure of LD's performance: the larger
the AUC, the more accurate the detector.  We specifically experiment with seven
state-of-the-art ML algorithms: random forest, 2-class SVM, kNN, decision
trees, naive Bayes, and their ensemble versions -- boosted decision trees with
AdaBoost algorithm and Random SubSpace ensemble of kNN classifiers
(Figure~\ref{fig:windows-LD-roc}).  We also evaluated 1-class SVM as an anomaly
detector -- however, it yielded an extremely high FP rate and we exclude it
from further discussion.  Overall, the random forest classifier worked best --
it has the highest AUC and we pick an operating point of
92.4\% true positives at a false positive rate of 6\%. 
%We also evaluated 1-class SVM as an anomaly detector and Naive Bayes
%classifier -- however, both yielded an extremely high FP rate and we exclude
%them from further discussion.  In total, we consider these 7 candidate LDs to
%choose the best one.  We compare all of them using ROC curves To construct ROC
%curves we apply 10-fold cross validation to avoid any bias from the dataset,
%i.e. our classifiers predict labels of in-fold observations using a model
%trained on out-of-fold observations. 

\begin{figure}[tbp]
%\vspace{-0.2in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/windows/ROC/roc-curves.eps}\par
\caption{(ROC curves) True positive v. False positive curves shows detection
accuracy of seven local detectors.  
%In terms of detection accuracy and
%computational efficiency, 
Random Forest outperforms all others;
%However, any of these local malware detectors
but has unacceptably high false
positive rate (above 10\%) if one wants to achieve at least 95\% true positive
rate.}
   \vspace{-0.2in}
\label{fig:windows-LD-roc}
\end{figure}

==> notes/graph-size.tex <==
% Graph Size

I am not convinced that we need to process any graph larger than 15k nodes to prove our point. Consider the UT computer network. Here, machines are probably distributed between \textit{buildings} or \textit{departments} with reasonable density. Consequently, we can consider strong subgraphs as a partition of the overall graph structure. Each subgraph contains some notion of a community structure and the connectivity between subgraphs is extremely low (potentially disjoint) therefore we can process each subgraph independently and aggregate at a later time. This should reduce processing time dramatically at the cost of adding noise to the time to detection.   


==> overhead.tex <==
%{\color{red} Rev.A. Computational complexity of the proposed scheme can be further elaborated. }
%Recall that Shape GD requires only the
%low-dimensional alert FVs -- this leads to a two-fold dimensionality reduction
%when sending data from individual nodes to the GD. First, the FVs are
%low-dimensional (here, 10-dimensional vectors). Second, only alert FVs are
%needed -- this leads to a 16-fold reduction in data (roughly only 6\% of the
%FVs lead to alerts). Further, the Shape GD is a batch processing algorithm,
%thus, the individual nodes can batch their data at coarse time-scales (e.g.
%once every NTW) and send the data to the Shape GD. Finally, it does not matter
%even if some batches are lost/missed; recall that the Shape GD is robust to
%precisely this type of noise.

\noindent{\bf Performance Overheads.} Recall that Shape GD requires only 
alert FVs -- this leads to a two-fold dimensionality reduction
when sending data from individual LDs to the GD. First, the FVs are
low-dimensional (here, 10-dimensional vectors).  Second, only alert FVs are
needed -- this leads to a 16-fold reduction in data (roughly only 6\% of the
FVs lead to alerts). Further, the Shape GD is a batch processing algorithm,
thus, the individual nodes can batch their data at coarse time-scales (e.g.
once every NTW) and send the data to the Shape GD.  Finally, it does not matter
even if some batches are lost/missed; recall that the Shape GD is robust to
precisely this type of noise.  
%Appendix~\ref{sec:appendix-overhead}
Appendix~A
discusses overheads in more depth but the key takeaway is that
Shape GD has low overheads -- 
each LD can use simple dot products and scalar comparisons to implement PCA and
Random Forests, the total incoming bandwidth to the Shape GD server ranges from
40KBps to 174KBps for phishing and waterhole respectively, and the server only
needs to bin data (into 50 bins) and compute Wasserstein distance (add 10
counters in each bin).

%Obviously, Shape GD's overhead scales linearly with the number of attack types that it is configured to detect.

%Overall overhead of running LDs on end-hosts and Shape GD on a dedicated server is negligible.
%Overall, the entire system has negligible overhead, which comes from running LDs and Shape GD on a dedicated server
%Here we mainly focus on estimating overhead associated with Shape GD, which includes transferring FVs from end-hosts to a centralized server and server-based computations.
%Overhead of local detectors has been extensively evaluated in prior work \cite{mihai} and it is very low ...\%.

%Finally, Shape GD computes a dot product of reference histogram and
%the previously estimated pmf of incoming FVs, each vector has 10
%dimensional. 

%Memory overhead on a server side is constant -- $\sim 2 KB$: number
%of bins (50) times dimensionality of FVs (10) for building pmf and
%computing neighborhood score.


==> results.tex <==
%\input{results/intro_results}

%\subsection{Local Detectors and Feature Extraction algorithms}
%\label{sec:LDs}
%\input{results/LDs}

\todo{

Assume:
\begin{itemize}
\item community
\item neighborhood. applied to phishing and waterhole.
\item filtering
\item shape (idea) --> wasserstein distance (metric).
\end{itemize}

Why each subsection?
\begin{itemize}
\item Top-level goal: Early detection as malware infects a neighborhood.
How early? We proceeed in three steps.

\item Step 1: 
How well can GD distinguish between {\em purely} benign v. malicious
neighborhoods? This is a baseline test for shape-based GD. In the
next two subsections, we will use shape-GD to classify neighborhoods 
with early-stage infections from benign neighborhoods -- i.e., when
malicious neighborhood has {\em a mix of benign and malware FVs}.
%-- i.e., shape-GD has to
%distinguish a mix of malicious and benign nodes.

\item Step 2: 
Phishing: how {\em quickly} can shape-GD detect malware if it spreads through
a few malicious emails among many benign emails in a enterprise network?

\item Step 3:
Waterhole: how {\em quickly} can shape-GD detect malware if it spreads
through a few malicious servers that compromise clients that visit the
malicious servers?

\end{itemize}



How + Results.
\begin{itemize}

\item [Ref Section 4] Each nbd has a score -- i.e., 
Wasserstein distance metric -- and in Fig X, we will plot the histogram
of scores from N benign nbds v. N malicious nbds.

Explanation: Perfect separation at 15k FV/nbd. 
But partial overlap of benign and malicious histograms may be ok -- this 
creates GD FPs. 

\item Phishing. Early detection using shape-only: shape works at 22 [Fig X].
On the other hand, small errors in count lead to large errors in 
time to detection [Fig Y]. In Fig Z, we show that shape + NF improves
shape-only by 4X

\end{itemize}
}






We now report the main results of our computations. Ultimately our
goal is to demonstrate that our overall LD + GD framework is effective
and hence presents a new paradigm for early detection of new malware
epidemics. In addition, we present a host of ancillary or intermediate
results, that demonstrate the conceptual underpinnings of this
paper. We present results on our local detectors. We test the
effectiveness and robustness of the shape-based detection that
underlies our GI engine, and compare to count-based algorithms. We
expand on Figure~\ref{fig:intro-histogram} to show what at some level
is the cornerstone technical piece of our approach: the fact that the
conditional distributions of false positives and true positives are
well separated in the right metric -- we present several more
supporting results.

\subsection{Local Detectors are Noisy}

In Section \ref{sec:exp-set}, we describe the local detector we finally select.
We provide here some interesting aspects of the detector we use in our overall
framework. The LD results in Figure~\ref{fig:ROC} show three interesting
trends. First,  Random Forest outperforms all other classifiers.  2-class SVM
and Decision Tree algorithm are close to but lower than Random Forest in terms
of detection accuracy. Second, the \intbasis LD algorithm leads to poor
detection results across all ML classifiers. The Histogram and n-gram FE
algorithms are almost identical in terms of detection accuracy -- hence we
favor histogram FE algorithm over n-grams because n-gram models are
computationally expensive to run on client devices.

The key result from this study is that we use Random Forest with a
histogram-based FE algorithm as a representative LD. In our choice, the
assumption is implicit that the best performing LD will yield the best GD. This
is plausible because if we have no side information about the new malware we
are hoping to detect (and indeed, we assume this is the case), any degraded LD
performance is simply noise that we should not expect to do anything but
deteriorate the performance of any global inference engine using its output as
input. A related point to make is that we believe our main contributions in our
Global Inference Engine framework, begin where the LD leaves off. That is to
say, we expect that a better LD could be easily integrated into our framework,
and we believe it would only lead to improved results.

\subsection{True from False Positives: The Power of Shape}
\label{sec:pure_shape}
\input{results/pure_shape}

\subsection{Global Inference Engine: ROC}
\label{sec:GD_ROC}
\input{results/GD_ROC}

\subsection{Shape vs Count without censoring}
\label{sec:shape_vs_count}
\input{results/shape_vs_count}

%\subsection{Number Of Bins}
%\label{sec:bin_number}
%\input{results/bin_number}

%\subsection{Censoring algorithm.}
%\label{sec:censoring}
%\input{results/censoring}

\subsection{Censoring Algorithm: Neighborhood Filter}
\label{sec:censoring}
\input{results/detection_threshold_vs_censoring_threshold}

\subsection{Detection Threshold Scales As Log(n)}
\label{sec:ttd_as_log_n}
\input{results/log_n}

\subsection{Detection threshold vs percentile}
\label{sec:detection_threshold}
\input{results/detection_threshold_vs_percentile}

%\subsection{Learning the basis.}
%\label{sec:basis_learning}
%\input{results/basis_learning}

%\subsection{Robustness To Polluted Training Data}
%\label{sec:robustness_polluted_training_data}
%\input{results/robustness_polluted_training_data}

%\subsection{Robustness To Compromised Local Detectors}
%\label{sec:robustness_compromised_LDs}
%\input{results/robustness_compromised_LDs}

%\subsection{Protecting Multiple Versions Of An App [Michael]}
%\label{sec:multiple_app_versions}
%\input{results/multiple_app_versions}
%
%\subsection{Android Monkey vs Real User Input [Michael] (Drop it)}
%\label{sec:monkey_vs_real_user}
%\input{results/monkey_vs_real_user}
%
%\subsection{Cause Analysis. Supervised Learning???}
%\label{sec:cause_analysis}
%\input{results/cause_analysis_intuitive_basis}


==> results/GD_ROC.tex <==
\begin{figure*}[t]
  \begin{minipage}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/GD_ROC/GD_ROC_Random_Forest.pdf}\par
    \subcaption{Random Forest}
\label{fig:GD_ROC_RF}
  \end{minipage}
  \begin{minipage}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/GD_ROC/GD_ROC_2_class_SVM.pdf}\par
    \subcaption{Two-Class SVM}
\label{fig:GD_ROC_SVM}
  \end{minipage}
  \begin{minipage}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/GD_ROC/GD_ROC_AdaBoost_Decision_Trees.pdf}\par
    \subcaption{Boosted Decision Trees}
\label{fig:GD_ROC_BOOSTED_DTs}
  \end{minipage}
  \caption{Shape GD's ROC curves. In most of the cases we consider,
      Shape GD perfectly separates false and true positives -- this is shown by
      black  step-wise curves. It is worth noting that histogram separation
      depends on an LD that is used -- GD and LD should be co-designed.}
  

\label{fig:GD_ROC}
\end{figure*}

For most apps, Shape GD achieves perfect separation of false and true positive
distributions of FVs (Figure~\ref{fig:histogram}); sometimes, however, we observe in our results that the conditional distributions display a slight overlap. In those cases, the robustness threshold
$\gamma$ (see Section~\ref{sec:algo_description}) should be carefully chosen to avoid
global false positives, i.e., to avoid mislabeling communities as infected. In this section, we explore and quantify more carefully, our ability to separate true and false positives, i.e., we quantify the performance of Shape GD. We do this via ROC curves. ROC curves provide a standard method for analyzing the trade-off between global FPs and TPs.% before choosing a particular $\gamma$.

%As discussed earlier, 
%Shape GD makes a decision on labeling incoming FVs as malicious or benign based
%on the hypothesis test parameterized by the robustness threshold $\gamma$ (Section\todo). In our implementation, we set $\gamma$ 
%based on the shape of FP and TP distributions (Figure~\ref{fig:histogram}),
%%When choosing a particular $\gamma$, we try 
%with the goal of minimizing the global false positive rate.

To build an ROC curve, 
%instead of choosing a concrete value of $\gamma$, 
we sweep the entire range of values that $\gamma$ can take. For each such
value, we record a corresponding GD true and false positive rate
%And then by combining them, we 
to obtain an ROC curve for the app. 
%We have plotted ROC curves for
Figure~\ref{fig:GD_ROC} shows the Shape GD's 
ROC curves for all apps in our experiment.
%Shape GD and all the apps from our corpus 

%As expected, ROC plot shows the trade-off between global false and true
%positives. 

The most interesting part of this ROC plot is that half of the apps' ROC curves
-- the black line -- have a step-shape because Shape GD achieves flawless
separation between local FPs and TPs. This follows from the TP v. FP histograms
in Figure~\ref{fig:histogram}.
%From analysis of ROC plot, we see that Shape GD demonstrates ideal accuracy
%when running on the following 
The five apps with perfect ROC curve are AVG, Buzzfeed, All Recipes, Wikipedia, and Zedge.  Three
other apps -- Walmart, Bible, eBay -- have slightly overlapping distributions
of local false and true positives, hence the corresponding ROC curves deviate
from the step-shape. And finally the last two apps -- Yelp and Html5 -- do not
have separable distributions of TPs and FPs when processed by our Shape GD,
i.e., global detection may lead to community-level misclassification. 

%We exclude those apps from the further consideration.
GD's performance depends on a choice of LD (Figure \ref{fig:GD_ROC}). When
using Random Forest as LD, GD does not work for Yelp and HTML5. However, if we consider
2-class SVM, then GD is able to process Yelp. Similarly, if 
we switch to Boosted Decision
Trees LD, then GD can handle both apps, but it does not work well for Buzzfeed.
Thus, LD and GD should co-designed.

In summary, 
%when choosing a concrete value for 
setting the robustness $\gamma$, i.e., the GD's false positive rate, 
to 10\%, yields a true positive rate close to 100\% for 
%accurate results and does not sacrifice detection rate because 
all apps except Yelp and Html5. In comparison, the constituent LD
only yields a detection rate of 80\% for a false positive rate of 10\% (Figure~\ref{fig:ROC}). And again, for the majority of the apps we tested, GD's (global) false positive rate is reduced to effectively 0\%, while achieving a detection rate of 100\%. 
%\todo{Say what the baseline LD} 
%have global true positive rate higher than 95\%.
%\todo{for what FP rate: zero?}




==> results/bin_number.tex <==
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/number_of_bins.pdf}\par
\caption{\textit{(Shape detector: Effect of binning on the detector's sensitivity.}}
\label{fig:num_of_bins}
\end{figure}

When tuning parameters of our global detector, we noticed that the way we discretisize  the data, i.e. compute \textit{pmf}, is crucial for the overall performance of the global detector.

By analyzing distribution along every principal in the training phase, we notice that distributions usually have very long tails. When we apply standard binning algorithm with uniform bin sizes, we obtain many empty or almost empty bins. The drawback of such straightforward binning is that 1) global detector has to operate high-dimensional pmfs; 2) \sysname is extremely sensitive to any noise due to huge number of low populated bins.

To overcome this issue, we trim the tails of the distribution -- the data below 1th percentile and above 99\% percentile. The trimmed tails are represented as two separate bins of infinite size. The rest of the distribution is covered with a few dozens of bins, whose number is defined based on either "square-root choice" sqrt(n) or Scott's normal reference rule $3.5*sigma/n^0.33$. The Scott's rule calculates different number of bins for each dimension of data. And we choose the maximum number to achieve the highest resolution. For example, in the case of Wikipedia the former rule results in 33 bins and the latter results in 55 bins. In our experiments we do not observe significant difference between these strategies of choosing the number of bins. Thus, we stick to Scott's rule for consistency.

As an alternative solution we tried to apply non-uniform binning, but binning based on either square-root choice or Scott's rule gives better results than non-uniform binning.

Also we swept the parameter space to get a better feeling of whether our binning strategies are reasonable or not~\ref{fig:num_of_bins}. The resolution of the x axis is 10. For every value of the parameter "number of bins", we computed the contamination level of the input data set that triggers global detector. We averaged the results over 10 runs of the experiment. The plot shows that the global detector starts reacting to malware if its level exceeds 8\%. Indirectly, the plot proves that our strategy for choosing the number of bins is adequate because none of the two choices gives advantage over the other one.

==> results/censoring.tex <==
%\begin{figure}[tbp]
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/wiki_vs_censoring_threshold.pdf}\par
%\caption{\textit{(Wikipedia) Detection rate vs censoring threshold.}}
%\label{fig:wiki_vs_censoring_threshold}
%\end{figure}


==> results/detection_threshold_vs_censoring_threshold.tex <==
%Despite the low detection threshold (5-15\% in sec.~\ref{sec:shape_vs_count})
%achieved by Shape GD, large absolute numbers of nodes in a network need to be
%infected before \sysname is able to spot malware. 

To further reduce the time to detection, we apply the Neighborhood Filtering
(NF) algorithm (see Section~\ref{sec:algo_description}) to the baseline Shape GD.
Recall that NF is a neighborhood alert-density dependent censor, i.e., it
considers an alert in the Shape GD only if the number of alerts in
its local space-time neighborhood are above a {\em censoring threshold}. 
%Here we analyze the Shape GD benefits from
%Neighborhood Filtering.
%We have already seen (Figure~\ref{fig:shape_vs_count}) that Shape GD is able to achieve detection rate of 8.8\% (Figure~\ref{fig:shape_vs_count_random}) and 14.4\% (Figure~\ref{fig:shape_vs_count_social}) in a network with random graph topology and in a social network respectively. Its performance is much better in the case of grid topology - 4.6\% (Figure~\ref{fig:shape_vs_count_grid}). Even if these numbers are quite small, the absolute number of infected nodes can be large in big networks.

Intuitively, to eliminate a majority of false positives, the censoring
threshold $\lambda$ should be above the LD's FP rate. To confirm this, we vary the
censoring threshold from 0\% up to 100\% and record the corresponding value of
detection threshold. Figure ~\ref{fig:censoring} shows the results of
this experiment with three types of networks: random, grid
and social network. The horizontal axis shows censoring threshold $\lambda$,
and the vertical axis corresponds to the detection threshold. The robustness
threshold $\gamma$, i.e., the GD's false positive rate, is set to 10\%.
%Whatever topology an underlying network has, 

We find that the optimal range for the censoring
threshold $\lambda$ is between 35\% and 80\% for all three network topologies. 
When $\lambda$ is less than 35\%,
i.e., close to the LD's false positive rate, detection threshold is higher and unstable.
Conversely, if censoring threshold is too high, too many true positives
get filtered out and GD is only able to spot malware in a community when almost
all nodes are infected. 

%If we look how NF affects GD's performance for individual networks, 
We observe that NF improves GD's performance the most for random
networks (detection threshold drops from 10\% down to 3\%) -- this happens due
to the presence of multiple long-range connections between network nodes. Even
though Shape GD worked best for a grid network, NF improves its performance by a 
%spite of demonstrating the best detection results in grid network, Shape GD is
further 5$\times$ (0.6\% from 3\%). For the
social network, detection threshold goes down to 2.2\% from the
original 10\%.

Overall, NF censoring helps to bring detection threshold down by 3-5$\times$ and keeps it under 3\% level for all three networks.


%GD's performance on random network is affected the most by censoring and detection threshold drops from 10\% down to 3\%. One can observe similar trend for social network -- detection rate goes from 9\% down to 2.2\%. GD also benefits when running on a graph with grid topology -- drop from 3\% down to 0.6\%. Thus, censoring helps to bring detection threshold down by 3-5x and keep it under 3\% level for all types of network.

%Detection threshold remains low till reaching 80\% censoring threshold. After that it goes up because censoring algorithm ignores too many malicious neighborhoods, thus GD does not receive any incoming data. Only if a large portion of a network is infected, then GD starts receiving malicious data and is able to label it correctly.

%We choose 50\% censoring threshold for the remaining experiments.


==> results/detection_threshold_vs_percentile.tex <==
Shape GD relies on the hypothesis test (Section~\ref{sec:algo_description}) that
is parametrized by the robustness threshold $\gamma$. 
%For a fixed $\gamma$,
%GD's output has confidence $1-\gamma$. 
Low values of $\gamma$ lead to a low GD false positive rate, but they may also result in low detection thresholds (and thus late malware reporting). We analyze GD's sensitivity to $\gamma$ to balance time to detection and accuracy of GD's output.

We vary the robustness threshold $\gamma$ from 0\% (percentile) up to 50\%
and 
%When $\gamma$ is set to 50\%, GD's output
%is correct with probability 50\% -- it is equivalent to random guess, that's
%why we do not go beyond the value of 50\%. As usual, we repeat the same
experiment with the three types of networks: random, grid, and social network.

Figure~\ref{fig:detect_vs_prctile} plots the detection threshold v. the censoring
threshold -- so that a low value on Y-axis is better. 
If we exclude effect of NF,
detection threshold drops fast -- 36\% vs 12\%, 28\% vs 8.8\%, 11.5\% vs 3.5\%
for random, grid and social networks respectively -- when increasing $\lambda$
from 0\% up to 10\%. With no censoring, 
10\% is a reasonable value for $\lambda$ that
%moves GD's performance to the desirable range, i.e., 
moves detection threshold to
under 12\%.

Neighborhood filtering (NF) (sec.~\ref{sec:censoring}) brings
the curves closer to the horizontal axis and makes them flatter
(Figures\ref{fig:detect_vs_prctile}). However, the left-hand side part of
the curves corresponding to the values of $\gamma < 10\%$ has steep slope. It
is still beneficial to admit 10\% error by setting $\gamma = 10\%$. If
censoring threshold $\lambda = 50\%$, i.e., the third graph on the right, then setting $\gamma$ to 10\% let us
reduce detection threshold to less than 2\% level across all network toplogies
that we consider. It is worth noting that Shape GD's detection threshold in
grid network has very low value of 0.3\%.

Shape GD is mainly governed by two parameters - the censoring threshold
$\lambda$ and the robustness threshold $\gamma$. Based on the analysis of GD's
sensitivity (sec.~\ref{sec:censoring} and sec.~\ref{sec:detection_threshold})
to these parameters $\lambda = 50\%$ and $\gamma = 10\%$ seem to be an optimal
setting that allows Shape GD to identify malware spread at an early stage and
keep high accuracy of GD's detection results.


==> results/intro_results.tex <==
\mikhail{In the the following subsections we walk a reader through the process of
building a network-level malware detector and justify every step. 

First, we start with consideration of a few local detectors (LDs). 
Second, we
address our premise that shape of distribution contains much more information
than a simple aggregation of LDs' outputs. Third, we evaluate the role of
space-time geometry for both shape and count-based detectors. Forth, we
estimate fault-tolerance properties of our system under assumptions that some
LDs and network media may be brought down by an attacker or due to
software/hardware failure. And finally, we bring our attention to the one of
the most crucial problems in malware detection -- "cause analysis". As a result
of the design solutions made at earlier stages, \sysname allows a malware
analyst easily find out high-level malicious behavior. Partially, this is
achieved by using a completely novel technique in the field of computer
security -- dictionary learning.}


==> results/log_n.tex <==
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/log_n/log_n_all.pdf}\par
\caption{(Wikipedia app) Detection threshold scales as a logarithmic function of network size.}
\label{fig:wiki_vs_censoring_threshold}
\end{figure}


\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/detection_threshold_vs_censoring_threshold/combined.pdf}\par
\caption{(Wikipedia app) Detection threshold vs censoring threshold. We analyze the effect of censoring on the detection threshold. Censoring threshold reduces detection threshold if it is above LD's FP rate.}
\label{fig:censoring}
\end{figure}

\begin{figure*}[t]
\begin{minipage}[tbp]{0.3\linewidth}
%   \begin{flushleft}
  \centering
   \includegraphics[width=\textwidth]{figs/detection_threshold_vs_prctile/no_censoring/combined.pdf}\par
   \subcaption{{No censoring}}
   \label{fig:detect_vs_prctile_no_censoring}
%   \end{flushleft}
\end{minipage}
%\hfill
\begin{minipage}[tbp]{0.3\linewidth}
%   \begin{flushright}
  \centering
   \includegraphics[width=\textwidth]{figs/detection_threshold_vs_prctile/censoring_0.3/combined.pdf}\par
   \subcaption{{30\% censoring threshold}}
   %\caption*{{Angry Birds game + click fraud}} 
   \label{fig:detect_vs_prctile_0.3_censoring}
%   \end{flushright}
\end{minipage}
\begin{minipage}[tbp]{0.3\linewidth}
  \centering
%   \begin{flushright}
   \includegraphics[width=\textwidth]{figs/detection_threshold_vs_prctile/censoring_0.5/combined.pdf}\par
   \subcaption{{50\% censoring threshold}}
   \label{fig:detect_vs_prctile_0.5_censoring}
%   \end{flushright}
\end{minipage}
\caption{(Wikipedia) Detection threshold vs robustness threshold $\gamma$. In this experiment we lower detection rate by decreasing confidence of GD's results. We consider three types of censoring thresholds: 0\%, 30\%, 50\%.}
\label{fig:detect_vs_prctile}
\end{figure*}


Standard hypothesis testing theory implies that under appropriate independence
assumptions, the probability of error decays exponentially in sample
size. To ensure that the probabilities of error goes to zero, it follows that
the sample size needs to scale logarithmically in network size ($e^{-\alpha
\log(n)} \to 0$ as $n \to \infty$). In a network of mobile applications,
{\it a priori}, it is not clear if independence across samples holds, or even a
weaker condition such correlation decay across samples holds (which also can
lead to exponentially decaying bounds).


%\sanjay{please, rewrite the text in this section}
% It can be proven that Shape GD's detection threshold scales as a logarithmic function of the number of nodes in a network while Count GD's detection threshold is proportional to the square root of the network size. Given a very large network, Shape GD can identify infected communities much faster than Count GD. Considering exponential nature of malware propagation process, even a small reduction in detection threshold can significantly reduce time to detection.

To study this, we conduct the following experiment (repeated 300 times):
we abstract away from a particular network topology because this result
should hold in a network with any internal structure. As we have described in
Section~\ref{sec:shape_vs_count}, we train Shape GD on 11,000 benign FVs.
We then run Shape GD on data sets that contain various portions of malicious
FVs (from 0\% up to 100\%) and have different sizes (from 1,000 up to 32,000).
%By varying portion of malicious FVs in a data set, we can 
We then determine detection threshold for a false positive rate of 10\%. 

%To gain statistical significance we repeat the experiment 300 times.

%When plotting the 
Figure~\ref{fig:wiki_vs_censoring_threshold} shows  detection threshold vs network size (logarithmic
scale) -- detection threshold scales down as a logarithmic function of network
size.  Specifially as we increase network size from 1,000 to 32,000, the
detection threshold drops from 19\% to 10\%. This, in turn, implies that we can
detect malware spreads at the very early stages.


% Thus, in the large communities \sysname can spot
% infection at the very early stages. Deviation from logarithmic
% dependency may have been caused by limited number of samples in our
% experiment.



==> results/pure_shape.tex <==

%\begin{figure}[tbp]
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/histogram.pdf}\par
%\caption{\textit{(Wikipedia app) Distribution of Wasserstein distances between FPs/TPs and a reference histogram. Shape-based GD can reliably separate FPs and TPs through extracting information from the data that has been unutilized by an LD.
%*The constant offset -- 8,948,200 -- has been subtracted from the Wasserstein distances.}}
%\label{fig:histogram}
%\end{figure}
%

\begin{figure*}[t]
\begin{minipage}[tbp]{0.24\linewidth}
  \centering
   \includegraphics[width=\textwidth]{figs/histogram/histogram_walmart.pdf}\par
	\subcaption{Walmart app}  
%%   \label{fig:histogram_walmart}
\end{minipage}
\begin{minipage}[tbp]{0.24\linewidth}
  \centering
   \includegraphics[width=\textwidth]{figs/histogram/histogram_avg.pdf}\par
	\subcaption{AVG app}  
%%   \label{fig:histogram_avg}
\end{minipage}
\begin{minipage}[tbp]{0.24\linewidth}
  \centering
   \includegraphics[width=\textwidth]{figs/histogram/histogram_buzzfeed.pdf}\par
	\subcaption{Buzzfeed app}  
%%   \label{fig:histogram_buzzfeed}
\end{minipage}
\begin{minipage}[tbp]{0.24\linewidth}
  \centering
   \includegraphics[width=\textwidth]{figs/histogram/histogram_yelp.pdf}\par
	\subcaption{Yelp app}  
%%   \label{fig:histogram_wiki}
\end{minipage}
\caption{(Wikipedia app) Distribution of Wasserstein distances between FPs/TPs and a reference histogram. Shape-based GD can reliably separate FPs and TPs through extracting information from the data that has been unutilized by an LD.
}
\label{fig:histogram}
\end{figure*}


A key property our framework builds on, is the fact that \textit{the distributional shape of true positive feature vectors differs from that of false positives}. We build here on the discussion initiated in Section \ref{sec:intro} and the results displayed in Figure \ref{fig:intro-histogram}. 

%Recall our discussion in Section~\ref{sec:ideas}: the discriminating
%power of the feature vectors is more than that of alerts. We now
%quantify if this observation can be used by a Global Detector.


% Thus,
% they leave behind a lot of unutilized information.  \todo{cut
%   candidate. Or, fold content into algo section.}

%To quantify the separation between FPs and TPs that Shape GD is able to
%achieve
In our experiments, we sample uniformly from random two subsets of feature
vectors -- one subset from a benign data set and the other one from a malicious
data set.  Each subset contains 3,000 unique feature vectors.
% i.e.  they are sampled without replacement. 
After passing these two subsets through an LD -- the Random Forest trained on both benign and malicious system call histograms -- we obtain a collection of false positives (FPs) and true positives (TPs) for the chosen subsets. We then compute the community score described in Section \ref{sec:model}. Recall that this is the Wasserstein distance between the FPs obtained in the previous step, and a uniform reference vector-histogram; and then the same thing for the TPs. To insure statistical significance of our results, we repeat this exact experiment 500 times, and then represent the histogram of Wasserstein distances as two normalized histograms in Figure~\ref{fig:histogram}.  We note that for convenience of the display, we have subtracted a large constant ($10^5$) from both FP and TP Wasserstein distance histograms -- our tests are translation invariant, so clearly this has no effect on their performance or significance.

The non-overlapping distributions (Figure~\ref{fig:histogram}) indicate that our shape-based GD (we call this Shape GD for short) can indeed separate FPs from TPs. We only show the results for four apps, but Shape GD achieves similar completely separable distributions for 8 of 10 apps in our test -- Yelp and eBay yield partially overlapping distributions which lead to some false positives and negatives in the Shape GD's output. 

The distance between the distributions varies across the apps -- Wikipedia has
the largest separation (Figure~\ref{fig:intro-histogram}) while Walmart's distributions have smaller separation -- however, as long as they can be separated, the performance of Shape GD is unchanged.

As an interesting side note, we observe that the relative distance of the FP and TP distributions from the uniform distribution is not fixed -- the only key is that these distances are different. Indeed, the order depends on an underlying app and LD's properties -- for example, Wikipedia's false positive distribution is closer to the reference vector-histogram, whereas for AVG, Walmart, Buzzfeed and other apps TPs are closer to the reference histogram.

%However, the order of distributions is irrelevant to the GD's detection results
%-- GD only needs to separate TPs and FPs from each other.
%this property of our algorithm does not interfere with its detection results.

To summarize, our experiments with multiple real-world mobile apps  
%we have empirically
confirm that the Shape GD is an accurate and robust method for
distinguishing LD's outputs into true and false positives.

%The large gap between two distributions on the Figure~\ref{fig:histogram} witnesses Shape GD's ability to separate FPs and TPs. Shape GD achieves similar results for all the apps in our corpus, i.e. it can reliably separate LD's TPs and FPs. The only difference across all the experiments resides in the relative order of two distributions. For example, Wikipedia's false positive distribution is closer to the reference vector-histogram. Nevertheless, AVG, Walmart, Buzzfeed and other apps have reverse order of the distributions.

%After choosing an appropriate LD, we proceed to the next logical step -- designing a global detector (GD) for aggregate analysis of alerts raised by LDs.
%
%As we mentioned before, the key difference with the other previous work on CIDS~\cite{seurap, survey ...} resides in the type of information being processed by GD. In comparison to the state-of-the-art CIDS, Shape GD does not aggregate LDs alerts (binary LDs' outputs) -- it reanalyzes feature vectors causing alerts. Also, Shape GD does not need to know the global network topology (e.g. size of a network at every moment of time, possible connections between all nodes and etc) -- local network topology (1-hop neighborhoods) is enough to efficiently detect malware in a community.
%
%When analyzing Shape GD, the first question we want to address is how well Shape GD separates LD's false positives and true positives. 

%To analyze Shape GD's ability to distinguish between FPs and TPs, we do the following experiment: we sample two groups of feature vectors 500 times -- one group from a benign data set and the other one from a malicious data set. Each group contains 5,000 unique feature vectors, i.e. they are sampled without replacement. However, individual benign/malicious groups may overlap. After passing these two groups through an LD, we obtain its FPs and TPs. Then for each FP/TP set we compute Wasserstein distance between the set and the uniform reference vector-histogram. As a result of this experiment, we collect 500 distances between FP/TP sets and the reference histogram, which we represent as a normalized histogram to obtain an empirical estimation of FP/TP distributions (Figure~\ref{fig:histogram}). 
%
%The large gap between two distributions on the figure~\ref{fig:histogram} witnesses Shape GD's ability to separate FPs and TPS. From information-theoretic point of view, we can say that Shape GD is able to extract the information from the underlying data that has been missed by an LD. In the experiments with all the apps in our corpus, we have observed similar results, i.e. Shape GD can reliably separate LD's TPs and FPs. The only difference is which of the two distributions is closer to the reference vector-histogram. For example, for Wikipedia's distribution of FPs is closer to the reference vector-histogram. Nevertheless, AVG, Walmart, Buzzfeed and other apps lead to the reverse arrangement of the distributions.


%Such an approach does not work in the setting where the exact number of nodes in a network fluctuates over time. In many cases, we cannot model such fluctuation, thus we have no estimate of the expected number of nodes in a network. Consequently, classic GD is not able to distinguish between malware spread and fluctuations of the number of false positives due to constantly changing size of a network.

%To overcome such a shortcoming, we have designed a network-oblivious GD. It does not need to know the global topology (e.g. size of a network at every moment of time, possible connections between all nodes and etc). As has been mentioned in the~\ref{algo sec}, our GD needs to have access to the original feature vectors that resulted in alert and local network topology -- 1-hop neighborhood. In this section we compare performance of our GD with classical approach -- count-based GD.

%In this section we compare performance of Shape GD with classical approach -- count-based GD.

%Another, and perhaps more insightful, way of looking at this is to consider the (empirical) probability mass function the feature vectors filtered in two different ways (i) the pmf of feature vectors that correspond to the true positives (real malware activity) of the local detector, and (ii) the pmf of feature vectors that correspond to the false positives of the local detector (misclassifications by the
%local detector). Information theoretic arguments in the higher dimensional feature space – effectively they have different shapes. However, their binary projections in the local detector output space is the same, thus the local detector does not (statistically) distinguish between these two collections. This points toward 
%eigen-filtering -- hypothesis testing in the feature vector space -- instead of simply aggregating outputs of the LDs.

%It is not surprisingly that the distribution of distances between FPs and the reference histogram is shifted to the left because we build a reference histogram to roughly approximate this distribution. In this setting the distances between TPs and the uniform histogram are no less than the distances between FPs and the reference histogram. 



%\begin{figure}[tbp]
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/pure_shape/NO_censorship_w_10_prctile_10.pdf}\par
%%\caption{\textit{(Wikipedia) Detection rate scales as log of the number of nodes in %the network.}}
%\label{fig:shape_vs_count}
%\end{figure}
%
%\begin{figure*}[t]
%\begin{minipage}[tbp]{0.3\linewidth}
%%   \begin{flushleft}
%   \includegraphics[width=\textwidth]{figs/pure_shape/censorship_0_3_w_10_prctile_1.pdf}\par
%   %\caption*{{} }
%   \label{fig:count}
%%   \end{flushleft}
%\end{minipage}
%%\hfill
%\begin{minipage}[tbp]{0.3\linewidth}
%%   \begin{flushright}
%   \includegraphics[width=\textwidth]{figs/pure_shape/censorship_0_3_w_10_prctile_10.pdf}\par
%   %\caption*{{Angry Birds game + click fraud}} 
%   \label{fig:ab-2}
%%   \end{flushright}
%\end{minipage}
%\begin{minipage}[tbp]{0.3\linewidth}
%%   \begin{flushright}
%   \includegraphics[width=\textwidth]{figs/pure_shape/censorship_0_3_w_10_prctile_30.pdf}\par
%   %\caption*{{Angry Birds game + click fraud}} 
%   \label{fig:ab-2}
%%   \end{flushright}
%\end{minipage}
%\caption{(Wikipedia) Effect of percentile threshold}
%\label{fig:pure_shape}
%\end{figure*}
%
%
%First, we compare detection rate of Shape and Count~\ref{fig:shape_vs_count}. In this experiment, we use normalized histograms for the Shape detector. Shape starts working at 14.4\% level, while Count starts working at 3.8\%. The error bars correspond to 10 and 90 percentile respectively.
%
%Second, we compare the effect of threshold (aka percentile parameter) on detection rate. When varying the detection confidence (consequently, FP rate) from 1\% to 30\%, detection changes from 27\% to 3.7\%~\ref{fig:pure_shape}


==> results/shape_vs_count.tex <==
\begin{figure*}[t]
\begin{minipage}[tbp]{0.33\linewidth}
  \centering
%   \begin{flushleft}
   \includegraphics[width=\textwidth]{figs/count_vs_pure_shape/no_censoring/random.pdf}\par
   %\caption*{{} }
   \subcaption{Random graph}
   \label{fig:shape_vs_count_random}
%   \end{flushleft}
\end{minipage}
%\hfill
\begin{minipage}[tbp]{0.33\linewidth}
  \centering
%   \begin{flushright}
   \includegraphics[width=\textwidth]{figs/count_vs_pure_shape/no_censoring/grid.pdf}\par
   %\caption*{{Angry Birds game + click fraud}} 
  \subcaption{Grid graph}
   \label{fig:shape_vs_count_grid}
%   \end{flushright}
\end{minipage}
\begin{minipage}[tbp]{0.33\linewidth}
  \centering
%   \begin{flushright}
   \includegraphics[width=\textwidth]{figs/count_vs_pure_shape/no_censoring/social.pdf}\par
   %\caption*{{Angry Birds game + click fraud}} 
   \subcaption{Real network}   
   \label{fig:shape_vs_count_social}
%   \end{flushright}
\end{minipage}
\caption{(Wikipedia) Shape GD vs Count GD. 
%(Count vs Shape -- no Censoring) Random -- Grid -- Social graphs (10\% percentile)
}
\label{fig:shape_vs_count}
\end{figure*}

We refer to Count GD as the algorithm that relies on increased
alert-count inside specific communities, in order to declare a global
infection (see also \cite{Dash2006,Seurat2004} for related approaches). In contrast to Count GD, our approach, Shape GD, does not critically need the number of nodes in the network. Indeed, when this information is not available, {\em Count GD cannot work}. But if we do have this information, the idea of Count GD can be useful. In this section, we compare Shape GD and Count GD in the setting most favorable to Count GD -- fixed and known graph topology. Our results show that even here, Shape GD does almost as well as Count GD. This suggests that in cases where we can reasonably expect to know the graph (and hence the total number of nodes), combining Count GD and Shape GD would give the best results. On the other hand, if the total number of nodes is not known, Shape GD is our only recourse.

We now describe in detail our experiments that lead to the results summarized in the previous paragraph. We quantify the ``price'' of such flexibility by comparing Shape and Count GDs' detection accuracy by running them on a random network, a grid, and a social network.

\ignore{
The training procedure for Shape GD and Count GD is identical: 1) choose a
low-dimensional basis; 2) project benign training data set onto the chosen
basis and compute LD's false positives; 3) appropriately discretize the data
and convert it into vector-histogram representation; 4) compute community
score; and 5) define a {\em detection threshold} for the GDs by fixing a 
false positive rate. }
%error
%bound.\todo{check for consistency: error bound -- false positive}


We allocate a training data set of 11,000 benign feature vectors (FVs) for each
app (i.e., over 3 hours of real usage per app).  To represent data in the form
of vector-histograms we need to determine optimal disretization, i.e., the
number of bins and their edges.
%These parameters are associated with a GD and once being set, they never get
%updated. 
We choose these parameters by passing the benign training set FVs through LDs
on each node to obtain false positive FVs, remove points below and above
1\%/99\% percentile respectively, and choose the number of bins proportional to
the square root of the number of suspicious samples.  Experiments show that 50
bins is an adequate number since the number of suspicious feature vectors is
around 2500 (out of 11000 samples, based on the LD's false positive rate).  We
then add two extra bins to represent data points below the lower bound and
above the upper bound.

Note that a GD is not constrained to use the same basis as LD. 
In our experiments, 
%we use different bases for both. 
although both GDs and LDs use the same FE
algorithm -- histogram of system calls -- and apply PCA to reduce
data to 10 dimensions,  GDs receive only the feature vectors that
lead to alerts by LDs. 
%and projects all suspicious feature vectors on top 10
%principal components.

The actual training procedure consists of 300 iterations. On each iteration we
sample without replacement a subset of 5,500 feature vectors from the
previously allocated set, pass it through an LD, obtain false positive FVs,
project them on the basis chosen above, discretize using the corresponding
bin edges, and compute a community score for the chosen FV-subset. We
repeat this iteration 300 times to determine the range of
community scores (based on the parameter $\gamma$ in Section~\ref{sec:model})
outside of which the GD declares a community as infected.
GDs thus act like anomaly detectors, and the key difference between Count and Shape 
GDs is that Count relies on the number of alerts, where as Shape GD goes back to the feature vectors and then uses the Wasserstein distance community score.

\ignore{
if its
score is outside the range. The range depends on the confidence parameter
$\gamma$ (sec.~\ref{algo_description}). In our case the upper bound of the
range is defined as $\gamma/medium FP-Score$ percentile, by analogy the lower
bound is $(100-\gamma)/medium\ FP-Score$ percentile. Thus, if in the deployment
mode GD finds a community score to be outside the range and labels a community
as infected, then the expected probability of error is $100-\gamma/medium\
FP-Score$. Count GD's training procedure is almost identical -- instead of
capturing the shape of false positive distribution, it captures the number of
alerts.  \mikhail{i could formally describe this if we need}
}

After training Shape and Count GD, we run both detectors on the three networks
and show the results for Wikipedia in 
%networks with different topologies:  random graph, a grid graph, and a social
%network 
Figure~\ref{fig:shape_vs_count}. The plots in the top row characterize
performance of Shape GD, while the ones at the bottom show behavior of Count
GD. The horizontal axis depicts infection rate (ground truth), i.e., the number
of infected nodes in a network, the vertical axis plots community scores. The
blue line shows the average community score for benign FV-sets obtained during
the training procedure. The red line corresponds to the community score
assigned to the groups of suspicious FVs. We set false positive rate $\gamma$
to be 10\% of  for each experiment. To show this
(Figure~\ref{fig:shape_vs_count}), we draw error bars that correspond to 10\%
and 90\% percentile community score values. For each discrete step in the
malware propagation process, we compute the community score of suspicious FVs
sent by LDs to GD for classification. Thus the earliest time step at which the
red curves 
achieve complete separation from the blue curves 
determines the GD's {\em detection threshold} (in terms of number of compromised nodes).

When comparing GDs' performance on random and grid networks, we see that grid
structure results in earlier detection (Shape GD: 8.8\% and 4.6\%; Count GD:
8.8\% and 3\% respectively) due to high and regular local connectivity.  In the
social network graph, Shape GD achieves the worst performance -- 14.4\% across
all network topologies, while the Count GD starts detecting malware at 2.4\%
level (the best result for Count GD). %This difference may be caused by \todo{Why?}.

In summary, the robustness of Shape GD leads to a higher detection threshold in
comparison to Count GD. Hence, it is possible to develop a hybrid GD that
incorporates both Shape and Count detectors to achieve the earliest detection
in a network with fixed topology and also cover cases when network nodes may
randomly switch on/off.

%To compare Shape GD with Count GD, %%we use both of them to detect malware spread over the network~\ref{fig:counts_vs_shape}. Even if we designed our system to be network-oblivious -- size of the network is unknown -- in this experiment we assume that network has a constant size, otherwise we would be unable to use Count-based GD.

%In this experiment, $\alpha=10%$, i.e., error bars correspond to 10- and 90- percentiles. The horizontal axis depicts infection rate, i.e., the number of infected nodes in the network. And for each discrete step in the malware propagation process we compute the community score of suspicious data transmitted by LDs to GD for classification.

%The blue line shows median distance between a group of false positives and a uniform reference histogram. The red line correspond to the community score assigned to the groups of suspicious data. Its error bars are 10- and 90- percentiles. We say that GD is able to detect malware if red and blue error bars do not overlap.

%Each subplot corresponds to one of the underlying network topologies that we consider in our experiemnts: random graph, grid graph and real social network. The subplots in the top row shows how Shape GD reacts to malware propagation, while the subplots at the bottom show the same for Count-based GD. 

%When we compare GDs' performance on random and grid networks, we see that grid structure results in earlier detection (Shape GD: 8.8\% and 4.6\%; Count GD: 8.8\% and 3\% respectively) due to high local connectivity. If compare random and grid graphs with a social network graph, we can notice that Shape GD achieves the worst performance -- 14.4\%, while the Count GD starts detecting malware at 2.4\% level. This difference may be caused by ???. 

%As malware gets propagated over the network, Count GD's malicious score grows as a linear function as one may expect. At the same time, Shape GD's malicious score resembles a logarithmic function that slowly stabilizes.



==> results_symantec.tex <==
We now quantify how \sysname concentrates malware in Symantec's Wine dataset
into neighborhoods and identifies malicious files and infected machines with
far lower false positives than using LDs~\cite{Symantec-LD} alone (while losing
only a few true positive malware that didn't get captured into neighborhoods).
On the other hand, the state-of-the-art downloader-graph based
detector~\cite{tudor-1,tudor-2} is limited to detecting downloaders (to reduce
false positives) -- in comparison, \sysname has significantly higher
true-positives at a comparable false positive rate. 

In addition, neighborhoods and shape together are good predictors of malware
behavior -- hence \sysname does not have to wait until the entire sequence of
malware payloads have been downloaded to declare a downloader or machine as
malicious. We find that on average, \sysname can identify a file as malicious
only \todo{20} days after it entered the Wine dataset and \todo{300} days
before VirusTotal confirms it as malware.  Tables~\ref{table:shape-file}
and~\ref{table:shape-machine} summarize these results.


\subsection{Neighborhoods Concentrate Malware}
\label{sec:nbd-conc}

We now summarize the operating points of the local detector (LD) that analyzes
files, the domain name classifier used to identify suspicious domains and form
neighborhoods, and the neighborhood-level detector that classifies the shape of
a suspicious neighborhood's LDs' alert-FVs. \mohit{Combined ROC plot}

Each LD comprises two parts -- feature extraction
described in Section~\ref{sec:algorithm} and an XGBoost binary classifier.  
We train the LD on the set of 2.6 million VirusTotal reports using 10-fold
cross-validation.  LD achieves 97.61\% are-under-the-curve metric
(Figure~\ref{fig:ld_roc}), and we chose an operating point of 5.0\% false
positive rate and 90.47\% true positive rate.  A 5.0\% false positive rate
yields over 1 million (of 20.7M) misclassified files -- \sysname's task is to
retain as many LD true positives as possible while improving the false positive
rate. 

We pick the domain name classifier's operating point to be 19.03\% false
positive and a 95.41\% true positive rate.  The domain name classifier labels
as suspicious any domain that serves at least one malicious file -- since
domains often serve many benign files as well, the classifier ends up favoring
true positives over false positives. We note that the domain name classifiers
can be improved significantly~\cite{cite-dns-classifiers} -- exploiting
information that is not available in the Symantec Wine dataset -- but we show
that \sysname can use even this weak detector to create neighborhoods,
and then use the neighborhoods' shape to dramatically improve upon LDs'
false positives.

%Even though the domain name classifier is not deployable by itself due its
%high false positive rate, it is an integral part of \sysname and it 
In particular, the domain name classifier helps \sysname efficiently filter out
domains that are unlikely to distribute malicious files.  It removes from
further consideration 68.62\% (214,884 out of 313,133) completely benign
domains that are responsible for  delivering 80.70\% (16,222,941 out of
20,103,211) benign files.  And at the same time the classifier retains 75.86\%
(30,448 out of 40,134) of malicious domains responsible for delivering 88.31\%
(94,457 out of 106,959) malicious files.

Using domain classifier to create neighborhoods and using shape-based features
to train a neighborhood-level classifier, \sysname achieves 96.13\% AUC score.
We choose an operating point of 5\% FP rate and 91.83\% TP rate.

Note the original malware concentration in the Wine dataset is only 0.663\%.
Pruning the files downloaded from benign domains leads to the 14.3 times
increase (9.49\%) of the neighborhood infection rate (upper
plot~\ref{fig:nbd_concentrator}). However, if we closely look at the upper
histogram~\ref{fig:nbd_concentrator}, we see the spike on the left-hand side,
which corresponds to the large number of neighborhoods with less than 1\% of
malware files in them. 

We use the neighborhood classifier to remove from further consideration low
infected neighborhoods.  It dramatically changes the distribution of
neighborhood infection rates, i.e. the peak shifts to the right -- from 1\% to
5\% (lower plot~\ref{fig:nbd_concentrator}).  The neighborhood classifier
brings the average neighborhood malware rate from 9.49\% (before filtering) to
24.6\% value, thus, it achieves 2.59 times increase in malware concentration.
Neighborhoods after the neighborhood filtering algorithm have 37.1 times higher
malware concentration than the Wine dataset.

\begin{figure}[tbp]
   \vspace{-0.0in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/symantec/nbd_effect/nbd_effect_2.eps}\par
   \caption{NBD algorithm acts as a malware concentrator. Top plot: distribution of nbds based on their infection rate.
   Bottom plot: Distribution of NBDs after filtering out benign and low-infected NBDs. The NBD algorithm keeps
   only highly infected NBDs.}
   \vspace{-0.2in}
\label{fig:nbd_concentrator}
\end{figure}

\subsection{\sysname Detection Results}
\label{sec:symantec-detection}




%
%\subsection{Count-GD is Fragile}
%\label{sec:symantec-count}
%
%\begin{figure}[t]
%\begin{minipage}[tbp]{0.24\linewidth}
%  \includegraphics[width=\textwidth]{figs/symantec/count-fragility/nbd-count-gd-fragility.eps}\par
%   \label{fig:ld_roc}
%\end{minipage}
%\begin{minipage}[tbp]{0.24\linewidth}
%   \includegraphics[width=\textwidth]{figs/symantec/count-fragility//file-count-gd-fragility.eps}\par
%   \label{fig:domain_roc}
%\end{minipage}
%\caption{Symantec Count-GD fragility .Left - Right: NBD vs File results.}
%\label{fig:symantec-count-gd-fragility}
%\end{figure}




%\ignore{
1. Evaluation of NBDs' role in malware detection process (an increase of malware concentration)

2.  Use of NBD objects: \\
2a. Run LDs within suspicious NBDs \\
2b. Select machines for deeper inspection within suspicious NBDs using greedy algorithm

3. [Mikhail \& BumJun] Aggregated statistics computed over the entire dataset

4. Temporal statistics computed for each detection window

4.5 replacing ML algorithms with ideal ones

5. Real-time malware removal process\\
   Estimate how many security incidents could have been prevented
   
6. [BumJun] Evasive malware\\
   Evaluate performance of the entire system on the evasive malware
   Add evasive modifications to downloader graphs to defeat CCS'15 detector and evaluate the current detector on evasive malware
   
7. [BumJun] Deep dive into the structure of suspicious NBDs\\
   Deep analysis of suspicious NBDs (~10K -- 100K nbds)
   What malware campaigns our NBDs catch


We structure the results section as follows: first, we analyze performance of individual 
components and describe dataset properties that affect the choice of algorithms' parameters,
second, we focus on the real-time malware detection, and finally we discuss 
overall malware detection results.

\subsection{Symantec Count-GD fragility}
\begin{figure*}[t]
\begin{minipage}[tbp]{0.24\linewidth}
  \includegraphics[width=\textwidth]{figs/symantec/count-fragility/nbd-count-gd-fragility.eps}\par
   \label{fig:ld_roc}
\end{minipage}
\begin{minipage}[tbp]{0.24\linewidth}
   \includegraphics[width=\textwidth]{figs/symantec/count-fragility//file-count-gd-fragility.eps}\par
   \label{fig:domain_roc}
\end{minipage}

\caption{Symantec Count-GD fragility .Left - Right: NBD vs File results.}
\label{fig:symantec-count-gd-fragility}
\end{figure*}



\subsection{Classifiers}
\sysname employs three binary classifiers for soft decision making: a local detector, 
a domain name classifier and a neighborhood classifier.
In this section, we describe their performance and their contribution towards
overall malware detection. When training these classifiers, we follow the parameter tuning
approach outlined in Section~\ref{}.
%And after that we analyze the lifespane of
%malicious domains in the Wine dataset, which is important for choosing an appropriate length
%of the neighborhood time window.

\begin{figure}[tbp]
\begin{minipage}[tbp]{0.48\linewidth}
  \includegraphics[width=\textwidth]{figs/symantec/LD_domain_classifier_roc_combined.eps}\par
   \label{fig:ld_roc}
\end{minipage}
\begin{minipage}[tbp]{0.48\linewidth}
   \includegraphics[width=\textwidth]{figs/symantec/nbd_ld_roc/nbd_roc.eps}\par
   \label{fig:nbd_roc}
\end{minipage}
\caption{Receiver operating curve of local detectors; Receiver operating curve of a domain name classifier; Receiver operating curve of a domain name classifier weighted with files associated with URLs; NBD classifier's ROC. (ROC of the algorithm that filters out low infected NBDs.}
\label{fig:roc-curves}
\end{figure}


%\begin{figure*}[t]
%\begin{minipage}[tbp]{0.24\linewidth}
%  \includegraphics[width=\textwidth]{figs/symantec/LD/ld_roc.eps}\par
%   \label{fig:ld_roc}
%\end{minipage}
%\begin{minipage}[tbp]{0.24\linewidth}
%   \includegraphics[width=\textwidth]{figs/symantec/domain_name_classifier/domain_roc.eps}\par
%   \label{fig:domain_roc}
%\end{minipage}
%\begin{minipage}[tbp]{0.24\linewidth}
%   \includegraphics[width=\textwidth]{figs/symantec/domain_name_classifier/domain_file_roc.eps}\par
%   \label{fig:domain_file_roc}
%\end{minipage}
%\begin{minipage}[tbp]{0.24\linewidth}
%   \includegraphics[width=\textwidth]{figs/symantec/nbd_ld_roc/nbd_roc.eps}\par
%   \label{fig:nbd_roc}
%\end{minipage}
%\caption{Receiver operating curve of local detectors; Receiver operating curve of a domain name classifier; Receiver operating curve of a domain name classifier weighted with files associated with URLs;NBD classifier's ROC. (ROC of the algorithm that filters out low infected NBDs.}
%\label{fig:roc-curves}
%\end{figure*}

%\begin{figure}[tbp]
%   \vspace{-0.0in}
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/symantec/LD/ld_roc.eps}\par
%   \caption{Reciever operating curve of local detectors.}
%   \vspace{-0.2in}
%\label{fig:ld_roc}
%\end{figure}

\noindent \textbf{Local detectors.}
We start with the evaluation of local detectors (Section~\ref{sec:algorithm}).
Each local detector algorithm comprises two parts -- feature extraction described in
Section~\ref{sec:algorithm} and an XGBoost binary classifier.
We train a local detector on the set of 2.6 million VirusTotal reports using 10-fold cross validation.% and we plot the ROC curve on the Figure~\ref{fig:ld_roc}.
%Following the parameter tuning approach outlined in Section~\ref{}, we 
LD achieves 97.61\% are-under-the-curve metric (Figure~\ref{fig:ld_roc}). 
And we chose the operating point of 5.0\% false
positive rate and 90.47\% true positive rate. Note due to the high number of benign files
in the dataset, 5.0\% false positive rate corresponds to more than 1 million  misclassified
files, which is likely to prevent deployment of such local detectors in practice.
Throughout the rest experiments we use out-of-fold predictions made by such a classifier.


%\begin{figure}[tbp]
%   \vspace{-0.0in}
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/symantec/domain_name_classifier/domain_roc.eps}\par
%   \caption{Reciever operating curve of a domain name classifier.}
%   \vspace{-0.2in}
%\label{fig:domain_roc}
%\end{figure}

%\begin{figure}[tbp]
%   \vspace{-0.0in}
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/symantec/domain_name_classifier/domain_file_roc.eps}\par
%   \caption{Reciever operating curve of a domain name classifier weighted with files associated with URLs.}
%   \vspace{-0.2in}
%\label{fig:domain_file_roc}
%\end{figure}

%\begin{figure}[tbp]
%   \vspace{-0.0in}
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/symantec/nbd_ld_roc/nbd_roc.eps}\par
%   \caption{NBD classifier's ROC. (ROC of the algorithm that filters out low infected NBDs.)}
%   \vspace{-0.2in}
%\label{fig:nbd_roc}
%\end{figure}

\textbf{Domain name classifier.} To analyze performance of the domain name
classifier (Algorithm~\ref{algo:domain_classifier}), we employ the following
two metrics: a traditional receiver operating curve (ROC) and a file-weighted
receiver operating curve (ROC).  We train and evaluate the classifier on 251
thousand VirusTotal domain reports using 10-fold cross validation.

Despite intensive parameter tuning, the classifier achieves only 83.80\% AUC
(Figure~\ref{fig:domain_roc}).  Therefore, its low accuracy makes it unusable
by itself in practice.

The main reason for the classification algorithm being inaccurate is the
conservative approach to labeling domains, i.e.  an entire domain is considered
malicious if it serves at least one malware sample. However, only a single
webpage may be compromised.  In such cases, the features extracted from
VirusTotal domain reports contradict domain labels -- the features represent
benign nature of a domain, while its label is malicious.  Thus, they do not
carry information necessary for the classifier to predict possibility of some
webpages being compromised.  Such an issue can be addressed by working with
individual URLs rather than domain names, but the Wine dataset lacks such data.
Also an analysis of a webpage content together with URL arguments could improve
classifier's performance.

Note we deliberately employ conservative approach to labeling domains in order
not to miss domains capable of distributing malware.

%In some cases domain labeling, which is done based on Wine dataset, may contradict domain attributes in the VT report because
%a single compromised webpage may not significantly affect the benign nature of the domain. Therefore, it's hard for the classifier
%to make correct (conservative) predictions based on a limited information present in the VT reports.

For \sysname to achieve good overall detection results, the domain name
classifier needs to prioritize correct labeling of domains distributing
majority of the files.  To analyze this a property, we introduce a file-level
ROC curve~\ref{fig:domain_file_roc}, i.e. for each value of the classifier's
threshold the true positive rate is the number of malicious files distributed
by the domains labeled as malicious by the classifier, and, respectively, the
number of benign files distributed by those domains is the false positive rate.
%where each malicious domain is weighted by the total number of malicious
%samples that it servers and each benign domain is weighted by the total number
%of benign files that it distributes.

The file-level ROC has higher steep at the beginning than the traditional ROC.
And its AUC metric (91.58\%) also is significantly higher than the analogous
parameter of the ROC curve because the classifier correctly labels domains
distributing large number of files due to their VirusTotal attributes being
consistent with the domains' essence.  However, the classifier often mislabels
domains that distribute few malware samples due to inconsistency between
features and labels, which may often occur due to short lived compromises.

Because \sysname eventually operates on files rather than domain names, we
select the operating point using the file-level ROC~\ref{fig:domain_file_roc}.
To capture large number of malware sample, \sysname needs a conservative domain
name classifier -- the one that can identify as many malicious domains as
possible. Thus, we adjust the classifier's threshold to achieve higher than
95\% TP rate. Specifically, we choose the following operating point: 19.03\% FP
rate and 95.41\% TP rate.

Even though the domain name classifier is not deployable by itself due its high
false positive rate, it is an integral part of \sysname and it lets \sysname
efficiently filter out domains that are unlikely to distribute malicious files.
Specifically, it removes from further consideration 68.62\% (214,884 out of
313,133) completely benign domains that are responsible for  delivering 80.70\%
(16,222,941 out of 20,103,211) benign files.  And at the same time the
classifier retains 75.86\% (30,448 out of 40,134) of malicious domains
responsible for delivering 88.31\% (94,457 out of 106,959) malicious files.

It is worth noting that prior work presents more accurate URL- or Domain-level
classifiers~\ref{}, however, it exploits the information that is not available
in the Wine dataset.


\textbf{Neighborhood classifier.} The role of the neighborhood classifier is to
discover neighborhoods with malware concentration higher than in the underlying
dataset.  And it achieves this effect by exploiting transient correlations
between file downloads.

Specifically, we design а classifier such that it detects neighborhoods
containing more than 5\% of malicious files. We empirically found that if such
threshold is lower than 5\%, then the neighborhood effect becomes less
noticeable. In the extreme case of 0\% threshold, the neighborhood classifier
will supply all neighborhoods and all files in the system to the deep analysis
framework, which is equivalent to having no neighborhood classification
algorithm.  In the other extreme case of high threshold values, the
neighborhood algorithm will negatively impact recall (true positive rate) of
the overall system because it will aggressively filter out malicious
neighborhoods -- the neighborhoods whose infection rate is below the threshold.

As we see on the ROC plot (Figure~\ref{fig:nbd_roc}), the neighborhood
classifier mostly correctly classifies neighborhoods. The classifier achieves
96.13\% AUC score.  And we choose the following operating point: 5\% FP rate
and 91.83\% TP rate.

Note, at this point we can not make any conclusions about the performance of
the entire malware detection framework because we do not know how many
malicious and benign files are covered by the neighborhoods labeled as
malicious.  We noticed that due to correlation of LDs' FPs the files included
in the 5\% of misclassified domains largely overlap rather being completely
distinct.


\textbf{Neighborhood effect.}
\begin{figure}[tbp]
   \vspace{-0.0in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/symantec/nbd_effect/nbd_effect_2.eps}\par
   \caption{NBD algorithm acts as a malware concentrator. Top plot: distribution of nbds based on their infection rate.
   Bottom plot: Distribution of NBDs after filtering out benign and low-infected NBDs. The NBD algorithm keeps
   only highly infected NBDs.}
   \vspace{-0.2in}
\label{fig:nbd_concentrator}
\end{figure}

Now we turn our attention to quantifying the neighborhood effect and its impact
on the overall malware detection. The neighborhoods labeled as malicious are
likely to contain more than 5\% of malicious files, but at the same time such
neighborhoods need to achieve high total malware coverage.

Note neighborhood filtering increases malware concentration in two steps
(Algorithm~\ref{}).  First, it filters out files downloaded from benign
domains, second, it further filters out neighborhoods containing low number of
malicious files.  To analyze these effects, we plot the distribution of
neighborhood malware rates before after the neighborhoods being formed (upper
figure~\ref{fig:nbd_concentrator}) and after mostly benign neighborhoods being
filtered out (lower plot~\ref{fig:nbd_concentrator}).

Note the original malware concentration in the Wine dataset is only 0.663\%.
Pruning the files downloaded from benign domains leads to the 14.3 times
increase (9.49\%) of the neighborhood infection rate (upper
plot~\ref{fig:nbd_concentrator}). However, if we closely look at the upper
histogram~\ref{fig:nbd_concentrator}, we see the spike on the left-hand side,
which corresponds to the large number of neighborhoods with less than 1\% of
malware files in them. 

We use the neighborhood classifier to remove from further consideration low
infected neighborhoods.  It drammatically changes the distribution of
neighborhood infection rates, i.e. the peak shifts to the right -- from 1\% to
5\% (lower plot~\ref{fig:nbd_concentrator}).  The neighborhood classifier
brings the average neighborhood malware rate from 9.49\% (before filtering) to
24.6\% value, thus, it achieves 2.59 times increase in malware concentration.
Neighborhoods after the neighborhood filtering algorithm have 37.1 times higher
malware concentration than the Wine dataset.

If we look at the concrete numbers, we see that the number of neighborhoods
with the infection rate less than 1\% drops by 437.6 times (from 8752 on the
upper plot to 20 on the lower plot). Overall, the neighborhood classifier
reduces the number of low infected neighborhoods (neighborhoods with less than
5\% of malicious files) by 22.9 times (from 13,735 to 599).


\subsection{Lifespan of malicious domains.}

\begin{figure}[tbp]
   \vspace{-0.0in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/symantec/domain_lifespan/lifespan.eps}\par
   \caption{Distribution of the lifespan of malicious domains. 
   After removing domains serving only a single malicious file,
   the average lifespan goes up to 157 days. And we set NTW to 150 days.}
   \vspace{-0.2in}
\label{fig:domain_lifespan}
\end{figure}
Before discussing to detection results, we analyze lifespan of compromised domains to choose an appropriate
duration of the neighborhood time window (NTW).
We define the lifespan of a malicious domain as a time interval between the first malware sample and 
the last malware sample distributed by the domain.
In reality, the domain may be compromised multiple times within its lifespan. Unfortunately, the Wine
dataset lacks information necessary to distinguish between independent compromises.
However, such a coarse grain definition of lifespan allows us conservatively estimate how long a domain
remains compromised or how long a malicious domain remains active if its sole purpose is to distribute malware.

The histogram~\ref{fig:domain_lifespan} shows the distribution of domain lifespan in \textit{log scale}. 
We split the range of lifespan parameter (from 0 days up to 1822 days) into 100 bins (the horizontal axis).
And for each bin we compute the probability of a lifespan value to fall into it (the vertical axis).
We use the log scale to better visualize the long-tale distribution of lifespan values.

The large portion of malicious domains, specifically, 62.4\%, in the Wine data set serves only a single malicious file.
We are likely to observe such an effect due to the Wine dataset being incomplete, i.e. it captures not all malicious downloads, 
and also due to hackers actively employing domain generation algorithms~\cite{usenix-dg-paper} that register domains serving few malicious files.
Across the data set, the average lifespan of malicious domains is 59 days and the median is 0 days. If we remove domains serving only a single malicious file, 
the average lifespan goes up to 157 days and median is 44 days. 

Therefore, we consider file downloads within 150 days time window correlated, and set the neighborhood time window in our experiments to 150 days.
However, if we had more detailed information on individual domain compromises in the dataset, we would be able more accurately estimate
the average lifespan and, thus, the average size of a neighborhood time window within which malicious downloads are actually correlated. And more accurate estimation of the NTW length would improve overall
malware detection.
Thus, gathering more information would increase accuracy of our neighborhood formation algorithm.





\subsection{Real-Time Detection}
In this section we analyze the real-time detection properties of \sysname and compare it
against other detectors.
Specifically, we focus our analysis on the following two characteristics -- how well
\sysname detects malicious files and how well it detects infected machines, i.e. 
machines that have downloaded at least one malicious file.

To perform real-time analysis, we replay the 5-year long history of download events in the Wine dataset 
(each event has a timestamp associated with it)
and execute \sysname every 30 days. In our experiments we found that
shorter period between consecutive runs of \sysname does not significantly affect
results, it only improves time to detection and early detection parameters~\ref{sec:}. 
We intentionally stick to a 30-day period between consecutive runs of \sysname{} 
to keep execution time ($\sim$12 hours) and resource consumption manageable.

We compare real-time behavior of three detectors -- local detectors~\cite{vt_report_classification}, 
a neighborhood detector, which conservatively labels all the files within a malicious neighborhood as malicious, 
and \sysname that comprises of the neighborhood classifier and local detectors 
-- in terms of precision, recall, and F-1 score, which is a commonly used way to combine precision and recall.

$
\displaystyle
\begin{aligned}
Precision = \frac{TP}{TP + FP}
\end{aligned}
$

$
\displaystyle
\begin{aligned}
Recall = \frac{TP}{TP + FN}
\end{aligned}
$

$
\displaystyle
\begin{aligned}
F1 = 2 \cdot \frac{precision\cdot recall}{precision+ recall}
\end{aligned}
$



\subsubsection{File-level real-time detection}

\begin{figure*}[t]
\begin{minipage}[tbp]{0.24\linewidth}
   \includegraphics[width=\textwidth]{figs/symantec/temporal_analysis/file_stat.eps}\par
   \label{fig:temporal-file-stat}
\end{minipage}
\begin{minipage}[tbp]{0.24\linewidth}
   \includegraphics[width=\textwidth]{figs/symantec/temporal_analysis/file_ld_precision_recall.eps}\par
   \label{fig:temporal-file-stat-LD}
\end{minipage}
\begin{minipage}[tbp]{0.24\linewidth}
   \includegraphics[width=\textwidth]{figs/symantec/temporal_analysis/file_nbd_precision_recall.eps}\par
   \label{fig:temporal-file-stat-NBD}
\end{minipage}
\begin{minipage}[tbp]{0.24\linewidth}
   \includegraphics[width=\textwidth]{figs/symantec/temporal_analysis/file_shape_gd_precision_recall.eps}\par
   \label{fig:temporal-file-stat-Shape}
\end{minipage}
\caption{File-level dynamic behavior. Left to Right: Raw statistics, LD-level stat, NBD-level stat, Shape-LD - level stat}
\label{fig:temporal-file-stat-minipage}
\end{figure*}

\mikhail{log scale?}
\textbf{File statistics.}
We start with the analysis of the temporal distribution 
of the download events (Figure~\ref{fig:temporal-file-stat}) to visualize file downloads over time.
As \sysname operates on a 150-day long NTW, 
for each timestamp we compute the total number and the number of malicious file downloads 
within the previous 150 days (upper plot~\ref{fig:temporal-file-stat}).
For example, the value on the figure~\ref{fig:temporal-file-stat} labeled as 01/2011 includes file
downloads from 06/2010 till 01/2011.
We also visualize the total number of distinct downloads and
the number of distinct malicious downloads (bottom figure~\ref{fig:temporal-file-stat}).

Every point on these curves characterizes the number of files \sysname has to deal 
in the real-time malware detection mode. Benign files constitute the large portion of the files 
in the Wine dataset, i.e. the difference between the black and the red curves. 
And \sysname exploits this by efficiently filtering out benign files.

When taking a deeper look at the plots, we notice that file downloads in the 
Wine dataset exhibit a nonuniform pattern over time. 
The total number of downloads increases from January 2008 and reaches its peak (51 million downloads per NTW)
within the NTW ending in October 2010, and after that it decreases over time.
The temporal pattern of distinct downloads slightly differs -- 
intensity of distinct downloads reaches a flat plato (4.74 million per NTW) in September 2010 and
remains on the approximately same level until April 2011.
However, malicious files are responsible for only
the small percentage of all downloads -- at most 1.43 million total malicious downloads and at most 27 thousand
unique malicious downloads.

%At the peak, the number of downloads reaches 51 million downloads (total) and
%4.74 million of distinct downloads per a NTW. However, malicious files constitute only
%small percentage of all downloads -- 1.43 million malicious downloads and 27 thousand
%unique malicious files.

Note the low intensive ends of the distribution impose an obstacle for \sysname 
because of the insufficient number of correlated file downloads.
And due to this reason we discard file downloads before June 2008.
Therefore we run \sysname the first time on the neighborhood window spanning 
the interval from 06/2008 until 01/2009 and label the results with the `01/2009' timestamp.
% due to insufficient data because
%\sysname is not able to robustly discover correlations between file downloads.

\textbf{Local detectors.}
When we analyze analyze the temporal behavior of local detectors~\ref{fig:temporal-file-stat-LD}, we
notice anti-correlation between the total number of unique downloads and LDs' precision.
The peak of unique downloads corresponds to the large number of benign downloads.
Therefore, when LDs process them, they output a large number of false positive alerts, 
which results in a precision drop (it drops down to less than 5\% level). 
However, the recall stays in the range of 84\% -- 95\% 
because it depends only on LDs' ability to detect malicious files. 
F-1 score leans more towards precision than to recall, 
that's why LDs have mostly low F-1 score over the large period of time (between 9\% and 66\%).

\textbf{Neighborhood detector.}
Before analyzing \sysname real-time detection, we briefly discuss the neighborhood detector's detection performance.
We assume that the neighborhood detector~\ref{fig:temporal-file-stat-NBD} labels all the files within malicious
neighborhoods as malicious.
As local detectors, the neighborhood detector suffers from low precision as well, however,
the underlying cause is different. The neighborhood classifier is supposed to label as
malicious neighborhoods containing more than 5\% of malicious files. Usually, most files
in a neighborhood are benign. Thus, when the neighborhood detector 
conservatively labels all the files as malicious, it suffers from high false positive rate,
consequently, low precision.
Hence, the neighborhood detector is designed to be conservative.
Also the neighborhood detector inadvertently filters out some malicious files, which leads 
to lower than LDs' recall.

%The goal of the neighborhood algorithm is to filter out benign files and retains as many as
%possible malicious files, thus it is designed to have high false positive rate because
%neighborhoods usually include many benign files. The neighborhood effect comes at the price
%of slightly lower recall~\ref{fig:temporal-file-stat-NBD} because neighborhoods filter out
%some malicious files as well, and low precision due to the high number of benign files included into the %neighborhoods.

\textbf{\sysname{}.}
Comparing to local detectors, \sysname boosts precision and inherits slightly 
lower recall from the neighborhood classifier because it aggregates LDs' predictions 
collected only across suspicious neighborhoods (Figure~\ref{fig:temporal-file-stat-Shape}). 
The reason \sysname achieves high precision is because it has much lower false positive rate 
as many benign files are already filtered out by
the neighborhood detector. And thus LDs running within suspicious neighborhoods analyze fewer
benign files than LDs in the traditional deployment scenario.
At the same time, \sysname has slightly lower recall than both LDs and the neighborhood detector
because \sysname labels 
a file as malicious only if it is contained within a suspicious neighborhood and a local detector
raises a file-level alert. However, the neighborhood and domain name classifiers are imperfect --
they may fail to correctly label malicious neighborhood and domains respectively. 
Therefore, \sysname does not aggregate LDs' output across
all malicious files, which results in a slightly lower recall. 
\sysname{}'s F-1 score is bounded by close values of precision and recall and it is much higher
than the analogous parameter of local detectors and the neighborhood detector.

To quantitatively compare \sysname with local detectors we compute the area under F-1 curve. 
In the case of file
detection, \sysname achieves 96.6\% higher area under F-1 curve than the local detector.
%And \sysname achieves much higher precision than LDs~\ref{fig:temporal-file-stat-LD} and Neighborhoods~\ref{fig:temporal-file-stat-NBD} because
%it has much lower false positive rate as many benign files are already filtered out by
%the neighborhood filter. And thus LDs running within suspicious neighborhoods analyze fewer
%benign files than LDs in the traditional deployment.
%At the same time, \sysname has lower recall than both LDs and NBDs because \sysname labels 
%a file as malicious only if it is contained within a suspicious neighborhood and an LD
%raises a file-level alert. However, the F-1 score is much higher than the F-1 score pure
%LDs and the NBD concentrator.


\textbf{Machine-level real-time detection.}

\begin{figure*}[t]
\begin{minipage}[tbp]{0.24\linewidth}
   \includegraphics[width=\textwidth]{figs/symantec/temporal_analysis/machine_stat.eps}\par
   \label{fig:temporal-machine-stat}
\end{minipage}
\begin{minipage}[tbp]{0.24\linewidth}
   \includegraphics[width=\textwidth]{figs/symantec/temporal_analysis/machine_ld_precision_recall.eps}\par
   \label{fig:temporal-machine-stat-LD}
\end{minipage}
\begin{minipage}[tbp]{0.24\linewidth}
   \includegraphics[width=\textwidth]{figs/symantec/temporal_analysis/machine_nbd_precision_recall.eps}\par
   \label{fig:temporal-machine-stat-NBD}
\end{minipage}
\begin{minipage}[tbp]{0.24\linewidth}
   \includegraphics[width=\textwidth]{figs/symantec/temporal_analysis/machine_shape_gd_precision_recall.eps}\par
   \label{fig:temporal-machine-stat-Shape}
\end{minipage}
\caption{Machine-level dynamic behavior. Left to Right: Raw statistics, LD-level stat, NBD-level stat, Shape-LD - level stat}
\label{fig:temporal-machine-stat-minipage}
\end{figure*}

Though \sysname is designed to work at the file level, we also present machine level detection results.
We use a natural definition of a compromised machine as a machine that has downloaded 
at least one malicious file.
We repeat the previous experiments at the machine level.
In particular, we are interested in how well \sysname detects infected machines.
Here we mostly focus on the differences between machine-level and file-level detection results.

\textbf{Machine statistics.}
Machine-level statistics (Figure~\ref{fig:temporal-machine-stat}) is similar to the file-level statistics --
only a small percentage of machines is compromised within each NTW window.
The number of machines and compromised machines reach their peak values of 1.43 million and 126.9 thousand
respectively in October 2010, i.e. less than 8.9\% of compromised machines at the peak.

Overall, we observe higher values of precision and recall for all detectors (Figure~\ref{fig:temporal-machine-stat-minipage}) 
because they do not have to be very precise, 
i.e. they need to detect at least one malicious file on a machine, and 
file-level false positives on a particular machine do not count if that machine is infected.

As at a file-level, local detectors still suffer from low precision because of the high
number of false positives. However, precision is significantly higher 
-- its mean value is 41\% as opposed to the mean value of 19\% for the file-level detection. 
Such an effect occurs because file-level false positives on compromised machines do not affect machine-level precision.
And the recall exhibits a behavior similar to the previous case.

We observe a similar trend for the neighborhood detector -- the mean precision value is 48\% versus
12.5\% in the case of file-level detection. The recall value remains
in the range of 36\% -- 92\%.

Finally, \sysname brings the precision curve up at the cost of slightly lowering the recall -- this is
exactly the same effect that we observe in the case of file-level malware detection.

%reduces the FP rate even further and as a result the precision curve gets shifted 
%upward, but it looses some true positives. Interestingly, \sysname brings two curves --
%precision and recall -- together and achieves higher F-1 score than other detectors.
%\mikhail{add area under F-1 curve.}

Overall, \sysname achieves better results at the machine-level malware detection, which means that it can
identify infected machines earlier and more robustly than individual malware samples.
In the case of real-time detection, the main \sysname{}'s competitors are local detectors.
However, \sysname outperforms them by 28.6\% higher area under F-1 curve score.



\subsection{Aggregate detection.}

\begin{figure}[tbp]
   \vspace{-0.0in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/symantec/aggregated_analysis/aggregated_analysis_files.pdf}\par
   \caption{File-level aggregated analysis.}
   \vspace{-0.2in}
\label{fig:file_agg_analysis}
\end{figure}


\begin{figure}[tbp]
   \vspace{-0.0in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/symantec/aggregated_analysis/aggregated_analysis_machines.pdf}\par
   \caption{Machine-level aggregated analysis.}
   \vspace{-0.2in}
\label{fig:machine_agg_analysis}
\end{figure}

In this section we focus our attention only on the aggergate detection results that do not
include temporal aspect of real-time detection. Such analysis allows us to compare \sysname with
the state-of-the-art malware detector for the Wine dataset~\cite{downloader_graphs}.
We compute aggregate statistics by merging malware detection results across independent executions
of a corresponding detector. In comparison to the real-time detection, which may produce biased results if
a detector keeps detecting the same malware samples over multiple runs, aggregate results
demonstrate what percentage of malware is actually detected across all runs.
When presenting aggregate results, we count each file exactly once, i.e. whether it is
detected or not, irrespective of that it may be present within multiple neighborhood 
time windows.

As before, we compare all detectors using standard machine learning metrics -- precision,
recall, and F-1 score -- and security specific metrics -- time to detection, i.e. how quickly
a detector detects malware after it penetrates the infrastructure, early detection, i.e.
what percentage of files can be detected ahead of commercial antivirus tools employed
by VirusTotal and how early a detector captures mawlare. 
We present file-level results and machine-level results side-by-side for the purpose of comprehensive
comparison of the detectors.

\mikhail{move to intro or to the related work}
In addition to the detectors that we consider in the real-time detection section~\ref{},
we also compare \sysname{}'s results with the best known prior work -- 
the downloader detector~\cite{downloader_graphs}.
The detector introduced by Kwon et al. analyzes only downloaders -- the files that download
other files. For each downloader it extracts local features that characterize a subgraph
induced by a downloader and global features that characterize global behavior of a downloader
in the Wine dataset (e.g. how many other files a downloader downloads across the Wine dataset).
After extracting both local and global features from a subgraph, Kwon et al. use a Random Forest
classifier to predict whether a particular downloader is malicious or not.

Such an approach has several fundamental issues. First, it is applicable only to downloaders. If a malware
sample does not download other files, the detector is not able to classify it.
Second, the features used by Kwon et al. are not evasion resilient, which makes easy for
hackers to disguise malicious behavior. For example, they may design malware that
downloads not only malicious files, but also benign files. Alternatively they can obfuscate
malware such that the most important features in the Kwon's detector -- global features --
will not work because they consider files identical only if they have same hashes.
Finally, for a detector to make a decision regarding a file, it has to wait until the file
downloads other files which takes an order of several days. 
However, in the meantime a malicious file may cause irreparable damage
to the underlying system.

%In comparison to the temporal analysis, which merely provides an intuition towards how good
%results are for each run of \sysname, here we analyze results aggregated over all runs of
%our detectors. While the temporal analysis considers the same file belonging to different
%NTW as independent files when computing precision and recall parameters, the aggregated
%analysis counts each file just once. As in the previous section, we consider file-level and
%machine-level results separately. However, the primary focus of \sysname is to detect
%malicious files.

\subsubsection{File-level analysis}
\textbf{False positive rate.} We start with comparison of the false positive (FP) rate.
The downloader detector~\cite{downloader_graphs} achieves the lowest FP rate.
It has 3.9\% FP rate on the set of downloaders, however, downloaders constitute only a small
portion of the entire dataset (439 thousand out of 20.55 million files).
Thus, its effective FP rate is 0.076\%, which is reached at the cost of excluding
more than 20 million (or more than 97.3\%) files from the analysis.

The other prior work -- local detectors~\cite{vt_report_classification} -- has a fixed false positive
rate of 5\% that we set up in our experiments to make them above 90\% true positive (TP) rate.

Surprisingly, the neighborhood detector's FP rate is only marginally worse than local detectors'
FP rate -- 5.8\% in comparison to 5\%. However, it filters out significant portion of benign files
such that \sysname achieves 10.7 times FP rate reduction by reanalyzing its output, 
i.e. the FP rate drops from 5.8\% down to 0.54\%.
If we compare \sysname to the local detectors, it has 9.3 times lower FP rate, thus 
it brings the absolute number of false positives from $\sim$1.2 million down to $\sim$109.9 thousand.
Therefore, the deeper (even human-level) analysis becomes feasible, i.e.
$\sim$109.9 thousand false alerts over a 5-year period correspond to 60 false alerts per day on average.


%
%\textbf{False Positives}
%First, we analyze false and true positive rates of the four detectors that we consider 
%in the paper. The Downloader graph detector~\cite{downloader_graphs} achieves the lowest 
%FP rate 3.9\% among all downloaders, however, the total number of downloaders in the Wine
%dataset is only 439 thousand out of 20.55 million files. Thus, the effective FP rate is 
%only 0.076\%. And this achieved at the cost of excluding from the analysis more than 20 million (or more than 97.3\%) files.

%In comparison to the downloader graph detector, the local detector has 5\% false positive
%rate and in absolute numbers this means that more than a million files are misclassified.
%In comparison to LDs, NBD detector misclassifies even larger number of files -- 
%$\sim$6\% or 1.2 million files, and we choose this operating point deliberately to avoid
%NBD classifier to miss malware samples. Finally, \sysname reduces FP rate by more than 
%8 times in comparison to LDs due to smart filtering out benign files by the NBD classifier.
%\sysname{}'s FP rate of 0.55\% or 107.6 thousand misclassified files means that only 60
%misclassified files need to be reanalyzed per day, which lies in range of 
%human-level analysis.

\textbf{True positive rate.} Next, we compare detectors' true positive (TP) rate. As we explained before,
the downloader detector~\cite{downloader_graphs} has the lowest TP rate because
its inherent inability to analyze non-downloaders.
Thus, it discovers
96\% of malicious downloaders or only 31.39\% of all malware samples. 
It misses 94 thousand malware samples out of 137 thousands.
Note the Wine dataset 
may be skewed in the favor of malicious downloaders, i.e. approximately one third of 
malware samples in the dataset are malicious downloaders.

Due to the design -- we adjust local detectors' threshold to make them achieve higher than 90\% TP rate 
-- they demonstrate the highest TP rate (90.5\%) among all four detectors.
Compared to local detectors, the neighborhood detector achieves slightly 
lower TP rate -- 84\% TP because it accidentally filters out some malicious files while
the local detectors analyze all of them. Specifically, if the neighborhood detector
fails to correlate malicious downloads appropriately, it may distribute malware samples 
across the multiple predominantly benign neighborhoods. And due to low malware concentration
they may be excluded from the further analysis by the neighborhood classifier.
The other reason why the neighborhood classifier misses some malware is because it may
filter out malicious files based on underestimating the possibility of a domain, where those files
have been downloaded from, to distribute malware.

%\textbf{True positives}
%Second, we compare detectors in terms of true positive (TP) rate. In this case, 
%the downloader etector achieves the lowest TP rate because its ability to analyze files
%is limited by downloaders only. Even though the original paper~\cite{downloader_graphs}
%claims that the detector achieves 96\% TP rate on the set of malicious downloaders, which
%includes only 43.1 thousand, it excludes from the analysis 94 thousand files.
%By design, the downloader graph detector can not detect more than 43.1 thoisand malicious
%files. Thus, its TP rate is only 31.39\% on the entire dataset.
%Note if malicious files are mostly present in a dataset as leaf nodes as opposed 
%to downloaders, then the downloader detector is not able to detect those files.

%Local detectors have the highest TP rate because they analyze every file in the
%system. The NBD detector has slighly lower TP rate of 84.42\% because neighborhood detector may not be able to find enough correlations between those malicious files, thus they go 
%into the neighborhoods that have low malware concentration and therefore are discarded by
%the neighborhood classifier. Also the domain name classifier excludes some malicious
%files  from including them into a neighborhood.

Comparing to the neighborhood detector, \sysname{}'s has a slightly lower TP rate
because it relies on imperfect local detectors when aggregating alerts across 
suspicious neighborhoods produced by the neighborhood detector. 
If malware within suspicious neighborhoods was sampled uniformly at random, 
then \sysname{}'s TP rate would be roughly $90.47\%*0.8403=76.02\%$. 
However, in our experiments we found
that \sysname{}'s TP rate is 78.03\%, which is higher than expected 2\%. 
This is likely to happen because the neighborhood detector aggregates correlated malware samples, 
and consequently local detectors have a higher TP rate on such malicious files.

All four detectors explore different operating points in the FP/TP design space.
To actually compare them, we use a standard machine learning metric -- F-1 score 
(harmonic mean of the precision and recall). The F-1 score is bounded by 100\% value, which
is achieved only if a detector has 100\% TP rate and 0\% FP rate.
And \sysname achieves the highest F-1 score because it detects a large portion of
malware samples in the dataset (78\%) and it maintains a low FP rate (0.54\%).
The next closest competitor -- the downloader detector~\cite{downloader_graphs} --
achieves only 44\% F-1 score, which is 1.37 times lower than \sysname{}'s F-1 score (60.46\%)
because of the much lower TP rate.

%\textbf{F-1 score} On the Wine dataset \sysname{}'s closes competitor is the downloader
%detector, which achieves almost 44\% F-1 score, however, \sysname{}'s F-1 score is
%1.37 times higher (60.38\%). LDs and the NBD detector suffer from low F-1 score mainly
%because of low precision, i.e. high false positive rate.

\textbf{Time to detection.} To complete comparison of \sysname with the downloader detector,
we analyze the `time to detection' parameter (how quickly a detector can identify malware after it penetrates a system)
and the `early detection' parameter (how much earlier a detector detects malware ahead of commercial antivirus products).
Obviously local detectors have the best possible time to detection  -- 0 days -- because they analyze every file
once it is being downloaded for the first time. 
And \sysname detects malware approximately $\sim$20 days after it starts infecting machines. 
\sysname can improve this parameter if it runs more frequently rather than every 30 days.
Kwon et al.~\cite{downloader_graphs} do not report such a parameter for their downloader detector.

\textbf{Early detection.}
To estimate the other parameter, early detection, we use only malware samples (68,398 out of 137,279) that appear in 
the Wine dataset earlier than they are submitted the first time to VirusTotal.
As in the case of time to detection, local detectors achieve the best results -- they detect 92\% of malware 
214 days earlier on average than commercial antivirus tools employed by VirusTotal. \sysname detects 43\% of malware
samples 345 days earlier, and downloader detector can detect only 4.4\% of malware samples 9.24 days earlier.
The downloader detector demonstrates such low results because it analyzes disregard non-downloaders and,
when analyzing downloaders, it has to wait until a downloader downloads other files, 
but this takes several days.
As mentioned above, \sysname has a room for improvement by running it more frequently.

%Obviously, LDs lead in terms early detection because they analyze all the files in the system, thus they can detect malware as soon as it enters the system. And they detect 92\%
%of malware samples 214 days earlier commercial antiviruses employed by VirusTotal.
%\sysname detects early only 44\% of malware samples, and average early detection is 340 days
%ahead of commercial antivirus products. Malware remains undetected on average for less than 20 days when \sysname is deployed. It is possible to improve this parameter for \sysname
%by running the detector every few hours rather than every 30 days as we did in our experiments.



\subsubsection{Machine-level detection} 
For completeness we describe machine-level detection results as well, however, 
we mainly focus our attention on the new trends unobserved in the file-level detection.
As before, we consider a machine to be compromised (or infected) if it has downloaded at least one malicious file.
%One of the use-cases for a machine 

Even though we designed \sysname to be a real-time file-level detector, it also achieves
the best machine-level detection results~\ref{fig:machine_agg_analysis} --
the highest F-1 score.

\textbf{False positive rate.}
As for the FP rate we notice two opposite trends. First, the machine-level FP rate is getting higher
in comparison to the file-level FP rate for all detectors because if they mislabel a single benign
file, it may be downloaded on multiple clean machines, thus, those machines become false positives as well.
Second, the pairwise FP ratio between those detectors significantly change.
For example, the downloader detector has only 1.53 times lower FP rate than \sysname when they detect infected machines.
However, the same file-level ratio is 7.1 times.
The downloader detector's results worsen mainly because the detector often mislabels benign files 
that are frequently downloaded on multiple clean machines, so those machines are considered as false positives.
Surprisingly, the neighborhood detector's FP rate reaches almost 80\% and makes it completely
unusable -- due to this reason we exclude it from the further discussion.

\textbf{True positive rate.}
In comparison to the FP rate, the TP rate does not exhibit a single trend -- the direction,
in which it moves, depends on a particular detector.
The downloader detector's TP rate drops down by almost 3 times because the majority of machines
in the Wine dataset is infected by non-downloaders (malware that does not download other files).
As a result, the downloader detector misses almost 87\% of infected machines.

\sysname{}'s TP rate demonstrates the opposite trend -- it increases in comparison to the file-level
detection by 6.7\% because \sysname searches for correlated malicious downloads and thus it is likely to 
detect similar malware that infects multiple machines. As a result, spatial correlations between 
malware downloads boost detection results -- they raise from 78.03\% to 84.71\%.

Overall, \sysname achieves the best FP/TP trade-off -- the highest F-1 score (60.06\%). 
And the downloader detector demonstrates the poorest detection results -- the lowest F-1 score (17.08\%) --
mainly due to low its low TP rate.

\textbf{Time to detection.}
We observe that average time to detection slightly increases for \sysname (from 20.33 days up to 28.67 days),
but it is almost 3 times lower than the same parameter of the downloader detector because
\sysname makes a decision regarding a file without waiting until it downloads other files.



%repeat the same trends that we thoroughly
%described in the previous subsections, but the \sysname{}'s advantage is not that high.
%\sysname achieves twice lower FP rate in comparison to LDs and almost the same TP rate (2.5\% lower TP). 
%Overall, \sysname{}'s F-1 score is higher than LDs' F-1score by 12\%.
%Also, \sysname detects infected machines on average 28.5 days after malware penetrates them.
%As we discussed before, this parameter could be improved by running \sysname more frequently.

%
%Interestingly, the machine-level detection results repeat the same trends that we thoroughly
%described in the previous subsections, but the \sysname{}'s advantage is not that high.
%\sysname achieves twice lower FP rate in comparison to LDs and almost the same TP rate (2.5\% lower TP). 
%Overall, \sysname{}'s F-1 score is higher than LDs' F-1score by 12\%.
%Also, \sysname detects infected machines on average 28.5 days after malware penetrates them.
%As we discussed before, this parameter could be improved by running \sysname more frequently.
%
%Surprisingly, suspicious neighborhoods cover 80\% benign and 96\% malicious machines. This
%happens because the neighborhoods are operate at the file level rather than at the machine level. 
%To increase neighborhood effect and achieve higher FP rate reduction, the neighborhood
%algorithm should be designed to partition machines based on the correlated behavior 
%rather than files. When partitioning files, it does not consider the fact how many
%machines possess a particular file. Thus, neighborhoods are often not very discriminative in terms of machines, 
%i.e. they fail to filter out mostly benign machines. To achieve better
%results, we may need to use information about dynamic machine-level behavior, which is not
%available to us as a part of Wine dataset.

\textbf{GD ROC.}

%\begin{figure}[tbp]
%   \vspace{-0.0in}
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/symantec/shape_roc/shape_roc.eps}\par
%   \caption{ROC of Shape+LD detector computed by varying LD's threshold.}
%   \vspace{-0.2in}
%\label{fig:shape_roc}
%\end{figure}



\textbf{Ideal ML algorithms.}

\textbf{Evasive malware.}

\textbf{Deep dive.}


==> robust_prediction.tex <==
%\subsection{How many FVs does Shape GD need to make robust predictions?} 
%\label{sec:nbd-size}

%As we have just seen, Shape GD works well with neighborhoods of 15,000 FVs.
%Here we analyze in detail how Shape GD's detection ability depends on the size
%of neighborhoods used for training.

%As we discuss in the Section \ref{sec:algorithm}, Shape GD learns distribution
%of false positives (FPs).  And one of the most crucial parameters that governs
%the learning process is the number of feature vectors (FVs) per group, i.e.
%the size of an individual subset (Section \ref{sec:power-shape}).  It is worth
%noting that only a small fraction of a benign group, which is equal to LD's FP
%rate, is used for training a GD, the rest FVs are filtered out by an LD.

The number of FVs per neighborhood required by \sysname to make a robust
prediction is a crucial parameter.  With too few FVs produced by a
neighborhood, benign neighborhoods' ShapeScore will have high variance (i.e.
benign distribution in Figure~\ref{fig:windows-hist} becomes wide and the gap
between two distributions shrinks), leading to global false positives and
negatives.
%With too few FVs, 
%benign neighborhoods shape will have high variance (i.e.  benign
%distribution in Figure~\ref{fig:windows-hist} becomes wide and the gap
%between two distributions shrinks), leading to false negatives and
%positives. 
On the other hand, if neighborhoods are large, their ShapeScores
will be dominated by the large number of benign FVs and thus lead to
missed alerts (false negatives) especially in the early stages of
infection. 
Further, the number of alert-FVs generated by a neighborhood in a
deployed \sysname need to be comparable to or larger than those used
in training -- hence, we want to determine the smallest
number of FVs \sysname needs to make a robust prediction.

%Further, the number of alert-FVs per neighborhood in a
%deployed Shape GD need to be comparable to (or larger than) those used
%in training -- with these constraints, we want to find the smallest
%number of FVs Shape GD needs to make robust predictions.

%\todo{move to algo section} 
%Note that neighborhoods used by Shape GD in a deployment mode cannot be
%smaller than those used for training; otherwise, Shape GD will not be able to
%maintain its false positive rate. 

%Obviously, the size of the neighborhoods
%used for training affects the absolute value of the threshold and the gap
%between the two histograms (Figure \ref{fig:windows-hist}).
%Both extreme cases -- neighborhoods are either too small or too big --
%adversarially affect Shape GD's performance, i.e. they  decrease its
%sensitivity to mawlare spread.  On the one hand, if a neighborhood size is
%small, then 
% therefore Shape GD can recognize
%malware presence only in heavily infected neighborhoods, consequently it may
%easily overlook early stages of malware propagation.  On the other hand, large
%size of training neighborhoods requires all incoming neighborhoods to be even
%larger in order to maintain a fixed false positive rate, which may not be
%feasible due to, for example, a small number of nodes reporting suspicious
%activity.  Let's assume that in a deployment mode Shape GD receives a smaller
%neighborhood than the size of neighborhoods used for training, then the GD can
%still output the label `benign' if the data look benign.  However, it can not
%label incoming data as `malicious' because this would not allow Shape GD to
%maintain the global false positive rate at the level set during the training.

%Due to the large width of the FP distribution, a GD may ignore early stages of malware propagation in a network, which, in this case, slightly perturbs mostly false positive data flowing to a GD.
%On the other hand, high value will require an incoming rate of suspicious FVs to be higher than the value used for training a GD.
%For example, if a GD receives fewer suspicious FVs than the number of FPs used in the training procedure, it still can output the label `benign' if the data look benign. However, it can not label incoming data as malicious because this would not allow to maintain the global false positive rate at the level set during the training.

%When empirically analyzing dependence between the size of neighborhoods used
%for training and the characteristics of the histograms (Figure
%\ref{windows-hist-stability}), we are interested only in the parameters
%affecting Shape GD performance the most: the distance between the histograms
%and the size of the benign histogram.

Figure~\ref{fig:windows-hist-stability} shows the sensitivity of \sysname to
neighborhood size (i.e., the number of FVs generated by nodes in a neighborhood
during training stage).  We 
vary the number of FVs that a neighborhood generates from 3,000 up to
30,000 FVs and average the results of 10 experiments.
%We vary the size of neighborhoods used in training from 3,000 up to 30,000 FVs
%and average the result of 10 experiments.  
We present two metrics in Figure~\ref{fig:windows-hist-stability} -- the red
curve plots the inter-class distance (between histograms of benign and
malicious neighborhoods from Figure~\ref{fig:windows-hist}), and the blue curve
plots intra-class distance (i.e. the width of the benign histogram).
% Figure~\ref{windows-hist-stability} for each neighborhood size we compute
% shows the distance between the benign and malicious histograms (blue curve)
% and the width of the benign histogram (red curve).  The former parameter
% shows how While the blue curve measures how distinguishable the two shapes
% are, the red curve measures how quickly the variance in benign neighborhoods'
% shape decreases when increasing the size of neighborhoods.
%
%We experimentally analyze how the number of FVs per group affects a
%distribution of FPs and TPs \ref{windows-hist-stability}.  For this purpose,
%we vary the parameter from 3,000 up to 30,000 FVs and repeat the experiment 10
%times to avoid high variance of the results (horizontal axis).  Specifically,
%we focus our attention on two characteristics of the bi-modal distribution
%(Figure \ref{fig:windows-hist}): the distance between the FP and TP histograms
%and the width of the FP histogram (vertical axis).  The former parameter (blue
%curve) shows how distinguishable two distributions are, and this directly
%affects the number of GD's false positives, i.e. the larger the distance, the
%lower the number of GD's false positives.  The latter parameter (red curve)
%demonstrates how quickly the width of the FP distribution grows when
%increasing the number of FVs per group.
%
Figure~\ref{fig:windows-hist-stability} shows that the red inter-class distance
increases (and blue intra-class variance decreases) quickly as neighborhood
size increases, and both curves
%then it starts decreasing such that the curves
flatten out once the neighborhoods start generating more than 15,000
FVs.

%should generate  greater than or equal to 15,000 FVs 

This shows that (for our Windows programs dataset) neighborhoods generating
15,000 FVs or more are a good choice to train Shape GD because purely malicious
or benign distributions stabilize at this size.  In real scenarios with
mixtures of mostly benign and a few malicious neighborhoods, the number of FVs
will have to be scaled up depending upon the timescale of attacks (hours for
phishing v. seconds for waterhole) and the number of nodes affected by an
attack (tens of nodes  in enterprise email networks v.  thousands in a broader
waterhole attack on the enterprise). In the phishing and waterhole attack case
studies in the paper, we use neighborhoods of 1,086 and $\sim$17,000 nodes that
produce 15k FVs and 100k FVs respectively.

% \ignore{and discuss this choice in greater detail?}.

%When selecting a size
%of training neighborhoods, we should also take into consideration the time
%scale of an attack that we are trying to detect. For example, in the phishing
%experiment we use neighborhoods of 100,000 FVs for training Shape GD because a
%phishing attack has a large scale -- an order of several hours.  On the
%contrary, due to high variance of network requests in the waterhole scenario,
%we bring this parameter down to 15,000 FVs.
%<Histogram End>

%<Time-based NF Begin> <Overview of the rest of the section>

%Every experiment is performed 10 times with random initial parameters
% and the presented results are averaged across ten repetitions.

\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/windows/histogram/histogram_stability.eps}\par
   \caption{Analysis of ShapeScore histogram parameters when changing
     neighborhood size.  The curves flatten out on the right side from
     the operating point.}
   \vspace{-0.2in}
\label{fig:windows-hist-stability}
\end{figure}


==> theory.tex <==
% Sanjay's text goes here
%\section{Formal model}
\input{theory/model}



==> theory/model.tex <==
%% algorithm description

%In this section, we describe our algorithmic approach and the
%associated intuition.

%% \subsection{Notation}

%\noindent \textbf{Notation:} Let $G(V, E)$ be the network graph
%consisting of the vertex set $V$ and edge set $E,$ with $|V| = n,$
%where $n$ is the number of nodes in the network. Each node in this
%graph has a \underline{neighborhood}, consisting of all nodes that
%are one-hop away on the graph\footnote{In general, we could consider
%node $i$'s $k-$hop neighborhood $N_k(i)$, consisting of all nodes at
%most a distance $k-$hops from node $i.$}. Thus for node $i \in [n]$
%($[n] = \{1, 2, \ldots, n\}$), its neighborhood $N(i) = \{j | d(i, j)
%\leq 1\}$ where $d(\cdot, \cdot)$ is the standard hop-count metric.\\
%\noindent \textbf{Network Spread:} The key property of these graphs
%that we leverage is the presence of communities (i.e., subsets of the
%nodes) whose aggregate malware activity is correlated. Recall that
%this is precisely the case in the Anthem waterhole attack
%\cite{anthem}, the Cydia/Android App-Store attacks \cite{keyraider}
%and phishing attacks \cite{phishing-1,phishing-2}). Critically, there
%are algorithms developed in the social sciences and more recently in
%computer science and engineering to automatically detect these
%communities (e.g.,
%\cite{lancichinetti2009community,leskovec2010empirical,yang2013overlapping})
%and hence it is possible to leverage them to design global algorithms
%with much higher accuracy of detecting an outbreak.\\

%\subsection {System Architecture and Algorithm Ideas}
%\label{sec:ideas} As illustrated in Figure~\ref{fig:ab}, \sysname
%consists of three parts: {\em (i)} a Feature Extraction (FE)
%algorithm, {\em (ii)} a Local Detector (LD) algorithm, and {\em
%(iii)} a Global Detector (GD) algorithm. As the names suggest, the FE
%algorithm extracts feature-vectors from the underlying OS system call
%trace; the LD algorithm generates {\em alerts} -- noisy indicators to
%signal the potential presence of malware -- based on the
%feature-vectors at a device-level; and the GD algorithm dynamically
%combines the LD alerts and feature-vectors across devices in the
%community (using network topology) to infer the presence of malware
%in the community. \noindent \textbf{Algorithm Ideas:} Our key
%innovations are at the Global Detector level. As discussed in
%Section~\ref{sec:intro}, there are two insights that our algorithms
%depend on: {\em censoring using neighborhoods} and {\em difference in
%the shape of the distributions of true and false positives}. These
%properties, unlike counting alerts, are robust to the dynamic
%variations in community size.
%%% \mohit{discuss a baseline of count, and why it is not robust?}
% First is the idea of {\em censoring using graph neighborhoods}. To
%understand this, it is useful to recall our two key examples from
%above -- the Waterhole attack and the Phishing attack. In the Anthem
%Waterhole attack, recall that the community, or neighborhood, is
%defined by those employees that had visited the compromised website.
%In the Phishing attack, the community was defined by the company --
%all employees, for example. The Neighborhood Filter (NF) algorithm
%serves to automatically detect which of these communities are the
%ones of central interest. The NF algorithm works within the Global
%Detector. Once an alert is detected at a particular node, the NF
%algorithm counts all alerts over a nearby space-time window -- that
%is, over other nodes in the same community (or communities) as that
%node, with controlled temporal proximity. If this count exceeds a
%threshold, then the alert and associated feature-vector is retained
%for further processing, otherwise the alert is censored. This local
%filtering serves, effectively, to boost the signal, since it allows
%us to focus only on candidate nodes, and therefore a much smaller
%portion of the signal. This has the potential to significantly reduce
%the number of false positives and negatives of our algorithm. In
%recent work, algorithms have been proposed that have a graph notion
%associated to a node-to-node spreading of an attack, and this graph
%then serves to define communities. This bears similarity to our local
%filtering approach for identifying the subcollection of nodes on
%which we wish to focus. Most prior work, however, then focuses on
%decisions based on counts. For example, work in \cite{meirom14}
%counts the number of locally dense alert regions. If this count
%exceeds a predetermined threshold, malware is reported. The authors
%have theoretical results showing asymptotically vanishing (in network
%size) error rates. As with other count-based mechanisms, if the
%community size estimates are noisy, determining a reliable threshold
%becomes hard in this setting as well. Instead, in our work, we use
%local densities to simply censor alerts, and then rely on the shape
%of the distribution (see below) for decision making -- a metric we
%show is highly robust to count errors.
%%An important point to note is that we are not relying on
%%predetermined and static detectors in the network; instead we are
%%dynamically getting observations from currently participating
%%community members, and censoring based on current network
%%neighborhood state.
% This robustness to count fluctuations comes from the second key idea
%that makes up our global detector. This is what we refer to as {\em
%shape}, and in place of a simple counting criterion, it critically
%uses the {\em shape of the distribution.} Specifically, our main
%observation is that in aggregate, looking at the {\em inputs to the
%local detectors that send an alert} is informative. That is, instead
%of simply counting alerts, {\em we need to exploit the actual
%feature-vectors generating the alerts} (these are eigenvalues if the
%feature extraction from the OS trace is based on PCA
%\cite{jolliffe2002principal,hearst1998support,scholkopf1998support}).
%This idea has an information theoretic justification as well. The
%entropy at the input (feature vector space) to the (noisy) local
%detector is greater than that at its output (binary space). This
%principle is known as the {\em data processing inequality} in
%information theory \cite{cover2012elements}. As we describe in detail
%below, we exploit this idea in the following way. The signals flagged
%by the local detectors consist of true positives and false positives.
%By definition, the local detectors cannot distinguish between these
%(otherwise the local detector would have flagged fewer false
%positives). This does not mean that {\em on aggregate} false
%positives and true positives {\em look different}. This difference
%can be revealed by computing a distributional distance. That is, we
%employ a measure of distance between distributions called the
%Wasserstein distance, to see how far an aggregation (histogram) of
%the inputs that led to flags at the local detectors, is from a
%reference distribution. We find that this procedure has great
%discriminatory power. To demonstrate the informative power of this
%procedure, we plot (i) the score distribution of the {\em true
%positives} (real malware activity) of the local detector (Wikipedia
%app with malware, random forest based LD), and (ii) the score
%distribution of feature vectors that correspond to the {\em false
%positives} of the local detector (misclassifications by the local
%detector). More specifically, in Figure~\ref{fig:intro-histogram},
%for each of the cases above, we first construct a (multi-dimensional,
%here 10-dimensional) (normalized) histogram of the feature-vectors.
%We then determine the Wasserstein distance
%\cite{vallender1974calculation} (see Section
%\ref{sec:algo_description} for the description of this scoring)
%between this histogram and a multidimensional-uniform baseline.
%%\footnote{Suppose that the feature-vectors are $l$-dimensional Then,
%%we construct a $L$-dimensional baseline histogram that has, in each
%%dimension, a uniform pmf over the support of the feature-vector in
%%the corresponding dimension.}
%This distance is a {\em community score}. Qualitatively, the
%community score encodes the deviation of the collection of
%neighborhood filtered feature-vectors from a uniform baseline. The
%crucial observation is that this score function is statistically
%different for LD false positives and true positives. {\em In other
%words, a GD can distinguish a set of false positives from true
%positives without using count and only using the shape of the feature
%vectors.} \subsection{Algorithm Description}

%\label{sec:algo_description}

Our algorithm consists of feature extraction, local detector (LD), and the
global detector (GD). Our key innovations are in the GD, however, 
we also discuss feature extraction and LD design for completeness.
\ignore{Our key innovations are in the GD and we discuss feature
extraction and LDs further in}

\begin{figure}
\removelatexerror
\begin{algorithm}[H]
 \small
 \DontPrintSemicolon
  \SetKwInOut{Input}{Input}
 \SetKwInOut{Output}{Output}
 \Input{Sequence of executed system calls}
 \Output{Alert-FVs}
 Let $id$ be LD's identifier\;
 \BlankLine
 
 \While{True}{
   
%   // histogram of system calls\;
   $syscall$-$hist$ $\leftarrow$ $r$-sec histogram of system calls\;
   %\BlankLine
     
   %// reduce dimensionality\;
   $syscall$-$hist_{PCA}$ $\leftarrow$ project $syscall$-$hist$ on $L$-dim PCA basis\;
   %\BlankLine
     
   %// perform binning with \textit{b} bins along each dimension\;
   $label$ $\leftarrow$ BinaryClassifier($syscall$-$hist_{PCA}$);
  \BlankLine

   \If{$label = malicious$}{
     $alert$-$FV$ $\leftarrow$ $syscall$-$hist_{PCA}$\;
     send $<alert$-$FV$, $id>$ to \sysname\;
   }
 }
 \caption{Local Detector}
 \label{LD_algorithm}
\end{algorithm}
 \vspace{-0.2in}
%\label{LD_algorithm}
\end{figure}


\noindent {\bf Feature Extraction algorithm.} 
\mikhail{
We employ two different feature extraction algorithms.
In the Wine experiment, we build a feature extractor based on the previous work~\cite{vt_report_classification}.
The algorithm converts the following fields of VirusTotal reports into a feature vector: the output of commercial tools such as
TRID, ClamAV, Symantec, statically imported libraries and functions, information about whether a file is packed,
information about whether it is digitally signed and other binary metadata.
We modified the the original feature extraction algorithm~\cite{vt_report_classification} to make it capable of processing
2.6 million VirusTotal reports. And also we apply feature hashing to reduce dimensionality of resulting feature vectors down
to 1024. We found that the output dimensionality of 1024 allows us to 
achieve the best trade-off between classifier's performance and memory consumption.

In the waterhole and phishing experiments, we apply the following standard feature
extraction approach.
}
The algorithm transforms
continuously evolving 390-dimensional time-series of Windows system calls into
a discrete-time sequence of feature-vectors (FVs). 
%% \todo{Change to windows. Check if $L=10, r = 1.$} 
This is accomplished by chunking the continuous time series into $r-$second
intervals, and representing the system call trace over each interval as a
single $L-$dimensional vector (Algorithm \ref{LD_algorithm}, lines 3--4). $L$
is typically a low dimension, reduced down from 390 using PCA analysis, to (in
our experiments) $L=10$ and $r = 1$ second.
%\mikhail{\st{, Markov models, or $n-$grams}} The output of the FE algorithm at
%each node $i \in [n]$ and each (discrete) time $\{t = 1, 2, 3, \ldots\},$ is a
%sequence of FVs $\{x_{t,i}, i \in [n], t \geq 1 \}$ where each $x_{t, i}$ is a
%$L-$dimensional real-valued vector. 

% For PCA, which is what our algorithm employs, this
% $L$-dimensional vector is the vector of eigenvalues corresponding to
% an $L$-dimensional representation of the $r-$ second chunk of the
% function call trace). We call the FVs corresponding to
% true malware activity as {\em malware feature-vectors (FVs)} and those
% corresponding to true benign app activity as {\em benign
% feature-vectors (FVs)}.\\


\noindent {\bf Local Detector (LD) Algorithm.} The LD algorithm (Algorithm
\ref{LD_algorithm}) leverages the current state-of-the-art techniques in
automated malware detection to generate a sequence of {\em alerts} from the FV
sequence. Specifically, using both its internal state and the {\em current} FV,
the LD algorithm generates an alert if it thinks that this FV corresponds to
malware, and produces no alert if it thinks that the current FV is benign
(lines 5--8). Henceforth, we define an {\bf alert-FV} to be an FV that
generates an LD alert (either true or false positive). In our experiments each
LD employs \mikhail{either Boosted Decision Trees~\cite{xgboost} (Wine experiment) or}
Random Forest (waterhole and phishing experiments) as a binary classifier for malware detection because
Random Forest and Boosted Trees achieves the best performance on the training data set 
among the classifiers from a prior survey~\cite{Canali2012}  and
have been shown to be robust to adversarial inputs.%~\cite{?}.

\mikhail{In the Wine experiment, we pick an operating point of 80.05\% 
true positive rate at a false positive rate of 2.3\% from the LD's
ROC curve and in the other two experiments our LD achieves 92.4\% true positive rate 
at a false positive rate of 6\% (which is similar to detection rates in prior work~\cite{Canali2012}).  
%We have described our experiments with picking the best LD from a
%prior survey~\cite{Canali2012} in Appendix~\ref{sec:LDs} and Figure
%\ref{fig:windows-LD-roc}.}
}

% -- we pick an operating
%point of 92.4\% true positives at a false positive rate of 6\% from the LD's
%ROC curve (which is similar to detection rates in prior work~\cite{Canali2012}).  
%We have described our experiments with picking the best LD from a
%prior survey~\cite{Canali2012} in Appendix~\ref{sec:LDs} and Figure
%\ref{fig:windows-LD-roc}. 
%in the Appendix~\ref{sec:LDs}).  \mikhail{Further information on LD design can
%be found in the Appendix~\ref{sec:LDs}.} Thus, the output of the LD algorithm
%is a sequence $\{a_{t, i}\}$ where $a_{t, i} \in \{0, 1\}.$ Here, $a_{t,i} =
%1$ encodes `alert' at time $t$ and node $i,$ and $a_{t,i} = 0$ encodes
%`no-alert'. As has been discussed earlier, this binary sequence is noisy even
%with the best known local detectors, and thus results in many false positives
%and false negatives.

%\textbf{Domain name classifier.}
%\mikhail{
%For completeness we also describe a domain name classifier that identifies suspicious domain names.
%This algorithm is
%
%We also build a classifier to identify suspicious domains. For this purpose, we convert VT's domain name
%classification -- categorical information assigned by commercial tools -- into feature vectors using one-hot
%encoding. After that we train an xgboost classifier~\cite{} using 10-fold CV and 
%AUC as an objective.
%We do not use any explicit information in domain name reports that may reveal whether those domain names have
% ever served malware.
% As in the the case of LDs, we use an xgboost algorithm~\cite{xgboost} to predict probability of a particular domain name to be malicious. At the training stage we use domain names explicitly computed over the Wine dataset,
%i.e. if a domain name has ever distributed malware, then it is labeled as malicious, otherwise it is benign. 
%We notice that frequently the same domain servers both benign and malicious files. 
%
%As before, we use out-of-fold predictions to assign labels predicted by the classifier to the domain names.
%As a result, the classifier is able to achieve 85.33\% AUC, which corresponds to 19.5\% false positive rate and
%71.86\% true positive rate. Note, such a classifier is not deployable by itself due to its high false positive rate.  Classifying urls rather than domain names, might increase accuracy, however, Wine dataset lacks such data.
%}


\noindent {\bf Neighborhood Instances from Attack-Templates.} Each neighborhood
time window (NTW), Shape GD generates neighborhood instances
(Algorithm~\ref{NI_algorithm}) based on statically defined attack vectors --
each attack vector is a ``Template'' to generate neighborhoods with.
Algorithm~\ref{NI_algorithm} shows
%The most prominent feature of this algorithm is an ability to find a common
%ground for
how the concept of neighborhood unifies operationally distinct attacks like
waterhole and phishing. 

%Though these attacks look differently, a single
%algorithm is able to build neighborhoods to enforce their detection.  Note the
%algorithm can be extended to detect other network-level attacks.

The template for detecting a waterhole attack forms a neighborhood out of
client nodes that access a server or a group of servers within a neighborhood
time window. The other template, which is used for detection of a
phishing attack, includes in a neighborhood email recipient machines belonging
to a set of mailing lists.  The two templates are shown in lines 3--10. 
\begin{figure}
\removelatexerror
\begin{algorithm}[H] 
 \small
 \DontPrintSemicolon
 \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
 \SetCommentSty{mycommfont}
 \SetKwInOut{Input}{Input}
 \SetKwInOut{Output}{Output}
 \Input{Template-type, NTW}
 \Output{Set of active neighborhoods NBDs}
 \BlankLine
 \codecomm{[\textit{time, time+NTW}] \textit{defines the current time window}}\;
 \textit{time} $\leftarrow$ \textit{current time}\;
 \BlankLine
 
\While{True}{
 \uIf{Template-type = $waterhole\ attack$}{
% 	$V$ $\leftarrow$ client machines\codecomm{*}\;
	$V$ := client machines\codecomm{*}\;
% 	$S$ $\leftarrow$ accessed servers\codecomm{*}\;
	$S$ := accessed servers\codecomm{*}\;
% 	predicate := (Client, Servers) --> {$true$, $false$} 
 	predicate(A:Client, B:Servers) := $A$ accesses $B$\;
 	\BlankLine
 }
 \uElseIf{Template-type = $phishing\ attack$}{
 	$V$ := email recipient machines\codecomm{*}\;
 	$S$ := mailing lists\codecomm{*}\;
 	predicate(A:Recipient, B:Mailing list) := $A$ $\subseteq$ $B$\;
 }
 \BlankLine

 \codecomm{partitioning a set into non-disjoint sets to incorporate}\;
 \vspace{-.03in}
 \codecomm{structural filtering}\;
 ${P_{1}, P_{2}, ..., P_{N}}$ $\leftarrow$ partition-set($S$), where $S$ = $\bigcup\limits_{i=1}^{N}    P_{i}$\;
 %\BlankLine 
 
 \codecomm{form neighborhoods $NB_i$ using partitions $P_i$}\;
 $NB_i$ $\leftarrow$ $\{V |$ predicate($V$, $P_i$)$\}$\;
 %\BlankLine 
 
 \codecomm{set expiration time for a neighborhood $NB_i$}\;
 $NB_i$.expiration-time $\leftarrow$ \textit{t+NTW}\;
 %\BlankLine
 
 \codecomm{add all neighborhoods to the set $NBDs$}\;
 $NBDs$ $\leftarrow$ $\{NB_i$ $|$ $\forall i$ in $[1,N]\}$\;
 %\BlankLine
 
 \codecomm{advance time by NTW sec}\;
 \textit{time} $\leftarrow$ \textit{time+NTW}\;
 }
 \BlankLine
 \codecomm{*active within the time window [\textit{time, time+NTW}]}\;
 %//*active within the time window [\textit{time, time + NTW}]
 \caption{Neighborhoods from Attack-Vectors}
 \label{NI_algorithm}
\end{algorithm}
 \vspace{-0.2in}
%\label{NI_algorithm}
\end{figure}


%We leave development of a template language and a general
%algorithm for instantiating arbitrary templates for future work. For now these
%hardcoded within the algorithm itself (

For simplicity we present a batch version of the neighborhood instantiation
algorithm (Algorithm \ref{NI_algorithm}) which advances time by NTW and creates
new neighborhoods for each NTW.
%, however, Shape GD uses an online version.  In comparison to the batch
%algorithm, 
In contrast, the online Shape GD version updates already existing
neighborhoods while monitoring client--server interactions in real-time -- we
demonstrate the online Shape GD algorithm to detect waterhole attacks 
%(since we
%have time-stamped traces from Yahoo data centers to conduct these experiments)
and the batch version against phishing attacks 
%(since the data-set does not have fine-grained timing information) 
in our evaluation.  

%We omit presenting the online
%neighborhood instantiation algorithm .

%because its
%technical details that may impede understanding of the algorithm itself.



The neighborhood instantiation algorithm accepts a template type as input, i.e.
either a template for detecting a waterhole attack or a phishing attack, and
duration of an NTW. 
%Whatever template is supplied, its instantiation is similar in both cases.
%%The only difference is the objects that an algorithm operates on.  The
The algorithm runs once per NTW -- starting by defining the sets $V$ and $S$ that will
be used to form neighborhoods.  For a waterhole attack, the set
$V$ includes all client machines accessing a set of servers and $S$ is a set of
the accessed servers. To instantiate neighborhoods for a phishing attack, 
%the algorithm uses slightly different definitions of the sets $V$ and $S$: 
$V$ is a set of all email recipient machines and $S$ is a set of mailing lists.
In both cases the algorithm considers only the entities that are active within
a current NTW window.

Each attack requires a predicate that determines relation between the elements
of the sets $V$ and $S$. For a waterhole attack such a predicate is true if a
client \textit{accesses} one of the servers (line 6). In the case of a phishing
template, the predicate is evaluated to true if a recipient \textit{belongs} to
a particular mailing list (line 10).

%After finishing initialization of the variables $V$ and $S$, 
The neighborhood instantiation algorithm proceeds with partitioning the set $S$
into one or more disjoint subsets $P_i$ (line 11). This is to incorporate
`structural filtering' into the algorithm, allowing an analyst to create
neighborhoods based on subsets of servers (instead of all servers in case of
waterhole) or divide all mailing lists into subsets of mailing lists (in the
phishing).  Structural filtering boosts detection under certain conditions (see
Section \ref{sec:time-struct}). 

%In our
%experiments, we split the set $S$ into equal parts, however, partitions do not
%have to be of equal size.

The neighborhood instantiation algorithm builds a neighborhood for each partition
$P_i$ using a corresponding predicate (line 12).  After forming a
neighborhood, the algorithm sets its expiration time (line 13), which is the
end of the current NTW window. All the neighborhoods in the set $NBDs$
are discarded at the end of the current NTW window.
%As mentioned earlier, we could deal with an online version of the algorithm,
%but for ease of explanation we stick to a batch version of hte algorithm to
%avoid unnecessary technical complications.
Finally, the algorithm adds the just formed neighborhoods to $NBDs$ (line
14) and advances time by one NTW (line 15). 

The template-based neighborhood instantiation algorithm (Algorithms
\ref{NI_algorithm}) 
shares the $NBDs$ data structure with the 
Algorithm \ref{ShapeGD_algorithm}
that uses neighborhoods' shapes to detect malware.
%synchronized with each other through 
%which holds information about neighborhoods.

\mikhail{We intentionally postpone discussion of neighborhoods that we use in the Wine 
experiment until we describe Wine's data format in the section~\ref{sec:wine_dataset}.}

%They are supposed to acquire a lock before updating/reading $NB$-$LIST$.
%
%The list $NB$-$LIST$ is updated here and is also accessed in the read-only mode by Shape-GD (Algorithm \ref{ShapeGD_algorithm}).



%\mikhail{
%After being able to dynamically form neighborhoods with the template instantiation algorithm, the next step is
%to develop an algorithm that can determine the presence of malware

%\textbf{Wine Neighborhoods.}
%\mikhail{
%
%In the Wine experiment we customize the previously described waterhole template. Specifically, a neighborhood is 
%a collection of files scattered across multiple machines that are transitively downloaded from a suspicious domain within a neighborhood time window.
%As in the case of the watering hole attack, the intuition behind such a neighborhood definition is
%that if a process contacts a suspicious domain, it is likely to download malicious files. 
%By traversing downloader graphs, we recursively apply such intuition to other files.
%
%Before diving into the details of the details of the algorithm, we briefly describe a domain name classifier whose goal
%is to predict probability of a domain name to serve malware based on its categorical attributes extracted from VirusTotal reports.
%Specifically, each report includes multiple categories assigned to the domain name by various commercial tools.
%For example, Websense categorizes a domain name into 1 out of 253 categories, which include advertisements, business and economy, job search and others. Based on domain attributes we train a classifier~\cite{xgboost} 
%that predicts whether a domain has ever served malware.
%As a result, the classifier is able to achieve 85.33\% AUC, which corresponds to 19.5\% false positive rate and
%71.86\% true positive rate. Note, such a classifier is not deployable by itself due to its high false positive rate. Classifying urls rather than domain names, might increase accuracy, however, Wine dataset lacks such data.
%
%After outlining the design of the domain name classifier, we can proceed to describing the difference 
%between waterhole neighborhoods and the neighborhoods we use in the Wine experiment.
%Technically the algorithm performs the following steps, which are illustrated on the figure~\ref{downloader_graph}.
%For each domain name the domain classifier outputs the probability of being malicious. If a domain is considered
%malicious (globaldl.net), we start forming a neighborhood by identifying all files that access that domain within 
%a NTW (chrome.exe on the figure) and
%for each of them we perform a breadth-first search on the downloader graph.
%While traversing downloader graphs in the BFS manner, we use domain name predictions of our domain name
%classifier to discard files downloaded from likely benign domains (gravic.com).
%Had the domain name classifier correctly identified all suspicious domains, then the neighborhood would include the following malicious files -- E, F, G, I (A is discarded because it is whitelisted). 
%However, due to high false positive rate of the classifier, neighborhoods contain only 30\% malicious files.
%%At the end of this step, a neighborhood includes files transitively
%%reachable from a suspicious domain.
%}



\noindent {\bf Malware Detection in a Neighborhood.} 
Algorithm \ref{ShapeGD_algorithm} detects malware {\em per neighborhood}
instead of individual nodes. 
%\mikhail{\st{ Our goal is to develop an algorithm that can determine the
%presence of malware {\em in a neighborhood} (and not in individual nodes).}}
%
% with global false positive rates much lower than the rates of the best local
% detectors for single nodes. Moreover, we require our algorithm to be robust
% to uncertainty in both community size and signal noise (see also
% Section~\ref{sec:eval-count}).  %
%
The input to the algorithm is a set of alert-FVs from each neighborhood and its
output is a global alert for the neighborhood.
%score -- the neighborhood's ShapeScore.  -- the distance between the input
%alert-FVs LD alerts from a neighborhood along with the corresponding
%alert-FVs.  that triggered these LD alerts.  The Shape GD executes
%periodically, and computes a score based on the FVs that it has accumulated
%over that time window.
We now describe how the algorithm distinguishes 
%achieves robustness to neighborhood size noise by distinguishing 
between the {\em conditional distributions} of alert-FVs from true-positive and
false positive neighborhoods.

The key algorithmic idea is to first extract neighborhood-level features --
i.e., to map all alert-FVs within a neighborhood to a {\em single}
vector-histogram which robustly captures the neighborhood's statistical
properties.  Then, Shape GD compares this vector-histogram to a reference
vector-histogram (built offline during training) to yield the neighborhood's
ShapeScore.  The reference vector-histogram is constructed from a set of false
positive alert-FVs -- thus, it captures the statistical shape of
misclassifications (FPs) by the LDs but at a neighborhood scale. Finally,
Shape-GD trains a classifier to detect anomalous ShapeScores as malware.  This
is a key step in Shape-GD -- i.e., mapping alert-FVs from a neighborhood into a
{\em single} vector-histogram and then into a discriminative yet robust
ShapeScore lets us analyze the joint properties of all alert-FVs generated
within a neighborhood without requiring the FVs to be clustered or alerts to be
counted.  We describe these steps in further detail.


%\ignore{
%The key algorithmic idea is to first construct a single histogram from all the
%alert-FVs from a neighborhood and compare this histogram with a reference
%histogram, {\em both from the same neighborhood}, to yield the neighborhood's
%ShapeScore that is used for generating global alerts.  The reference histogram
%is constructed from a set of {\em false positive} alert-FVs --
%%the local detectors operating with benign applications.
%thus, the reference histogram captures the statistical shape of
%misclassifications (FPs) by the LDs at a neighborhood scale.
%}

%The Shape GD scores the statistical shape of the bucket
%of alert-FVs with respect to this reference.

%\noindent {\bf Why is vector-histogram mapping crucial?} 
%
%\mikhail{ The traditional approach would analyze alert-FVs using machine
%learning algorithms (e.g. SVM, Random Forest, Logistic Regression and etc).
%However, all such algorithms are inherently stateless, i.e. they make a
%decision based on the information incorporated into the current FV and
%completely disregard all previously seen FVs belonging to the same
%neighborhood. Thus, such algorithms output new refined labels for alert-FVs,
%and the next logical step is to compare the number of alert-FVs with the
%neighborhood size when deciding whether to raise a global alert or not -- this
%is what we term Count GD. However, all variations of Count GD severely suffer
%from the problem of accurately estimating a neighborhood size
%(Section~\ref{sec:eval-count}).


%The main requirement that we impose on such a mapping is to merge
%alert-FVs in unordered way. Due to this, conventional sequence analysis
%algorithms (LSTM, HMM and etc) are inapplicable because such algorithms
%preserve sequential information. And the only way to ignore it would require to
%run an algorithm on multiple permutations of the same alert-FV sequence, which
%suffers from exponential complexity.  }

\begin{figure}
\removelatexerror
\begin{algorithm}[H]
\small
 \DontPrintSemicolon
 \SetKwInOut{Input}{Input}
 \SetKwInOut{Output}{Output}
 \Input{$L$-dim projections of alert-FVs}
 \Output{Malicious neighborhoods}
 Let $NBDs$ be a set of neighborhoods\;
 \BlankLine

 \For{each NB in NBDs}{
   %// collect alert-FVs from the nodes in the neighborhood\;
   \codecomm{aggregate L-dim projections of alert-FVs on per neighborhood basis}\;
%   $\mathcal{B}$ 
  $B$ $\leftarrow$ $\{alert-FVs$  $|$ node $id$ $\subseteq$ $NB\}$\;
   %\BlankLine

   %// reduce dimensionality\;
%   $\mathcal{B}_{PCA}$ $\leftarrow$ project $\mathcal{B}_{FVs}$ on $L$-dim PCA basis\;
   %\BlankLine

   %// perform binning with \textit{b} bins along each dimension\;
   \codecomm{build an $(L, b)$-dim. vector-histogram}\;
%   $\mathcal{H}_{\mathcal{B}}$ 
   $H_B \leftarrow$ bin \& normalize $B$ along each dimension\;

   \codecomm{compute a neighborhood score -- ShapeScore}\;
   $ShapeScore$ $\leftarrow$ Wasserstein Dist.($H_B$, $H_{{\rm ref}}$)\;
  %\BlankLine

   \codecomm{perform hypothesis testing}\;
   \If{$ShapeScore > \gamma$}{
     label $NB$ as \textit{malicious}\;
   }
 }
 \caption{Malware Detection in a Neighborhood}
 \label{ShapeGD_algorithm}
\end{algorithm}
 \vspace{-0.2in}
%\label{ShapeGD_algorithm}
\end{figure}

\noindent {\bf Generating histograms from alert-FVs.} The algorithm aggregates
$L$-dimensional projections of alert-FVs on per neighborhood basis into a set
$B$ (Algorithm \ref{ShapeGD_algorithm}, line 3).
%The algorithm processes each neighborhood separately: it aggregates alert-FVs
%on per neighborhood basis and projects them on an $L$-dimensional PCA basis to
%reduce dimensionality (Algorithm \ref{ShapeGD_algorithm}, lines 3--4).  Thus,
%the set $\mathcal{H}_{PCA}$ contains $L$-dimensional alert-FV vectors.
After that, Shape GD converts low dimensional representation of alert-FVs, the
set $B$, into a single $(L, b)$-dimensional vector-histogram denoted by $H_B$
(line 4).  The conversion is performed by binning $L$-dimensional vectors
within the $B$ set along each dimension.  In each of the L-dimensions, the
scalar-histogram of the corresponding component of the vectors is binned and
normalized.  Effectively, a vector-histogram is a matrix $L$x$b$, where $L$ is
the dimensionality of alert-FVs and $b$ is the number of bins per dimension. 

We use standard methods to determine the size and number of bins and note that
the choice of Wasserstein distance in the next step makes Shape GD robust
against variations due to binning.  In particular, we tried square-root choice,
Rice rule, and Doane's formula~\cite{binning} to estimate the number of bins,
and we found that 20--100 bins yielded separable histograms (as in Figure
\ref{fig:windows-hist}) for the Windows dataset and fixed it at 50 for our
experiments. 


%\mikhail{\st{ The $L-$dimensional vector-histogram is parameterized by $(L,
%b).$ $L$ is the dimension of the histogram and $b$ is the number of bins per
%dimension. The vector-histogram, denoted by $\mathcal{H}_{\mathcal{B}}$, is
%generated from the $L-$dimensional vectors $\mathcal{B}$ that have been
%accumulated from a neighborhood.
%%over the current time
%%period. 
%In each of the $L$-dimensions, the scalar-histogram of the corresponding
%component of the vectors is binned and normalized. We use standard methods to
%determine the size and number of bins. }}
%

\noindent {\bf ShapeScore.} 
%\todo{change language to ShapeScore throughout this paper.} 
We get the ShapeScore by comparing this histogram, $H_B$, to a {\em reference
histogram}, $H_{{\rm ref}}$,  which is generated during the training phase
using only the false positive FVs of the LDs.  We run LDs on the system-call
traces generated by benign apps -- the FVs corresponding to the alerts from the
LD (i.e., the false positives) are then used to construct the reference
histogram $H_{{\rm ref}}.$ ShapeScore is thus the distance of a neighborhood
from a benign reference histogram -- a high score indicates potential malware.

To collect known benign traces, a straightforward approach is to
use test inputs on benign apps or use record-and-replay tools to re-run
real user inputs in a malware-free system.  Or, like any anomaly detector, an
enterprise can train \sysname using applications deployed currently and recompute
$H_{ref}$ periodically. 

%-- this is
%similar to anomaly detectors where the goal is to detect anomalous behaviors as
%(potentially) malicious.

The ShapeScore of the accumulated set of FVs, $B$,
is given by the sum of the coordinate-wise Wasserstein distances
\cite{vallender1974calculation} (Algorithm \ref{ShapeGD_algorithm}, line 5) between 
%$$\mathcal{H}_{\mathcal{B}} =
%(\mathcal{H}_{\mathcal{B}}(1) \ \mathcal{H}_{\mathcal{B}}(2) \ \ldots
%\ \mathcal{H}_{\mathcal{B}}(L))$$ 
$$H_B =
(H_{B}(1) \ H_{B}(2) \ \ldots \ H_{B}(L))$$ 
and 
%$$\mathcal{H}_{{\rm ref}} =
%(\mathcal{H}_{{\rm ref}}(1) \ \mathcal{H}_{{\rm ref}}(2) \ \ldots \
%\mathcal{H}_{{\rm ref}}(L)).$$ 
$$H_{{\rm ref}} = (H_{{\rm ref}}(1) \ H_{{\rm ref}}(2) \ \ldots \
H_{{\rm ref}}(L)).$$ 
In other words,
%$$
%{\rm ShapeScore} = \sum_{l=1}^L d_W(\mathcal{H}_{\mathcal{B}}(l),\mathcal{H}_{{\rm ref}}(l)),
%$$
$$
{\rm ShapeScore} = \sum_{l=1}^L d_W(H_{B}(l),H_{{\rm ref}}(l)),
$$
where for two scalar distributions $p, q,$ the Wasserstein distance
\cite{vallender1974calculation,wasser-wiki} is given by
$$
d_W(p, q) = \sum_{i=1}^b \left |\sum_{j=1}^i \left(p(j) - q(j) \right) \right |.
$$

This Wasserstein distance serves as an efficiently computable one dimensional
projection, that gives us a discriminatively powerful metric of distance
\cite{vallender1974calculation,benbre00}. Because the Wasserstein distance
computes a metric between distributions -- for us, histograms normalized to
have total area equal to 1 -- it is invariant to the number of samples that
make up each histogram. Thus, unlike count-based algorithms, {\em it is robust
to estimation errors in community size}. Figure~\ref{fig:windows-hist} verifies
this intuition, and shows that true positives and false positive feature
vectors separate well when viewed through the ShapeScore. 

Finally, to determine whether a neighborhood has malware present we perform
hypothesis testing. If ShapeScore is greater than a threshold $\gamma$, we
declare a global alert, i.e., the algorithm predicts that there is malware in
the neighborhood (lines 6--7).  The robustness threshold $\gamma$ is computed
via standard confidence interval or cross-validation methods with multiple sets
of false-positive FVs (see Section \ref{sec:power-shape}).  

% that at this
%stage, one could use any ML algorithm to classify ShapeScores, but 
%%this would require more training data whereas
%a simple hypothesis test already provides good accuracy.




% It is important to note that not all LD alerts and their corresponding
% FVs may be available to the GD algorithm. Specifically, the GD may
% have access to only a subset of the alerts due factors outside its
% control, including user opt-in/opt-out and community churn where users
% move in and out of the community.

%The {\em Neighborhood Filter algorithm} further filters out (or
%censors) these alerts, based on the {\em neighborhood alert density}
%-- this is a key element that provides robustness to our algorithm.

%The \underline{Neighborhood Filtering (NF) algorithm} interprets an
%alert from the LD algorithm as potential malware activity. In order
%to ``amplify'' this alert, it first accumulates {\em alerts over a
%``nearby'' space-time window} consisting of nodes in one of the
%pre-defined communities of that node (as explained and illustrated
%above), and $|W|$ time steps, where $W$ is a window parameter. As
%malware activity is correlated over space and time, the window size
%is chosen to capture this correlation. Henceforth, we refer to this
%neighborhood $\times$ time window as a {\em space-time window.} As
%noted earlier, this is different from static filtering where a fixed
%collection of nodes act as malware observers. If the number of these
%alerts exceeds a threshold, then the alert is not censored, the
%corresponding {\em feature-vector}, $x_{s,i}$ is sent to the GI
%algorithm for further processing.


%Formally, each time an alert is generated at node $i$ and time $s$,
%the NF algorithm censors an alert if $|\mathcal{A}_{s,i}| <
%\beta |W| |N(i)|,$ where $\beta \in (0,1)$ is a filter parameter
%(chosen to be above the false positive probability of the LD), and
%$$\mathcal{A}_{s,i} = \{a_{u,j} | j \in i \cup N(i), u \in \{s - W
%+1, \ldots, s-1, s\}, a_{u,j} = 1\}.$$ If an alert is not censored,
%the corresponding {\em feature-vector}, $x_{s,i}$ is sent to the GI
%algorithm for further processing.

% * accumulate x_{s,i} from NF algorithm
% * \mathcal{H} construct L-dimensional histogram (normalized)


% \noindent {\em The Hypothesis Test:} We have now set up the machinery
% we need for our test: we compute the ShapeScore with false
% positive feature-vectors (FPScore), and determine a robustness
% threshold $\gamma$, which can be done via standard confidence interval
% or cross-validation methods. The test then is:
% $$|{\rm Score} - {\rm FPScore}| > \gamma, \ \rm {declare \ malware}$$



==> wine_section.tex <==
%\begin{figure*}[t]
%\begin{minipage}[tbp]{0.33\linewidth}
%   \includegraphics[width=\textwidth]{figs/windows/intro_plot/intro_plot_original_pdfs.pdf}\par
%   \label{fig:ab-1}
%\end{minipage}
%\begin{minipage}[tbp]{0.33\linewidth}
%   \includegraphics[width=\textwidth]{figs/windows/intro_plot/intro_plot_cond_pdfs.pdf}\par
%   \label{fig:ab-2}
%\end{minipage}
%\begin{minipage}[tbp]{0.33\linewidth}
%   \includegraphics[width=\textwidth]{figs/windows/intro_plot/intro_plot_VT_cond_pdfs.pdf}\par
%   \label{fig:ab-3}
%\end{minipage}
%\caption{---
%}
%\label{fig:ab}
%\end{figure*}

We evaluate our approach on the real data collected by Symantec over the period of 5 years (from 2008 till 2013).
which is available on the WINE analytics platform~\cite{wine_dataset,downloader_graphs,pup_ndss}.
The dataset includes summarized information about file download activities on the Symantec's clients' machines.
It contains 20.7 million unique files, which have been downloaded 67 million times from 500 thousand domains.

According to the graph abstraction introduced by Kwon et al.~\cite{downloader_graphs}, which succinctly describes
the data, the dataset is a collection of downloader graphs (DGs) -- one per end host. 
Each DG is a directed graph whose nodes represent downloaded files and an edge from a node $N_1$ to the node 
$N_2$ indicates that $N_1$ has downloaded $N_2$ on a particular end host. The figure~\ref{fig:downloader_graph}
demonstrates an example of a downloader graph, which includes 9 nodes annotated with their file names and edges
labeled with domain names where the corresponding files have been downloaded from.

\begin{figure}[tbp]
   \vspace{-0.0in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/windows/wine/downloader_graph.pdf}\par
   \caption{---}
   \vspace{-0.2in}
\label{fig:downloader_graph}
\end{figure}


\textbf{Ground truth.}
One of the limitations of the dataset is the lack of ground truth. To solve this problem, we rely on 
VirusTotal (VT), an online service that maintains a database of previously submitted benign and malicious files
along with their analysis results and allows to query the results with a file hash. Upon submission of a new
file, it runs 62 commercial antivirus tools and multiple other heuristic tools and stores file reports in a database. 

We queried 20.7 million file hashes present in our dataset and were able to successfully retrieve 2.6 million
file reports. We conservatively assume that the rest files are benign.
When labeling a particular file as malicious, we follow the methodology established in~\cite{downloader_graphs}
and assign a malicious label if more than 30\% of antivirus products label it as malware. Such labeling schema
does not consider files as malicious if they do not exhibit strong signs of malicious activity and also it
minimizes discrepancy between different AV vendors. Our file labels perfectly matche partial classification presented in~\cite{downloader_graphs} and the partial classification provided by Symantec.
After labeling we found that the dataset contains 20.566 million benign and 137 thousand malicious files. 

Besides querying VT for file reports, we also retrieved 251 thousand domain name reports out of 295 thousand
(data processing step removed 200 thousand domain names from the dataset). 
A domain name report includes the set of categories assigned to the domain names by multiple multiple commercial
tools. For example, Websense categorizes a domain name into 1 out of 253 categories, which include advertisements, business and economy, job search and others.

\textbf{Data preprocessing.}
We follow the methodology established in~\cite{downloader_graphs} and perform necessary data preprocessing. First, we whitelist 165 thousand browser
nodes that are downloaded 6.6 million times over the dataset lifespan. Second, we remove non-executable files
because our local detectors, which are based on prior work~\cite{ling_dimva}, are not designed to work with non-binary files and also
VT lacks necessary tools for the analysis of non-binary files. The large portion of the dataset is composed of html and text files, it also includes various scripts such as asp, VB, php, bash and etc. 

We identify non-binary files using VT file reports if present or we analyze file extensions in the dataset. 
The latter approach is safe because files that lack corresponding VT reports are considered benign, thus their 
developers have no intention to masquerade their extensions. Data preprocessing shrinks the dataset down to 4.8 million benign and 96.3 thousand malicious files that are downloaded 36 million times.
%The set of non-binary files include 54 thousand
%malware samples. 


\textbf{Local detectors.}
LDs quickly analyze downloaded files by extracting syntactic features and using a classifier to determine whether they are malicious or not. Specifically, LDs extract the following information from binary files: they run existing commercial tools 
such TRID, ClamAV, Symantec, analyze statically imported libraries and functions, detect common packers, check whether a file is digitally signed or not, and obtain its binary metadata. 
The benign files lacking corresponding VT reports are assigned VT reports of other benign files at random.

Rather than actually running all these tools, we extract such
information from VT reports. To convert human-readable data into a set of feature vectors suitable from ML classifiers, we
rely on the recent work~\cite{ling_dimva}. However, it suffers from producing very high-dimensional feature
vectors that have limited usability due to "curse of dimensionality" 
and due to memory overhead, the latter results in often program crashes. To overcome such an issue, we use a common method for dimensionality reduction -- feature hashing~\cite{}. Empirically we found that the output dimensionality of 1024 allows us to 
achieve the best trade-off between classifier's performance and resource consumption. 

Finally, we train an xgboost classifier~\cite{xgboost} with 10-fold cross-validation 
and set area-under-the-curve (AUC) as classifier's objective. After parameter tuning, we achieve 97.19\% AUC, which
translates into 2.3\% false positive rate and 80.05\% true positive rate. Due to the high number of benign files in the
dataset, 2.3\% false positive rate corresponds to more than 107 thousand misclassified files.
We use out-of-fold predictions made by such classifier throughout the rest experiments.


\textbf{Domain name classifier.}
We also build a classifier to identify suspicious domains. For this purpose, we convert VT's domain name
classification -- categorical information assigned by commercial tools -- into feature vectors using one-hot
encoding. After that we train an xgboost classifier~\cite{} using 10-fold CV and 
AUC as an objective.
We do not use any explicit information in domain name reports that may reveal whether those domain names have
 ever served malware.
 As in the the case of LDs, we use an xgboost algorithm~\cite{xgboost} to predict probability of a particular domain name to be malicious. At the training stage we use domain names explicitly computed over the Wine dataset,
i.e. if a domain name has ever distributed malware, then it is labeled as malicious, otherwise it is benign. 
We notice that frequently the same domain servers both benign and malicious files. 

As before, we use out-of-fold predictions to assign labels predicted by the classifier to the domain names.
As a result, the classifier is able to achieve 85.33\% AUC, which corresponds to 19.5\% false positive rate and
71.86\% true positive rate. Note, such a classifier is not deployable by itself due to its high false positive rate.  Classifying urls rather than domain names, might increase accuracy, however, Wine dataset lacks such data.


%-- running experiments: NBD time window
%\textbf{Experiment parameters.}
%We use a neighborhood time window of 150 days and run a detector algorithm every 30 days.


\textbf{Neighborhoods.}
We define neighborhoods using a slightly modified watering hole template. Specifically, a neighborhood is 
a collection of files transitively downloaded from a suspicious domain within a neighborhood time window.
As in the case of the watering hole attack, the intuition behind such a neighborhood definition is
that if a process contacts a suspicious domain, it is likely to download malicious files and it's likely that
the original file is malicious also. By traversing downloader graphs, we recursively apply such intuition to
other files.

Technically the algorithm performs the following steps (Figure~\ref{downloader_graph}).
For each domain name the domain classifier outputs the probability of being malicious. If a domain is considered
malicious (globaldl.net), we start forming a neighborhood by identifying all files that access that domain within a NTW (chrome.exe on the figure) and
for each of them we perform a breadth-first search on the downloader graph.
While traversing downloader graphs in the BFS manner, we use domain name predictions of our domain name
classifier to discard files downloaded from likely benign domains (gravic.com).
Had the domain name classifier correctly identified all suspicious domains, then the neighborhood would include the following malicious files -- E, F, G, I. However, due to high false positive rate of the classifier, 
neighborhoods contain only 30\% malicious files.
%At the end of this step, a neighborhood includes files transitively
%reachable from a suspicious domain.


%\begin{table}[tbp]
%\centering
%\begin{tabular}{|l|c|c|c|c|c|}
%Parameter 												& CCS'15 & NDSS'17 & LDs 		& NBDs 		& Shape-GD + LDs \\
%\multirow{2}{*}{False Positives, samples}				&        &         & 107,186    &  664,064  & 32,886		 \\
%										 				&        &         &  2.3\% 	&  14.26\%  & 0.7\%			 \\
%\multirow{2}{*}{True Positives, samples}				&        &         & 77,123     &  70,710   & 63,395		 \\
%										 				&        &         &  80.05\% 	&  73.4\%   & 65.8\%		 \\										 				
%Early Detection, days          							&        &         & 203.1    	&  322.9    & 326.8			 \\
%Detecting after first\\ appearance in the dataset, days   &        &         & 0		    &  18.8		& 18.6		     \\
%\multirow{2}{*}{Early detection, samples} 				&        &         & 39,209     &  19,567   & 17,693		 \\
%														&        &         & 83.62\%    &  41.73\%  & 37.73\%		 \\
%Possible early detection, samples          				&        \multicolumn{5}{l}{46,886}							 \\
%Malicious samples				          				&        \multicolumn{5}{l}{96,335} 						 \\
%Benign samples					          				&        \multicolumn{5}{l}{4,657,166}						 
%
%\end{tabular}
%\label{fig:wine_file_table}
%\caption{My caption}
%\end{table}

\begin{figure}[tbp]
   \vspace{-0.0in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/windows/wine/file_table.pdf}\par
   \caption{Comparison of \sysname with prior work. \sysname outperforms CCS'15 in number of detected samples and early detection
   and it has 3 times lower false positive level in comparison to LDs.}
   \vspace{-0.2in}
\label{fig:wine_file_table}
\end{figure}

\textbf{Results.}
We evaluate performance of \sysname on the Wine dataset and compare it with 
the traditional approach -- a set of LDs deployed on end hosts~\cite{ling_dimva} -- and with the previous work~\cite{downloader_graphs}. Note, the other prior work~\cite{pup_ndss} is not directly comparable because it 
focuses on detecting malware delivery campaigns rather than detecting individual malware samples.

We simulate real-time malware detection with \sysname by replaying all file downloads in the Wine dataset -- each file has a time stamp associated with it. And we run \sysname every 30 days with the neighborhood time window set to 150 days. In our evaluation, we primarily focus on the following aspect -- aggregated statistics collected over the entire length of the simulation.% and temporal statistics collected during the live replay (remove this???).

Here we present two flavors of \sysname. The first one, which is denoted as "NBDs" in the 
table~\ref{fig:wine_file_table}), only outputs neighborhoods with high malware concentration and helps us understand
the role of neighborhoods in the entire system.
The second one, denoted as "Shape-GD + LDs", outputs alerts raised by LDs within suspicious neighborhoods. 
In our evaluation we
focus on the properties of the latter one and discuss its advantages over the previous work.


\textbf{Malware detection.} The 
We observe that previous work achieves low false positive rate -- 3.9\%~\cite{downloader_graphs} 
and 2.3\%~\cite{ling_dimva}, however, due to the large volume of benign files in the dataset, these numbers
correspond to high number of benign files labeled as malicious (185K and 107K respectively).

The key limitation of Kwon et al.'s~\cite{downloader_graphs} approach is that the system is capable of detecting
only malicious downloaders after they download several other files. Even though it reaches 96\% true positive
rate computed over malicious downloaders, it is able to reach only 42.95\% in our experiments because only 48\%
of all malware samples download other files. Therefore, 48\% is an upper bound for its true positive rate.
Hence, LDs do not suffer from such limitations and achieve twice higher true positive rate -- 80\%.

\sysname ("Shape-GD + LDs") outperforms both previous approaches in terms of false positive rate. 
Its FP rate is 5.6 times lower
than FP rate of Kwon et al.'s~\cite{downloader_graphs} approach and 3 times lower than LDs' FP rate. 
And this result is achievable due to the ability of neighborhoods filter out mostly benign files.
If we look at the column "NBDs", we notice that neighborhood-based filtering removes ~85.74\% benign files
from further analysis, i.e. neighborhoods select groups of nodes with high malware concentration -- 35\% on average. However, this effect comes at the cost of reduced true positive rate in comparison to LDs 
(73.4\% vs. 80\%). After running LDs within the suspicious neighborhoods (column "Shape-GD + LDs"), 
\sysname catches 65.8\% malware, which is 1.53 times higher than previous work~\cite{downloader_graphs}.


\textbf{Early detection.} The other feature of \sysname is the early malware detection.
When computing this parameter, we assume that all alerts raised by those systems can be
analyzed almost immediately upon receiving them and compare the time when an alert is received with 
the time stamp of its first submission to VirusTotal, which roughly corresponds to the time
when commercial detectors starts detecting a particular malware.

\sysname achieves early detection of 326 on 37.73\% of malware samples out of the samples that appear 
in the Wine dataset before they get submitted to VirusTotal. The same parameters for Kwon et al.'s system
is slightly less -- 29.1\%, however, those samples are detected only 25.24 days earlier than they appear on VirusTotal. The dramatic difference in early detection time between \sysname and Kwon et al.'s approach comes from the design of the system: Kwon et al.'s system needs to wait until a malicious downloader actually
downloads several other files before it can decide whether a file is malicious, while \sysname makes a decision
irrespective of subsequent downloads.



%\textbf{Aggregated analysis.}
%Results shown in the table~\ref{} clearly demonstrate that \sysname +LDs outperforms state-of-the-art approaches by a large margin.
%In addition to our main result, \sysname +LDs, we also present the results for pure neighborhood based detector -- NBDs,
%which show the contribution of neighborhoods in the final system.
%
%We see that the concept of neighborhoods efficiently discovers hidden malware strains and aggregates them into neighborhoods --
%the neighborhoods labeled as malicious cover ~73\% of malware samples and ~14\% benign nodes. 
%The average malware concentration within such neighborhoods is 35\%, which is higher than malware concentration in the entire dataset ~2\%. 
%LDs running on end hosts are capable of capturing a slightly higher portion of malware (~80\%) at the cost of
%pretty high false positive rate ~2.3\%.
%\sysname reduces the baseline LDs' false positive rate by more than 3 times (from 2.3\% down to 0.7\%), however,
%the true positive rate drops down only by 17.75\%. 
%Interestingly, LDs have higher true positive rate on the samples preselected by the neighborhoods than on the 
%entire data set -- 89.65\% vs. 80\%. This is likely to happen due to neighborhoods aggregating the samples
%that significantly affect shape property of the neighborhoods, and thus they have very distinct feature vectors.
%
%Besides reducing the false positive rate, \sysname provides early malware detection.
%\sysname discovers ~38\% of malware more than 300 days prior to VT on average and such malware remains in 
%the system less than 19 days. Obviously, LDs can capture the highest portion of malware early among all systems
%under comparison due to their ability to analyze all malware files as soon as they enter the system.
%Due to the distribution of early detection times having long tail, we can notice the more files are detected earlier than VT's timestamp, less the average early detection time is.
%
%For completeness we compute the same statistical parameters on a small subset that was used in previous 
%work~\cite{}. \sysname improves false positive rate by 2 times (3.67\% vs. 1.85\%). It achieves 51.66\% true positive
%rate, which means that it can be efficiently combined with~\cite{} to detect remaining malware samples in
%this subset. Its early detection parameters still outperform~\cite{} -- 209.8 days vs ... and 22\% of
%malware samples can be discovered.
%
%-- add Recall / Precision


